Hole Detection and Shape-Free Representation and Double Landmarks Based Geographic Routing in Wireless Sensor Networks

In wireless sensor networks, an important issue of Geographic Routing is local minimum problem, which is caused by hole that blocks the greedy forwarding process. To avoid the long detour path, recent research focuses on detecting the hole in advance, then the nodes located on the boundary of the hole advertise the hole information to the nodes near the hole.

==> Jianjun_template/figures/HDAR/Makefile <==
#---------------------------------------------------------------------------
#  Makefile for latex documents with enhancements to make notes and slides.
#  You must use my macros.tex file if you want to utilize the enhancements.
#     Copyright (c) Jim Griffioen, 1997
#
#  Targets include:
#       init:   type 'make init' before doing anything
#	config:	reset the configuration to "student bw slides"
#       sg:     change the group ownership on RCS files (use after running ci)
#	all:	make the dvi file
#	ps:	make postscript file
#	pdf:	make pdf file
#	html:	make an html version (broken down by subsection)
#       html-nosplit: same as html, but create a single html file
#	bib:	make the bibliography and then .dvi file
#	gv:	make postscript file and ghostview it
#	acro:	make pdf file and acroread it
#	x:	run xdvi on the .dvi file
#	me:	configure for me
#	student: configure for student
#	notes:	configure for notes
#	slides:	configure for slides 
#       bw:	configure for black and white output
#	color:	configure for color output
#	portrait: configure for portrait orientation
#	landscape: configure for landscape orientation
#	2up:	make postscipt with 2 slides per page (plus note area)
#	4up:	make postscipt with 4 slides per page (no note area)
#	webnotes: make tar file with .ps, 2up, 4up, and html for class web page
#	clean:	remove all generated files
#	cleanlatex:  only remove the .dvi, .aux, .bbl, .blg, .log files
#	cleanhtml:  remove the generated html directory
#---------------------------------------------------------------------------

# Define the LaTex file filenames
PAPER=  main

ALLTEXFILES=	${PAPER}.tex \
		maincontents.tex \
		abstract.tex \
		conclusion.tex \
		definition.tex \
		evaluation.tex \
		introduction.tex \
		overview.tex \
		

# Name of figure files - these must be generated files
# because 'make clean' will delete them.
# Do not include non-generated figs here.
GENERATED_FIGS= 

# Names of xfig files used to generate the above .ps files
# Note, this variable is only used to checkout the xfig files
# from the RCS directory
FIG_FILES= 

# Image files (e.g., GIFs or JPGs) to be used directly in HTML docs
IMAGES=	

# Movie files (e.g., Quicktime, AVI, MPEGS) to be used directly in HTML docs
ANIMS=	

# Name of figure files that are not generated
OTHER_FIGS=	

# Name of the Unix group to set the RCS file ownership to
GROUP= netfac

#---------------------------------------------------------------------------
# You should not need to modify anything below this point
#---------------------------------------------------------------------------

#---------------------------------------------------------------------------
# Makefile code needed by all makefiles
#
# This section assumes that the following makefile variables have already
# been defined above
#    PAPER=
#    ALLTEXFILES=
#    GENERATED_FIGS=
#    FIG_FILES=
#    IMAGES=
#    ANIMS=	
#    OTHER_FIGS=
#    GROUP=
#---------------------------------------------------------------------------

# Set TEXINPUTS to find my tex macrosfiles
TEXINPUTS= .:../macros:../../macros:/homes/griff/lib/macros:

#---------------------------------------------------------------------------
# Define the names of the programs to use
#---------------------------------------------------------------------------

# Programs
GRAP=		grap
TPIC=		tpic
FIG2PS=		fig2dev -Lps -m 0.7
FIG2PIC=	fig2dev -Ltpic -m 0.7
LATEX=		latex
BIBTEX=		bibtex
DVI_TO_PS=	dvips -Z -t letter -P cmz
TBL=		tbl
XDVI=		xdvi
RM=		rm
GREP=		grep
GS=		gv
PDFVIEWER=	acroread
LPR=		lpr
CONVERT=	convert
L2H=		latex2html
PS2PDF=		ps2pdf


# name of the config file - defined in macros.tex
CONFIGFILE= config.tex

# name of the latex2html init file
LATEX2HTML_INIT= /homes/griff/.latex2html_init

# printer to use
PRINTER= lp
PRINTER_OPT= -P${PRINTER}


#---------------------------------------------------------------------------
# Rules for Making
#---------------------------------------------------------------------------
.SUFFIXES: .tex .dvi .fig .ps .detex .g .tbl .pic .gif .jpg .bmp .tif .tiff .tex,v .fig,v .pdf
.tex.detex: 	; $(DETEX) $*.tex > $*.detex
.tex.dvi: 	; $(LATEX) $* 
.fig.pic:	; $(FIG2PIC) -Ltpic $<  |  $(GREP) -v ".baseline" > $*.pic
.fig.ps:	; $(FIG2PS) -Lps $< $*.ps
.gif.ps:	; $(CONVERT) $*.gif $*.ps
.jpg.ps:	; $(CONVERT) $*.jpg $*.ps
.bmp.ps:	; $(CONVERT) $*.bmp $*.ps
.tif.ps:	; $(CONVERT) $*.tif $*.ps
.tiff.ps:	; $(CONVERT) $*.tiff $*.ps
.pic.tex:	; $(TPIC) $*.pic > $*.tex
.g.pic:		; $(GRAP) $*.g | $(GREP) -v ".lf" > $*.pic
.g.tex:		; $(GRAP) $*.g | $(GREP) -v ".lf" > $*.pic ; $(TPIC) $*.pic
.tbl.pic:	; $(TBL) $*.tbl > $*.pic
.dvi.ps:	; $(DVI_TO_PS) -o $*.ps $*.dvi 
.ps.pdf:	; $(PS2PDF) $*.ps $*.pdf
.tex,v.tex:	; co $*.tex
.fig,v.fig:	; co $*.fig
.jpg,v.jpg:	; co $*.jpg
.gif,v.gif:	; co $*.gif
.bmp,v.bmp:	; co $*.bmp
.tiff,v.tiff:	; co $*.tiff
.tif,v.tif:	; co $*.tif

# Different Make options

all: ${PAPER}.dvi ${PAPER}.ps

${PAPER}.dvi: ${ALLTEXFILES} ${FIG_FILES} ${IMAGES} ${ANIMS} ${GENERATED_FIGS}
	$(LATEX) ${PAPER}

setgrp: 
	chgrp $(GROUP) RCS/*
sg: 
	chgrp $(GROUP) RCS/*

generated_figs: ${GENERATED_FIGS}

print: ${PAPER}.dvi

ps: ${PAPER}.ps

pdf: ${PAPER}.pdf

${PAPER}.ps: ${PAPER}.dvi

${PAPER}.pdf: ${PAPER}.ps

x: ${PAPER}.dvi
	$(XDVI) ${PAPER}.dvi &

gv: ps
	$(GS) ${PAPER}.ps &

gs: ps
	$(GS) ${PAPER}.ps &

acro: pdf
	$(PDFVIEWER) ${PAPER}.pdf &

bib: ${ALLTEXFILES} ${PAPER}.ps
	echo "#!/bin/sh" > .makbib
	echo $(LATEX) ${PAPER} >> .makbib
	echo $(BIBTEX) ${PAPER} >> .makbib
	echo $(LATEX) ${PAPER} >> .makbib
	echo $(LATEX) ${PAPER} >> .makbib
	chmod a+x .makbib
	./.makbib
	rm .makbib

me:
	cat $(CONFIGFILE) | sed "s/studenttrue/studentfalse/" > .tmp
	cp .tmp $(CONFIGFILE); rm .tmp
	cat $(CONFIGFILE) | sed "s/instructorfalse/instructortrue/" > .tmp
	cp .tmp $(CONFIGFILE); rm .tmp
instructor:
	cat $(CONFIGFILE) | sed "s/studenttrue/studentfalse/" > .tmp
	cp .tmp $(CONFIGFILE); rm .tmp
	cat $(CONFIGFILE) | sed "s/instructorfalse/instructortrue/" > .tmp
	cp .tmp $(CONFIGFILE); rm .tmp
student:
	cat $(CONFIGFILE) | sed "s/studentfalse/studenttrue/" > .tmp
	cp .tmp $(CONFIGFILE); rm .tmp
	cat $(CONFIGFILE) | sed "s/instructortrue/instructorfalse/" > .tmp
	cp .tmp $(CONFIGFILE); rm .tmp
slides:
	cat $(CONFIGFILE) | sed "s/slidesfalse/slidestrue/" > .tmp
	cp .tmp $(CONFIGFILE); rm .tmp
	cat $(CONFIGFILE) | sed "s/notestrue/notesfalse/" > .tmp
	cp .tmp $(CONFIGFILE); rm .tmp
notes:
	cat $(CONFIGFILE) | sed "s/slidestrue/slidesfalse/" > .tmp
	cp .tmp $(CONFIGFILE); rm .tmp
	cat $(CONFIGFILE) | sed "s/notesfalse/notestrue/" > .tmp
	cp .tmp $(CONFIGFILE); rm .tmp
color:
	cat $(CONFIGFILE) | sed "s/wantcolorfalse/wantcolortrue/" > .tmp
	cp .tmp $(CONFIGFILE); rm .tmp
bw:
	cat $(CONFIGFILE) | sed "s/wantcolortrue/wantcolorfalse/" > .tmp
	cp .tmp $(CONFIGFILE); rm .tmp
portrait:
	cat $(CONFIGFILE) | sed "s/landscapetrue/landscapefalse/" > .tmp
	cp .tmp $(CONFIGFILE); rm .tmp
landscape:
	cat $(CONFIGFILE) | sed "s/landscapefalse/landscapetrue/" > .tmp
	cp .tmp $(CONFIGFILE); rm .tmp
init:	config
config:
	/bin/echo '\\slidestrue' > $(CONFIGFILE)
	/bin/echo '\\notesfalse' >> $(CONFIGFILE)
	/bin/echo '\\instructorfalse' >> $(CONFIGFILE)
	/bin/echo '\\studenttrue' >> $(CONFIGFILE)
	/bin/echo '\\wantcolortrue' >> $(CONFIGFILE)
	/bin/echo '\\landscapefalse' >> $(CONFIGFILE)

html-split: $(PAPER).dvi
	$(L2H) -split 8 -bottom_navigation -info "" -local_icons \
	-init_file $(LATEX2HTML_INIT) $(PAPER).tex
	@echo copying $(IMAGES) $(ANIMS) into the $(PAPER) directory
	cp $(IMAGES) $(ANIMS) $(PAPER)

html: $(PAPER).dvi
	$(L2H) -split 0 -no_navigation -info "" -local_icons \
	-init_file $(LATEX2HTML_INIT) $(PAPER).tex
	@echo copying $(IMAGES) $(ANIMS) into the $(PAPER) directory
	cp $(IMAGES) $(ANIMS) $(PAPER)

html-nosplit: $(PAPER).dvi
	$(L2H) -split 0 -no_navigation -info "" -local_icons \
	-init_file $(LATEX2HTML_INIT) $(PAPER).tex
	@echo copying $(IMAGES) $(ANIMS) into the $(PAPER) directory
	cp $(IMAGES) $(ANIMS) $(PAPER)

html-noimages: $(PAPER).dvi
	$(L2H) -split 0 -no_images -no_navigation -info "" $(PAPER).tex
	@echo copying $(IMAGES) $(ANIMS) into the $(PAPER) directory
	cp $(IMAGES) $(ANIMS) $(PAPER)

htmlln:
	ln -s /homes/griff/lib/macros/html.sty.foremergencies html.sty

2up: ps
	2up -p${PAPER}-2pp.ps ${PAPER}.ps

4up: ps
	mpage -P -4 ${PAPER}.ps > ${PAPER}-4pp.ps

webnotes: 2up 4up html tar

tar:
	tar -vcf - ${PAPER}.ps ${PAPER}-2pp.ps ${PAPER}-4pp.ps ${PAPER} \
	| gzip > webnotes.tgz

clean: cleanlatex cleanfigs cleanps cleanhtml cleanpdf

cleanlatex:
	$(RM) -f *.aux *.bbl *.blg *.log *.dvi

cleanhtml:
	$(RM) -rf ${PAPER}

cleanfigs:
	$(RM) -f ${GENERATED_FIGS}

cleanps:
	$(RM) -f ${PAPER}.ps

cleanpdf:
	$(RM) -f ${PAPER}.pdf

ppp5:
	rsh ppp5 rm pap.ps pap.ps.gz
	cat ${PAPER}.ps | gzip > pap.ps.gz
	rcp pap.ps.gz ppp5:
	rsh ppp5 gunzip pap.ps.gz
	rm pap.ps.gz

ppp6:
	rsh ppp6 rm pap.ps pap.ps.gz
	cat ${PAPER}.ps | gzip > pap.ps.gz
	rcp pap.ps.gz ppp6:
	rsh ppp6 gunzip pap.ps.gz
	rm pap.ps.gz

ppp9:
	rsh 204.198.76.89 rm pap.ps pap.ps.gz
	cat ${PAPER}.ps | gzip > pap.ps.gz
	rcp pap.ps.gz 204.198.76.89:
	rsh 204.198.76.89 gunzip pap.ps.gz
	rm pap.ps.gz



==> Jianjun_template/figures/HDAR/abstract.tex <==
In wireless ad-hoc networks, an important issue of Geographic Routing is ``local minimum" problem, which 
is caused by ``hole" that blocks the greedy forwarding process. Existing geographic
routing algorithms use perimeter routing strategies to find a long detour
path when such a situation occurs. To avoid the long detour path, recent research
focuses on detecting the hole in advance, then the nodes located on the boundary of the hole
advertise the hole information to the nodes near the hole. Hence the long detour 
path can be avoided in future routing. We propose a heuristic hole detecting algorithm which 
can identify the hole easily and quickly. In addition, we quantitatively figure out the areas
in the vicinity of the hole that need to be announced the hole information. With such information,
a new routing scheme was developed. Simulation results illustrate
that our approach can achieve better performance in terms of the average length and number of hops of routing 
paths. Simulation also shows that our approach introduces very small computational complexity.




==> Jianjun_template/figures/HDAR/algorithm.tex <==
\section{Intermediate Targets Geographic Routing (ITGR)}
\label{algorithm}
In this section, we describe our routing approach. We also discuss how to merge the entries that contain pairs of 
shaded area and associated landmark. 




\subsection{Intermediate Targets Routing outline}



%Algorithm 1 shows the approaches to find  the shaded destination area when there is a hole that blocks 
%the routing path from a source node $S$ to a destination node $D$.
%We further present our intermediate targets routing algorithm. 
In ITGR routing algorithm, when a source node $S$ intends to send packets to the destination 
node $D$, it looks up its local cache to see whether $<$ $shaded\_des\_area$, $landmark$ $>$ exists 
and whether $D$ is in this area. If $S$ finds this kind of entry in its cache, it will consider the landmark as its 
tentative target and forward the packets to next hop. Otherwise, the  node $S$ will perform greedy or 
perimeter routing to forward  packets with destination node $D$ to next hop. 
Once the packets reach the destination, the destination  checks whether there is a landmark in the routing path or not. 
If there is, the destination will inform the source node $S$ to calculate the shaded area and then $S$ will update  
its local cache by the fresh entry $<$ $shaded\_des\_area$, $landmark$ $>$ . Hence, if node $S$ forwards packets to any nodes in
a shaded area in the future, it will
extracte the corresponding landmark node from its local cache as a tentative target and then forward packets
to next hop.




\subsection{Determining nodes located in shaded areas}

For a destination node $D$, how can we determine if it is located in a certain shaded area?
Normally, the area is enclosed by rays and partial edges of the hole polygon. 
For instance, in Fig.~\ref{fig2}, 
the area is enclosed by ray $BE$, the hole's edges from $B$ to $F$ 
and ray $FC$. While $S$ does not know node $F${'}$s$ location,
 we need to find other point as reference to evaluate if a destination node is located in the shaded area or not. 
Since no active nodes in the hole,  we can simply determine if the destination is in the area $EBPC$.
 
Suppose that points $S$,$B$ and $P${'}$s$ coordinates are $S(x_s,y_s)$,$B(x_b,y_b)$ and $P(x_p,y_p)$ respectively. 
 If a destination node $G$ satisfies the following three conditions, it must be located in the shaded area:
 \begin{enumerate}
\item $G$ and $P$ are located on the same side of line $SB$;
\item $G$ and $B$ are located on the same side of line $SP$;
\item $G$ and $S$ are located on different sides of line $BP$.
\end{enumerate} 
 
To determine it, we write line $SB${'}$s$ function as: 
\begin{displaymath}
\frac{y-y_s}{y_b-y_s}=\frac{x-x_s}{x_b-x_s}
\end{displaymath}

It can be written as: \\*
$(y_b-y_s)x-(x_b-x_s)y+(x_by_s-x_sy_b)=0$     (1)

Suppose G's coordinates are $G$$(x_g,y_g)$. To determine if $G$ is in the shaded area, 
the first step is to determine if $G$ and $P$ are in the same side of line $SB$.
We substitute $x$ and $y$ in the left term of (1) by $x_g$ and $y_g$ and derive an expression: \\*
$(y_b-y_s)x_g-(x_b-x_s)y_g+(x_by_s-x_sy_b)$    (2)


We then substitute $x$ and $y$ in the left term of (1) by $P${'}$s$ coordinates $x_p$ and $y_p$ and derive another expression: \\*
$(y_b-y_s)x_p-(x_b-x_s)y_p+(x_by_s-x_sy_b)$     (3) \\*

If the symbols of (2) and (3) are identical, $G$ and $P$ are located in the same side of line $SB$, 
we can continue to determine if $G$ is in the shaded area $T$. Otherwise, $G$ cannot be in the shaded area. 

The second step is to determine if $G$ and $B$ are located in the same side of line $SP$.We write line $SP${'}$s$ equation:\\*
$(y_p-y_s)x-(x_p-x_s)y+(x_py_s-x_sy_p)=0$     (4)\\*

Then we substitute $x$ and $y$ in the left term of (4) by $G${'}$s$ coordinates and $B${'}$s$ coordinates and derive two expressions:\\*
$(y_p-y_s)x_g-(x_p-x_s)y_g+(x_py_s-x_sy_p)$      (5)\\*
$(y_p-y_s)x_b-(x_p-x_s)y_b+(x_py_s-x_sy_p)$       (6)

 
If (5) and (6) have different symbols, $G$ cannot be in the shaded area.Otherwise, $G$ and $B$ are located in the same side of 
line $SP$. We then
write the line $BP${'}$s$ equation and substitute $G$ and $S${'}$s$ coordinates to the left term of this equation 
and then got two expressions. 
If the two expressions have different symbols, $G$ and $S$ are located in two sides of 
line $BP$. That is, $G$ is in the shaded destination area. Hence if the destination node $G$ satisfies all the three conditions 
$S$ can conclude that $G$ is located in the shaded area. 



\subsection{Entries combination}
If a node $S$ sends multiple times packets to different destinations, many entries with the 
format $<$ $shaded\_des\_area$, $landmark$ $>$ might be 
generated and be intended to be saved in the node's cache. Among these entries, some landmarks may be identical and some 
shaded destination areas may be overlapped. 
We would like to merge them to save spaces and provide efficient entry lookup in the future. So once a node $S$ sends packets to a destination 
and generates a fresh entry $<$ $area\_SUV$, $B$ $>$, 
it looks up the entries in its local cache and update them.
There are two situations $S$ needs to deal with, one is that $S$ finds an entry in its cache with the same landmark $B$ as the new generated entry. 
Another is that
$S$ finds an entry in its cache whose landmark is not $B$ but whose destination area and $area\_SUV$ are overlap each other.
%to see if 
%there is an entry with the same landmark. If there exists one, then the node updates the entry in its cache by combining the new 
%generated shaded area and the area associated with this landmark that has been saved in its cache.
In the first situation, suppose $S$ finds an entry $<$ $area\_SU^{'}V^{'}$, $B$ $>$ existing in its cache, $S$ then updates
its entries according to the following cases:\\*
Case1: $SU^{'}V^{'}$ $\subset$ $SUV$, that is: $U$ and $V$ are in different sides of $SU^{'}$,
$U$ and $V$ are in different sides of $SV^{'}$.(Fig.~\ref{fig6}) \\*
This scenario can be represented by points' coordinates as follows: Suppose 
that points $S$,$U$, $V$,$U^{'}$ and $V^{'}${'}$s$ coordinates are $S(x_s,y_s)$,$U(x_u,y_u)$, 
$V(x_v,y_v)$,$U^{'}(x_{u^{'}},y_{u^{'}})$ and $V^{'}(x_{v^{'}},y_{v^{'}})$ respectively. \\*
Then line $SU^{'}${'}$s$ equation is: \\*
$(y_{u^{'}}-y_s)x-(x_{u^{'}}-x_s)y+(x_{u^{'}}y_s-x_sy_{u^{'}})=0$  (7)\\*
We substitute $U$ and $V${'}$s$ coordinates in the left term of (7) and derive two expressions: \\*
$(y_{u^{'}}-y_s)x_u-(x_{u^{'}}-x_s)y_u+(x_{u^{'}}y_s-x_sy_{u^{'}})$  (8) \\*
$(y_{u^{'}}-y_s)x_v-(x_{u^{'}}-x_s)y_v+(x_{u^{'}}y_s-x_sy_{u^{'}})$  (9) \\*
If (8) and (9) have different symbols, then $U$ and $V$ are located in different sides of $SU^{'}$.\\*
Line $SV^{'}${'}$s$ equation is:\\*
$(y_{v^{'}}-y_s)x-(x_{v^{'}}-x_s)y+(x_{v^{'}}y_s-x_sy_{v^{'}})=0$  (10)\\*
We substitute $U$ and $V${'}$s$ coordinates in the left term of (10) and derive two expressions: \\*
$(y_{v^{'}}-y_s)x_u-(x_{v^{'}}-x_s)y_u+(x_{v^{'}}y_s-x_sy_{v^{'}})$  (11) \\*
$(y_{v^{'}}-y_s)x_v-(x_{v^{'}}-x_s)y_v+(x_{v^{'}}y_s-x_sy_{v^{'}})$  (12) \\*
If (11) and (12) have different symbols, then $U$ and $V$ are located in different sides of $SV^{'}$.\\*
The update of this scenario is: $S$ removes $<$ $area\_SU^{'}V^{'}$, $B$ $>$ then insert $<$ $area\_SUV$, $B$ $>$. \\*

\begin{figure}[!htp]
\begin{center}
\includegraphics[width=8.0cm]{mer_1.eps}
\end{center}
\caption{The case when $SU^{'}V^{'}$ $\subset$ $SUV$.}
\label{fig6}
\end{figure}





Case2: $SUV$  $\subset$ $SU^{'}V^{'}$, that is: $U^{'}$ and $V^{'}$ are in different sides of $SU$,
$U^{'}$ and $V^{'}$ are in different sides of $SV$.(Fig.~\ref{fig7}) \\* Their relative locations can still be
represented by points' coordinates as case 1.
The coresponding update is: $S$ does nothing. \\*

\begin{figure}[!htp]
\begin{center}
\includegraphics[width=8.0cm]{mer_3.eps}
\end{center}
\caption{The case when $SUV$ $\subset$ $SU^{'}V^{'}$  .}
\label{fig7}
\end{figure}

Case3: The area of $SUV$ and $SU^{'}V^{'}$ are overlapped and $U$ and $V$ are in different sides of $SU^{'}$, 
$U$ and $V$ are in the same side of $SV^{'}$. (Fig.~\ref{fig8})
The update is: $S$ removes $<$ $area\_SU^{'}V^{'}$, $B$ $>$ then insert $<$ $area\_SUV^{'}$, $B$ $>$. \\*

\begin{figure}[!htp]
\begin{center}
\includegraphics[width=8.0cm]{mer_2.eps}
\end{center}
\caption{One case when $SUV$ and $SU^{'}V^{'}$ are overlapped. }
\label{fig8}
\end{figure}


Case4: The area of $SUV$ and $SU^{'}V^{'}$ are overlapped and $U^{'}$ and $V^{'}$ are in different sides of $SU$, 
$U^{'}$ and $V^{'}$ are in the same side of $SV$. (Fig.~\ref{fig9})
The update is: $S$ removes $<$ $area\_SU^{'}V^{'}$, $B$ $>$ then insert $<$ $area\_SU^{'}V$, $B$ $>$. \\*

\begin{figure}[!htp]
\begin{center}
\includegraphics[width=8.0cm]{mer_4.eps}
\end{center}
\caption{Another case when $SUV$ and $SU^{'}V^{'}$ are overlapped. }
\label{fig9}
\end{figure}

Case5: The area of $SUV$ and $SU^{'}V^{'}$ are disjoint.The update is just to insert $<$ $area\_SUV^{'}$, $B$ $>$. \\*
In the above cases, we use the nodes' relative locations to determine two areas' inclusion relation. This method  is
avaliable for the areas caused by a hole. However, it may not avaliable for general cases of Computational Geometry.


The second situation is that  S generate a new entry 
$<$ $area\_SUV$, $B$ $>$, it looks up its local cache and 
finds an entry $<$ $area\_SU^{'}V^{'}$, $B^{'}$ $>$. $area\_SUV$ and $area\_SU^{'}V^{'}$
are overlapped. For instance, in Fig.~\ref{fig10}, when $S$ sends packets to $D$, its generates an area enclosed by
$EB$, the hole perimeter from $B$ to $F$ and line $FC$(the extension of $SP$), which is represented by $SBP$ and associated with landmark $B$. When
$S$ sends packets to node $D^{'}$ later, it generates an area represented as $SB^{'}P^{'}$ and associated with landmark $B^{'}$.
A naive update is to simply insert the new generated entry to $S${'}$s$ cache. However, the new entry and the existing entry share the area
$EBF^{'}C^{'}$. Hence, if $S$ wants to send packets to a node $G$ located in the shared area, $S$ will be confused how to figure 
out the intermediate target. So we must keep all the areas stored in a certain node to be disjoint. 
In this scenario, The area $EBF^{'}C^{'}$ is associated with two landmarks $B$ and $B^{'}$,
the paths from $B$ to $G$ and from $B^{'}$ to $G$ are both greedy. The distance from  $B^{'}$ to $G$ is farer away than that from 
$B$ to $G$. We mark $B^{'}$=$argMax(distance(B,G),distance(B^{'},G))$.
We would like to let area $EBF^{'}C^{'}$ only be associated with
$B^{'}$ since if $S$ wants to send packets to a node $G$ in area $EBF^{'}C^{'}$ in the future, the tentative target $B^{'}$ will
cause less potential recursively  tentative target finding than $B$.
In general case, we mark the fresh generated entry is $<$ $area\_SUV$, $B$ $>$, $S$ looks up its entry and finds an entry $<$ $area\_SU^{'}V^{'}$, $B^{'}$ $>$,
$area\_SUV$ and $area\_SU^{'}V^{'}$ are overlapped. There are four cases to update $S{'}$$s$ entries.\\*
\begin{figure}[!htp]
\begin{center}
\includegraphics[width=7.0cm]{overlap_1.eps}
\end{center}
\caption{The case when $SUV$ and $SU^{'}V^{'}$ with different landmarks are overlapped. }
\label{fig10}
\end{figure}



Case 1: $SU^{'}V^{'}$ $\subset$ $SUV$, that is: $U$ and $V$ are in different sides of $SU^{'}$,
$U$ and $V$ are in different sides of $SV^{'}$(Fig.~\ref{fig11}). \\*
The update is: \\*
If $B$ is $argMax(distance(B,G),distance(B^{'},G))$,
$S$  removes $<$ $area\_SU^{'}V^{'}$, $B^{'}$ $>$ and then
   inserts $<$ $area\_SUV$, $B$ $>$. \\*
If $B^{'}$ is $argMax(distance(B,G),distance(B^{'},G))$,$S$ inserts $<$ $area\_SUU^{'}$, $B$ $>$ and inserts $<$ $area\_SVV^{'}$, $B$ $>$. \\*  
$S$ does this update because once an area is the overlap of two areas, $S$ makes it be associated with the landmark that is
farer away from an arbitratry  node in the shaded common area for less recursive tentative targets finding in the future.    

\begin{figure}[!htp]
\begin{center}
\includegraphics[width=4.0cm]{overope_1.eps}
\end{center}
\caption{The case when $SU^{'}V^{'}$ $\subset$ $SUV$.}
\label{fig11}
\end{figure}


Case2: $SUV$  $\subset$ $SU^{'}V^{'}$, that is: $U^{'}$ and $V^{'}$ are in different sides of $SU$,
$U^{'}$ and $V^{'}$ are in different sides of $SV$.(Fig.~\ref{fig12}) \\*
The update is:\\ If $B$ is $argMax(distance(B,G),distance(B^{'},G))$, $S$  removes $<$ $area\_SU^{'}V^{'}$, $B^{'}$ $>$, then
inserts $<$ $area\_SUV$, $B$ $>$, $<$ $area\_SU^{'}U$, $B^{'}$ $>$ and $<$ $area\_SV^{'}V$, $B^{'}$ $>$.\\*
If $B^{'}$ is $argMax(distance(B,G),distance(B^{'},G))$, $S$ does nothing.

\begin{figure}[!htp]
\begin{center}
\includegraphics[width=4.0cm]{overope_2.eps}
\end{center}
\caption{The case when $SUV$ $\subset$ $SU^{'}V^{'}$ .}
\label{fig12}
\end{figure}


Case3: The area of $SUV$ and $SU^{'}V^{'}$ are overlapped and $U$ and $V$ are in different sides of $SU^{'}$, 
$U$ and $V$ are in the same side of $SV^{'}$. (Fig.~\ref{fig13})
The update is: 
If $B$ is $argMax(distance(B,G),distance(B^{'},G))$,$S$  removes $<$ $area\_SU^{'}V^{'}$, $B^{'}$ $>$ and then
inserts $<$ $area\_SUV$, $B$ $>$ and $<$ $area\_SVV^{'}$, $B^{'}$ $>$. \\*
If $B^{'}$ is $argMax(distance(B,G),distance(B^{'},G))$,then $S$ inserts $<$ $area\_SUU^{'}$, $B$ $>$.
\begin{figure}[!htp]
\begin{center}
\includegraphics[width=4.0cm]{overope_3.eps}
\end{center}
\caption{One case when $SUV$ and $SU^{'}V^{'}$ are overlapped.}
\label{fig13}
\end{figure}



Case4: The area of $SUV$ and $SU^{'}V^{'}$ are overlapped and $U^{'}$ and $V^{'}$ are in different sides of $SU$, 
$U^{'}$ and $V^{'}$ are in the same side of $SV$. (Fig.~\ref{fig14})
The update is: 
If $B$ is $argMax(distance(B,G),distance(B^{'},G))$,$S$  removes $<$ $area\_SU^{'}V^{'}$, $B^{'}$ $>$ and then
inserts $<$ $area\_SUV$, $B$ $>$ and $<$ $area\_SU^{'}U$, $B^{'}$ $>$. \\*
If $B^{'}$ is $argMax(distance(B,G),distance(B^{'},G))$,then $S$ inserts $<$ $area\_SV^{'}V$, $B$ $>$.
\begin{figure}[!htp]
\begin{center}
\includegraphics[width=4.0cm]{overope_4.eps}
\end{center}
\caption{Another case when $SUV$ and $SU^{'}V^{'}$ are overlapped.}
\label{fig14}
\end{figure}










 


\begin{comment}
\begin{algorithm}[bt] 
\begin{algorithmic}[1] 
\caption{{\em Intermediate Targets Routing}}
\label{algorithm2}
\WHILE{packets have not arrived destination D}
\STATE{$S$ looks up its local cache to see if any $<$ $shaded\_des\_area$, $landmark$ $>$ exists 
and if its forwarding packets{'}$s$ destination $D^{'}$ is in the shaded destination area}
\IF{$S$ finds $D^{'}$ is in a shaded destination area in an entry}
\STATE{$S$ counts the corresponding landmark node $B$ as tentative target $D^{'}$ and forwards packets to next hop $S_1$}
\STATE{$S \leftarrow S_1$}
\ENDIF
\IF{$S$ finds no such entry}
\STATE{$S$ forwards packets with destination $D^{'}$ by GPSR to next hop $S_1$}
\STATE{$S \leftarrow S_1$}
\ENDIF
\ENDWHILE
\IF{packets arrive $D$}
\STATE{$D$ check if there the path is detour}
\IF{the path is detour}
\STATE{$D$ informs $S$ the  landmark and local minimal node $P$}
\STATE{$S$ calculates the shaded destination area and  updates its local cache}
\ENDIF
\ENDIF
\IF{the  packets never arrives the destination after a certain TTL}
\STATE{the packets are discarded and the source node reports $D$ is unreachable.}
\ENDIF


\end{algorithmic}
\end{algorithm}
\end{comment}



\subsection{ITGR routing scheme}

\begin{figure}[hbt]
\baselineskip=10.2pt

{\scriptsize
  \noindent\underline{\bf S initiates sending a packet to destination node D} \\
  \text{~~~~}Looks up its local cache to see whether any $<$ $shaded\_des\_area$, $landmark$ $>$ exists 
and whether $D$ is in the shaded destination area; \\
  \text{~~~~}\textbf{if} finds $D$ is in a shaded destination area \\
  \text{~~~~~~~~}Counts the corresponding landmark node $B$ as tentative target $D^{'}$;\\
  \text{~~~~}forwards packets to next hop;\\
  \text{~~~~}S is waiting to receive ACK after sending the packet;\\
  \text{~~~~}\textbf{if} didn't receive an ACK after a certain TTL\\
  \text{~~~~~~~~}Reports that data sending fails;
  \\
  
  \noindent\underline{\bf When a node receives the data packet} \\
  \text{~~~~}Extracts the destination node from the packet's header; \\
  \text{~~~~}\textbf{if} this node is the destination node D\\
  \text{~~~~~~~~}Checks whether local minimal P and landmark B exists\\
  \text{~~~~~~~~}\textbf{if} they exist\\
  \text{~~~~~~~~~~~~}Sends an ACK and a $landmark\_exist\_msg$ to source containing the locations of B and P\\ 
  \text{~~~~~~~~}\textbf{else} sends an ACK to the source\\
  \text{~~~~}\textbf{else} looks up its local cache to see whether any $<$ $shaded\_des\_area$, $landmark$ $>$ exists 
and whether its forwarding packets{'}$s$ destination node is in the shaded destination area; \\
  \text{~~~~~~~~}\textbf{if} finds the destination node is in a shaded destination area \\
  \text{~~~~~~~~~~~~}Counts the corresponding landmark node $B$ as tentative target $D^{'}$;\\
  \text{~~~~~~~~}Forwards packets to next hop;\\
  \\
  
  \noindent\underline{\bf When a node receives $landmark\_exist\_msg$} \\
  \text{~~~~}Calculates the shaded area by the method in Shaded Area Calculation Algorithm; \\
  \text{~~~~}Updates its local cache; \\
  
  
}

\protect\caption{Intermediate Targets Routing Algorithm}
\protect\label{routingfig}
\end{figure}







The algorithm in Fig.~\ref{routingfig} describes the routing scheme when $S$ sends packets to $D$. 
%Suppose the packets record the landmark if the path is detour then the destination will know it. 
In this algorithm, the source node
$S$ looks up its local cache to see if any $<$ $shaded\_des\_area$, $landmark$ $>$ exists 
and if its forwarding packets' destination $D$ is in the shaded destination area. If 
$S$ finds $D$ is in a shaded destination area in an entry, $S$ will count 
the corresponding landmark node $B$ as tentative target $D^{'}$  and forwards packets to next hop node, say $S_1$,
then $S_1$ will begin the entry lookup and forward packets to next hop. If $S$ finds no such entry, 
$S$ forwards packets with destination $D^{'}$ by GPSR to next hop $S_1$, $S_1$ will begin the entry lookup 
and forwrding  operations. 
%So at the beginning when $S$ attempts to forward
%packets, the $D^{'}$ in the algorithm is the final  destination node $D$. But once an entry is found, the $D^{'}$
%will be replaced  by a landmark node. 
%In any step, if the packets are forwarded to the fixed destination $D$,line 1 to line 8 will be done.
The algorithm contains two aspects, one is to select an intermediate node as tentative target to 
conduct the ITGR routing algorithm, another is to calculate the $<$ $shaded\_des\_area$, $landmark$ $>$
entry and save it to a node's cache.Both of them can be peformed  recursively.

The recursion mostly happen in the scenario such  that $\angle$ $BSD$ $\geq$ $\frac{\pi}{2}$ and
$\angle$ $BDS$ $<$ $\frac{\pi}{2}$(Fig.~\ref{fig3}) or the situation that $\angle$ $BSD$ $<$ $\frac{\pi}{2}$ 
and $\angle$ $BDS$ $\geq$ $\frac{\pi}{2}$(Fig.~\ref{fig4}). Fig.~\ref{fig5} is an instance to generate the
$<$shaded\_des\_area, landmark$>$ 
entry recursively. The first time when $S$ 
wants to send packet to $D$, it generates and saves the entry $<$ $area\_SBP$, $B$ $>$  to its cache. 
When $S$ selects $B$ as its intermediate target for routing, it will meets local minimal node $P^{'}$ and generate an entry
$<$ $area\_SB^{'}P^{'}$, $B^{'}$ $>$, then $S$ will update its cache.

\begin{figure} [!htp]
\begin{center}
\includegraphics[width=8.0cm]{figure5.eps}
%\includegraphics[width=8.0cm]{path2.eps}
%\includegraphics[width=8.0cm]{hops.eps}
\end{center}
\caption{Recursively generate shaded areas and recursively conduct ITGR}
\label{fig5}
\end{figure}

Intermediate targets routing algorithm can be recursively conducted as well. Suppose the pairs of entries 
$<$ $area\_SP^{'}P$, $B$ $>$ and $<$ $area\_SB^{'}P^{'}$, $B^{'}$ $>$ have been stored in S's local cache after updating(Fig.~\ref{fig5}). 
When S is forwarding packets whose destination is $D^{'}$,
 it looks up its local cache and finds that 
$D^{'}$  is in the shaded area $SP^{'}P$ and $B$ is the landmark,so $S$ counts $B$ it 
intermediate target. Then $S$ tries to send the packet to $B$, it looks up 
it local cache and finds node $B$ is in the shaded area $SB^{'}P^{'}$ and $B^{'}$ is the landmark, so $S$ counts 
$B^{'}$ its intermediate target, then tries to send packet to $B^{'}$ by greedy routing. Then from $B^{'}$ to $B$, 
the path is generated by greedy forwarding; 
from $B$ to $D^{'}$ , the path is greedy forwarding as well. This recursive routing makes the routing path is constructed by 
a series of sub-paths, which are all greedy forwarding paths.










==> Jianjun_template/figures/HDAR/conclusion.tex <==
\section{Conclusion}
\label{conclusion}

In this paper, we presented a heuristic algorithm that detects the hole. 
The hole can be represented concisely and announced to the nodes nearby that
potentially incur detour paths by face routing. The node benefited from 
the hole information can adaptively adjust the forwarding hop to avoid long detour path.
The novelty of the approach is that a single node can detect the hole
efficiently and then the nodes near the hole can benefit from it. 
The experiments indicate that our approach results in significant shorter 
routing path and fewer hops than an existing geographic routing algorithm. And it only
causes few computational complexities.



==> Jianjun_template/figures/HDAR/definition.tex <==
\newcommand{\bibdir}{./}

\newcommand{\msgrange}{potential range}
\newcommand{\msgranges}{\msgrange s}
\newcommand{\closestneighbors}{$m$-width neighborhood}

\newcommand{\newunstruct}{new unstructured}



==> Jianjun_template/figures/HDAR/discussion.tex <==
\section{Discussion}
\label{discussion}
In this section, we will discuss the method how to figure out the value of $\delta$, the 
situations  that will cause false positive or false negative when detecting holes and two
types of special circumstances about the hole representation.


\subsection{Derivation of the threshold}
\begin{comment}
In this paper, we define that a hole is a kind of polygon. In this kind of polygon, 
there exists a node p that is a vertex and satisfies that: a node d among the polygon's vertices can 
be found, p is closer to d than any of its neighbors but p cannot reach d directly. P is called local 
minimum node. Our hole detection algorithm is to detect such polygon that containing at least one local 
minimum node. 
\end{comment}
%We consider it is a hole. 

In geographic routing, when a hole exists, there will be a detour path. So we attempt 
to detect a hole by finding a detour path. The ``detour" path is defined as the routing path 
between two nodes that is much longer than their Euclidean distance in this paper. In order to quantitatively represent the 
``much longer", we introduce a threshold $\delta$ that is $length\_pro()/dist\_euc()$. To determine the value of $\delta$, 
we first attempt a polygon like a circle(Fig.~\ref{dis1fig}) in which $\delta$ is $\pi/2=1.57$. However, the circle is not a hole, 
so we will investigate $\delta>1.57$.
\begin{figure}[!htp]
\begin{center}
\includegraphics[width=4.0cm]{dis1.eps}
\end{center}
\caption{A circle is not a hole}
\label{dis1fig}
\end{figure}

We then increase the value of $\delta$. Suppose triangle $abp$ is a regular triangle(Fig.~\ref{dis2fig}), the length of each edge is 1, 
and the transmission range is slightly less than 1, such as 0.9. Then we move a to $a^{'}$ and let both $a^{'}p$ and $a^{'}b$ be equal to the 
transmission range. Then from $p$ to $b$, a path $p \rightarrow a' \rightarrow b$ exists and it is a slight detour path. 
But the triangle is not a hole since none of the three nodes is a local minimum node. In this circumstance,
the value of $\delta$ is approximate equal to 2.

\begin{figure}[!htp]
\begin{center}
\includegraphics[width=4.0cm]{dis2.eps}
\end{center}
\caption{A regular triangle is not a hole}
\label{dis2fig}
\end{figure}

Then we increase the value of $\delta$ to the one that is slightly larger than 2.
We found that $\delta$ =2.25 is a good choice for small false positive and small false negative
by experimental attempts.


\subsection{Discussion of false positive and false negative}
The false negative  and false positive may occur during the hole detection. 
The false negative occurs when the Euclidean distance from a source node to the destination node is close to the
transmission range and the detour path is slightly larger than the Euclidean distance.
%, such as the detour is one more hop than the Euclidean distance. 
For instance, in 
Fig.~\ref{dis3fig}, the transmission range is 0.9,$\mid pd \mid$=0.95, $\mid ad \mid$=$\mid bd \mid$=1,$\mid ed \mid$=$\mid df \mid$=0.9
and $\mid ap \mid$=$\mid pb \mid$=0.9. Then $p$ is a local minimum node and the polygon $paedfb$ is a hole. However, HDAR 
does not detect it is a hole. The false negative is introduced by a very special circumstance that the detour path is
about one hop distance longer than the Euclidean distance. If the detour is longer, then $\delta$ will be greater than
2.25 and the polygon will be considered as  a hole. If the Euclidean distance from $p$ to $d$ is much larger than the transmission
range, the polygon is a long and narrow area. The $\delta$ will be less than 2.25 from $p$'s point of view. But node $e$ or $f$ 
will detect the long and narrow polygon is a hole. The false negative in Fig.~\ref{dis3fig} will not affect the routing too much
because the detour is not too long, normally one hop.


\begin{figure}[!htp]
\begin{center}
\includegraphics[width=4.0cm]{dis3.eps}
\end{center}
\caption{False negative when detecting hole by HDAR}
\label{dis3fig}
\end{figure}

False positive occurs when Euclidean distance from a source node to the destination node is slightly larger than the
transmission range and the detour path is at least three hops long, and each hop is close to the transmission range.
 For instance, in 
Fig.~\ref{dis4fig}, the transmission range is 0.9,$\mid pd \mid$=1, $\mid ed \mid$=0.95,
and $\mid ep \mid$=$\mid ea \mid$=$\mid ad \mid$=$\mid dc \mid$=$\mid cb \mid$=0.9. Where 
 $p$ is not a local minimum node and then the polygon $peadcb$ is not a hole by hole's original definition. 
 However, HDAR 
detects it is a hole. And node $e$ and $p$ will advertise the hole information to an area $epk$. 
The area to be announced is not big
since only a few nodes(two nodes in this example) announce the hole information. If there are more nodes located in any edge such as 
$ea$ or $ep$, then the polygon is a true hole. Although this is a ``pseudo hole" detected by HDAR, the nodes in $epk$ will benefit from the hole information. 
For example, if $s$ wants to send
a packet to $d$, $s$ will send the packet to a directly(green path) instead of detour from $p$(red paths). The false positive 
will occur in very special situations. And the further hole announcement to a small area is not an expensive  task. But the nodes in this 
area will benefit from the hole information.


\begin{figure}[!htp]
\begin{center}
\includegraphics[width=6.0cm]{dis4.eps}
\end{center}
\caption{False positive when detecting hole by HDAR}
\label{dis4fig}
\end{figure}


\subsection{Further discussion of the hole representation}

The hole is represented by a segment that connects the most remote two nodes of the hole in this paper.
However, there may be a second segment that is a little shorter than the segment standing for the hole
and they are almost perpendicular. We will discuss how this situation affects the future routing by two
types of hole shapes. 

In the first type, the shape of hole is a convex polygon(Fig.~\ref{app1fig}). $ef$ represents the hole. There is a second 
segment $ch$ that is a little shorter than $ef$. We fit this polygon by a circle. When node $a$ intends to send a packet to node
$d$, who is on the same side of $a$ relative to $ef$, only GPSR can be used in our routing protocol. Since $a$ and $d$
 are located on the
boundary of a circle, $a$ can always find another node $b$ or $c$ or $g$ that is closer to $d$ as its next hop. So greedy forwarding
is available. In this circumstance, no matter which segment representing the hole will not affect the future routing.






\begin{figure}[!htp]
\begin{center}
\includegraphics[width=8.0cm]{app1.eps}
\end{center}
\caption{The polygon is fitted as a circle}
\label{app1fig}
\end{figure}



The hole is concave in the second type(Fig.~\ref{app2fig}). $ef$ represents the hole. There is a second 
segment $ch$ that is a little shorter than $ef$. We fit this polygon by a 3-regular tree in Poincare disk~\cite{ex31}. 
It can be considered as two sets of hyperbola. They divided the plane into four regions I,II,III and IV by
arc $fh$,$fc$, $ce$ and $eh$ excluding the hole. We illustrate that the possible detour will not be too much by an example node $a$.
When $a$ located in region III wants to send a packet to node $b$, $a$
 finds that $e$ is the tentative target and
the path is constructed by $ae$ and $eb$, both are greedy. When $a$ sends a packet to $g$, since $a$ and $g$
 are on the same side of segment $ef$, $a$ uses greedy to reach $k$, then from $k$ to $c$ by face routing and from $c$ to $g$ by greedy. 
When $a$ sends a packet to $d$, $a$ considers
$f$ as tentative target. Then the path will be constructed by $aj$,$jc$,$cf$ and $fd$, where $jc$
 is face routing path. So no matter what regions 
the source and destination nodes are located, there is at most one piece of face routing path included in one region. And it will not be 
two long. 



\begin{figure}[!htp]
\begin{center}
\includegraphics[width=8.0cm]{app3.eps}
\end{center}
\caption{The polygon is fitted as hyperbolas}
\label{app2fig}
\end{figure}










==> Jianjun_template/figures/HDAR/evaluation.tex <==
\section{Performance Evaluation}
\label{evaluation}

We conduct our performance evaluation using a
noiseless immobile radio network environment, where the nodes are
distributed in a given area and may each have a different
transmission range and bandwidth. 
Since what we are interested in is to
compare our results with the outputs generated by other allocation
approaches, we convert this network to a weight graph G=(V,E) where
the weight represents the bandwidth. 
We set the number of users to be 30 and 
let the number of channels vary from 25 to 50 with increment 5. 
We set the probability
that an edge exists between any pair of user and channel nodes to be 0.2 
and the edge weight is uniformly distributed from
1 to 9.
For each 
% pair of user number and channel number, 
configuration, 
we 
% randomly 
generate 10 graphs and
conduct the experiment 10 times based on the graphs. 
We calculate the average value from the experiments as the result 
for each configuration.

We use two metrics to evaluate the performance.
One is
%  system utilization, i.e., 
the sum bandwidth of all users by the allocation.
The other is the allocation ratio of the number of users 
who are allocated with at least one channel 
over the number of users who are competing for the spectrum pool.

We compare our solution with three other approaches. The first one 
is NMSB
(Non-collaborative-Max-Sum-Bandwidth). In each step, this approach
picks the vertex with the highest bandwidth and assigns it to its
associated user. Then the algorithm remove the edges that interfere
with this user until all the channels are allocated. The second one
is 
CMSB (Collaborative-Max-Sum-Bandwidth). This approach picks up
the vertex with the highest label, defined as the bandwidth of a
channel 
divided by the number of users interfering with each other with 
regard to this channel. The process is repeated until all channels
have been allocated. The
third approach is MINSTARVE, which tries to allocate the
channels to the users who have not been allocated before. In
this approach, each user has a priority. The user's priority is
decreased by one if the user is allocated with a channel. The
algorithm takes care of higher priority users first.

\begin{figure}[!htp]
\begin{center}
\includegraphics[width=8.0cm]{Fig8.eps}
\end{center}
\caption{Sum bandwidth of allocated channels} \label{fig11} 
\end{figure}

In Fig.~\ref{fig11}, we evaluate the sum bandwidth of these approaches.
The number of channels changes from 25 to 50. The results show
that our approach can achieve near optimal sum bandwidth, similar to 
NMSB.
Both NMSB and our approach are about 10\% to 25\% higher than
the other two approaches.


\begin{figure}[!htp]
\begin{center}
\includegraphics[width=8.0cm]{Fig9.eps}
\end{center}
\caption{Allocation ratios} 
\label{fig12} 
\end{figure}

In Fig.~\ref{fig12}, 
% has the identical network setting as fig 11. But what we concern is 
we evaluate the allocation ratio of the four approaches.
It shows that our algorithm can reach near 100\%
allocation ratio. MINSTARVE is close to 80\%, while the other two
range from 40\% to 70\%. It illustrates that our mechanism can 
better avoid starvation. 

% Combined by the two figures, we can see that Bipartite-graph based
% approach can guarantee as many as possible users to be benefit from
% spectrum and achieve large sum bandwidth as well.


==> Jianjun_template/figures/HDAR/hdar.tex <==
\section{Hole Detecting and Adaptive Routing}
\label{Algorithms}

\subsection{Hole Detection Algorithm}
In HDAR, a node $p$ begins to detect whether it is located on a hole only if the angle between its two 
adjacent edges is greater than 120 degrees~\cite{ex22}.
% This is because if there is no angle between 
%two adjacent edges respect to $p$ that is bigger than 120 degrees, $p$ can not be a local minimum node. 
$p$ initiates a probe message and writes its location to this message. Then $p$ sends the message to its 
leftmost node respect to the angle. Where the leftmost node is defined as: $p$ faces the area formed by the two rays of 
this angle, then $p$ uses the angle's bisector line to conduct anti-clockwise sweeping, the leftmost node is the first one that met
by the sweeping line. Upon receiving the probe message, $p$'s leftmost neighbor node writes 
its location into the message and passes it to its leftmost neighbor, here the leftmost or rightmost neighbor is defined similarly. The probe message will finally come back 
to node $p$ from $p$'s rightmost neighbor respect to the initial invested angle~\cite{ex22}~\cite{ex30}. 
When the probe message circulates, 
it collects the locations of the nodes on its way. So node $p$ knows all the nodes' locations on the way.


$p$ then begins to investigate the nodes on the way ordered clockwisely. For each node on the way, $p$ computes the length of their probe path $length\_pro()$ 
and their Euclidean distance $dist\_euc()$. For a node $x$, $length\_pro(p, x)/dist\_euc(p, x)$ is defined as hole detection ratio $p$ 
to $x$.
If there exists a node $v$, the hole detection ratio $p$ to whom is larger than a predefined threshold $\delta$, that is,\\
 \text{~~~~~~~~}$length\_pro(p, v)/dist\_euc(p, v)$ $>$ $\delta$ \text{~~~~~~~~}(1) \\
is satisfied, 
then $p$ is considered sitting on a hole. The value of $\delta$ affects the hole detection results. Too big value of $\delta$ introduces 
false negative and too small value of $\delta$ causes false positive. We derived that  $\delta$=2.25 is a good choice to detect 
most holes that will block greedy forwarding.
Fig.~\ref{hdarfig1}  is an example for hole detection. Node $p$ initiates the hole probe message. $p$ collects the nodes' 
locations during the message circulates the loop. Then $p$ finds that there exists a node $v$, 
satisfying $length\_pro(p, v)/dist\_euc(p, v)$ $>$ 2.25 , $p$ is considered sitting on a hole.

\begin{figure}[!htp]
\begin{center}
\includegraphics[width=6.0cm]{fig1.eps}
\end{center}
\caption{P initiates the probe message and it circulates the loop}
\label{hdarfig1}
\end{figure}


The hole that was detected is a polygon. Note that some nodes located on the polygon measure they are 
located on a hole, but other nodes may not consider they are on a hole. For instance, 
in Fig.~\ref{hdarfig1}, node $g$, $p$ and $h$  consider they are on a hole since there exist nodes on the polygon's
boundary to let them satisfy the hole definition (1). However, 
the vertexes $a$ and $b$ at the hole polygon found by $p$ don't consider they are on a hole because $a$ or $b$'s greedy
forwarding will not be blocked
%  does not have to generate detour routing path in future routing due to 
by the polygon. 
%That is, the polygon has minor effect to $a$ or $b$ for their  routing paths.

The node located on the polygon may detect the hole repeatedly, thus a lot of overhead will be generated. 
%In order to reduce the overhead, asynchronous detection is introduced. That is, one will send out the probe 
Fortunately, the overhead can be reduced because of the 802.11 MAC layer random backoff mechanism. In this mechanism,
one will not send out a packet 
%its probe message 
if it overhears an RTS sent to other node.
%that another node in its transmission is sending out a probe message.
Instead, it will wait for a period and then begin to send out its packet only when it hears the CTS plus a period. 
% asynchronous detection is introduced. That is, one will send out the probe 
%message and others will receive it  before sending out theirs. 
We use this mechanism that once a node hears a probe message, it would not schedule a probe message although it has 
not sent out its probe message yet.
% when a probe message comes to it. 
However, a node sitting on the polygon may only 
receive partial of the nodes' information based on this mechanism if the received probe does not start from this node. 
In order to make each node know the locations of all the nodes on the polygon, the probe initiating node sends two probe 
messages clockwise and anti-clockwise at the same time.(shown in Fig.~\ref{hdarfig1}). So each node on the polygon can obtain
the whole information of the polygon. Since the probe message is sent  by both clockwise and anti-clockwise directions,
there will be two probe paths, we choose the longer as the length of the probe path to calculate the hole detection ratio. 

The probe message initiating algorithm is described as Fig.~\ref{initiatefig}.


\begin{figure}[hbt]
\baselineskip=10.2pt
{\small
  \noindent\underline{\bf Probe\_msg\_initiating()} \\
  %\text{~~~~}\textbf{if} receives a probe message \\
  \text{~~~~}\textbf{if} doesn't receive a probe message \\
  %\text{~~~~~~~~}cancel probe\_initiate message; \\
  %\text{~~~~~~~~}\textbf{else} search whether it has an angle between two adjacent edges \\
  \text{~~~~~~~~}\textbf Search whether it has an angle between two adjacent edges \\
  \text{~~~~~~~~}larger than 120 degrees; \\
  \text{~~~~~~~~}\textbf{if} true \\
  \text{~~~~~~~~~~~~}Initiate a probe message; \\
  \text{~~~~~~~~~~~~}Write its location to this message; \\
  \text{~~~~~~~~~~~~}Send it to its left node and right node of the angle.\\
  %\text{~~~~~~~~}\textbf{else}\\
  %\text{~~~~~~~~~~~~}cancel probe\_initiate message. \\
 }

\protect\caption{Probe Message Initiating Algorithm}
\protect\label{initiatefig}
\end{figure}


 The probe message receiving algorithm is described as Fig.~\ref{receivefig}. In this algorithm,
upon receiving a probe message, a node determines whether it is the message initiate node. If it is,
the node will calculate the hole detection ratio when both probe massages come back.  If the node is not the 
message initiate node, it will write its location to the message and forward the message.


\begin{figure}[hbt]
\baselineskip=10.2pt
{\small
  \noindent\underline{\bf Probe\_msg\_receiving()} \\
  \text{~~~~}Compare its location with the message initiator's location to \\
  \text{~~~~}determine whether it is the message initiator \\
  \text{~~~~}\textbf{if} it is the initiator \\
  \text{~~~~~~~~}Search whether the two probe message from  \\
  \text{~~~~~~~~}different directions both reached it; \\
  \text{~~~~~~~~}\textbf{if} true \\
  \text{~~~~~~~~~~~~}Calculate the hole detection ratio \\
  \text{~~~~~~~~}\textbf{else} \\
  \text{~~~~~~~~~~~~}Wait for the second probe message; \\
  \text{~~~~}\textbf{else} \\
  \text{~~~~~~~~}Write its location;\\
  \text{~~~~~~~~}Forward the message to its left or right neighbor\\
  \text{~~~~~~~~}according to the forwarding direction.\\
 }

\protect\caption{Probe Message Receiving Algorithm}
\protect\label{receivefig}
\end{figure}







The probe initiator must have an angle between two adjacent edges with respect to it that is larger than 120 degrees. 
However, such an angle is necessary but not sufficient condition to determine the initiator is a local minimum node, 
but this does not affect our hole detection results since the initial node being regarded as  a local minimum is independent on the fact
that the node detects a hole. A relative destination is needed to determine a local minimum but our hole detection
algorithm does not need a specific destination.
 The objective of the hole probe message is to find a hole, but not to determine if 
the probe initiator is a local minimum node. 

The probe initiator who finds a hole finally may be or may not be 
a local minimum node. In Fig.~\ref{hdarfig1}, node $p$ initiates the hole probe message and finds that it is 
located on a hole. It is a local minimum node if it sends a packet to nodes in the vicinity of node d. In Fig.~\ref{hdarfig2}, node p 
initiates a hole probe message and detects the hole, but $p$ is not a local minimum node. The hole information 
will be announced to the nodes in a certain area and these nodes will be benefited from the hole announcement for future routing. 
%This situation occurs when there is a hole, but the hole probe message is initiated by a node that is not a local minimum node. 


In Fig.~\ref{hdarfig3}, $p$ is a local minimum node. $p$ initiates a hole probe message but it cannot detect the hole 
because the length of 
the probe path from $p$ to any node on the polygon over their Euclidean distance is approximate to 1. However, the hole can be 
detected by another node such as $n$ and the hole information will be announced to areas($ekf$ and $e^{'}k^{'}f^{'}$) containing 
the nodes which will be benefited 
from the hole information in future routing. This phenomenon that a true local minimum node $p$ cannot detect a hole 
occurs when the polygon is long and narrow then the initiator's 
routing will not be blocked by the polygon. So this detecting result has very minor effect to $p$'s forwarding.
Nevertheless, the hole will be detected by another node who suffers from the hole. 
%The hole detected by other node has very minor effect to p's forwarding. And by 
%our determining condition, the ratio of the length of p's probe path to any node in the hole over the Euclidean distance is 
%close to 1. 
%So the effect of this polygon to node $p$ and the hole detection ratio defined in this paper are consistent.


\begin{figure}[!htp]
\begin{center}
\includegraphics[width=6.0cm]{initiator2.eps}
\end{center}
\caption{P is not a local minimum but finds the hole}
\label{hdarfig2}
\end{figure}


\begin{figure}[!htp]
\begin{center}
\includegraphics[width=6.0cm]{initiator3.eps}
\end{center}
\caption{P is a local minimum but does not find the hole}
\label{hdarfig3}
\end{figure}

\subsection{Shape-Free Hole Representation}
The hole that is detected is a polygon. The representation of a polygon is a sequence of vertexes. 
However, in geographic routing, we don't have to care all the nodes on the polygon because most of 
them have minor effect to determine the routing paths. What we concern are the nodes that will block the 
greedy forwarding.
In our model, since $p$ has already obtained all the nodes' locations on the polygon(Fig.~\ref{hdarfig2}), 
$p$ calculates the two nodes whose Euclidean distance is most remote. The segment connecting these 
two nodes looks like a board that blocks the greedy forwarding. For instance, segment $ab$ in Fig.~\ref{hdarfig2} is 
the board that blocks the greedy forwarding. Then the hole is represented as $<a,b>$. 
No matter what the shape of the hole is, what we concern is 
the segment connecting the two most remote nodes.


\subsection{Determining the Shaded Area}
That the greedy forwarding is blocked by the board $<a,b>$ is because some potential  destination nodes 
are hidden behind the board, and the source nodes located in a certain area that is in the opposite 
side to the hidden destinations are not aware of them. In the basic routing approach, a source 
node just conducts the greedy forwarding until it fails due to the local minimum node, where the greedy 
forwarding changes to face forwarding. Thus the detour paths are generated. If the possible destination nodes 
hidden behind the board can be figured out in advance and be announced to the source nodes in the certain area, 
the length of the routing paths can be dramatically reduced. We determine the possible destination area(shaded area)
as follows: Draw line $ar$ perpendicular to segment $ab$, $r$ and $p$ are at the opposite sides of $ab$. Also draw line $bt$ 
perpendicular to line $ab$, $t$ and $p$ are at  the opposite sides of ab. Then the area $rabt$ is the shaded area(Fig.~\ref{hdarfig4}). 



\subsection{Hole Announcement}
The nodes in area $rabt$ are the possible destination nodes associated with some source nodes. 
We would like to figure out an area containing these source nodes that will be announced 
the hole information in the opposite side of $rabt$(Fig.~\ref{hdarfig4}). The hole information will help 
the nodes adaptively adjust the next forwarding hops to avoid detour routing paths. 
In order to determine the hole announcement area, the announcement breadth and depth 
need to be figured out. We first find node $e$ and node $f$ at the same side as node $p$ 
relative to segment $ab$ that are the left and right nodes furthest away from each other and satisfy the hole 
detection condition (1). Let $c$ be the midpoint of segment $ef$. Draw segment $ck$ perpendicular 
to $ef$. Then the triangle $efk$ is the area that should 
be announced the hole information. Note that hole announcement area is larger, 
more nodes will be advertised the hole information and the future routing path will be shorter. 
However, the area is larger, more overheads will be introduced. 
So there is a tradeoff between the benefit to the future routing path and the overhead. 
The optimal values of the hole information announcement size that can both shorten 
the future routing path and reduce the overhead need to be found. The announcement 
breadth is selected as segment $ef$ since $e$ and $f$ are most remote nodes on the hole's boundary
located on the same side of $p$ satisfying the hole detection condition.
%is the leftmost node that satisfies the 
%hole detection condition and $f$ is the rightmost node that satisfies the hole detection 
%condition. 
So the announcement depth determines the size of the area. 
We let the length of $ec$ be $l$ and
% approximate the length of $ef$ to be $L$. And we 
mark $\angle cek$ to be $\alpha$.
Assume that the nodes are distributed in the plane uniformly. So the number of the nodes in $\bigtriangleup$ekf
can be represented by the area of $\bigtriangleup$ekf:\\
\text{~~~~~~~~}$\frac{1}{2}$$\cdot$$2l$$\cdot$$l$$\tan\alpha$$=$$l^{2}$$\tan\alpha$,$\alpha\in\lbrack0,\frac{\pi}{2}\rbrack$ \\
For node $s$, if it intends to send a packet to node $d$ by HDAR routing protocol, the path includes the sub-paths $s \rightarrow k$,
$k \rightarrow e$, $e \rightarrow a$ and $a \rightarrow d$. The last two sub-paths are fixed, 
but $s \rightarrow k$ and $k \rightarrow e$ depend on $\alpha$. Let the length of $sc$ be $h$, 
we approximately represent the length of path $sk$ by $h-\mid kc\mid=h-l$$\tan\alpha$,
and the length of path $k \rightarrow e$ by $\mid ke\mid$ since the routing path generated by HDAR 
will be along $ke$. Here  $\mid ke\mid$ is $\frac{l}{\cos\alpha}$. Hence from $s$ to $e$, the length of paths is:\\
\text{~~~~~~~~}$(h-l$$\tan\alpha)+\frac{l}{\cos\alpha}$     \\
We want to find an $\alpha$ that can try to minimize both the area of $\bigtriangleup$ekf and the length of routing path.
The optimal value to minimize both is depended on $\alpha$. We deduced that the best solution is that when $\alpha$ is 1.05. 
We approximate the length of $ef(2l)$ to be $\mid ab\mid$. Then the optimal length of the depth ck 
is $\tan\alpha$*$\frac{1}{2}\mid ef\mid$, that is: $0.87*\mid ab\mid$. The details will be discussed in the appendix. 

The nodes on the arc $ef$ begin to advertise the hole information $<a,b>$ to their neighbors. 
In order to avoid duplicate messages, once a node in 
the area has received the hole information, it simply discards the duplicate. 
After the  advertisement of hole's information, each node in the area $efk$ knows that any possible 
destination node in area $rabt$ is hidden behind the the board $<a,b>$(The red nodes and boundary nodes from $e$ to $f$
in Fig.~\ref{hdarfig4}) .

\begin{figure}[!htp]
\begin{center}
\includegraphics[width=6.0cm]{main.eps}
\end{center}
\caption{Hole Announcement}
\label{hdarfig4}
\end{figure}





\subsection{Adaptive routing}
After the announcement, each node in the triangle $ekf$ knows that there is a hole $<a,b>$ that blocks the greedy 
forwarding to any destination node in area $rabt$. So the nodes in triangle $ekf$ can adaptively adjust the routing 
path. In the network plane, once a node $s$ intends to send a packet with destination $d$, it first looks up its local 
cache to see whether it has a hole information entry $<a,b>$. If there is no such entry in its local cache, it just 
conducts GPSR. Else if there is a hole information entry $<a,b>$ but $s$ and $d$ are located at the same side of segment 
$ab$, $s$ just conducts GPSR. If $s$ and $d$ are located on the opposite sides of $ab$ but $d$ is not in the shaded area $rabt$, 
$s$ just conducts GPSR. Else $d$ must be in the area $rabt$. In this situation, $s$ wants to consider $a$ or $b$ as its tentative 
target and then writes $a$ or $b$ to the packet's head as a tentative target. In order to make $s$ determine which one  
should be the tentative target, let $m$ be the midpoint of segment $ab$, $mn$ is perpendicular to segment $ab$ and 
$n$ is at the opposite side of $ab$ compared with $s$. Then if $d$ is 
located in area $ramn$, $s$ writes $a$ to the packet's head as its tentative target. If $d$ is located in area $nmbt$, 
$s$ writes $b$ to the packet's head 
as its tentative target. When the packet reaches $a$ or $b$, the tentative target will continue  
sending the packet to the destination node $d$.

When a node is forwarding a packet to its next hop, it calls $HDAR\_forwarding()$ described in Fig.~\ref{forwardfig}.

\begin{figure}[hbt]
\baselineskip=10.2pt
{\small
  \noindent\underline{\bf HDAR\_forwarding()} \\
  \text{~~~~}Look at the forwarding packet whether this node has a tentative \\
  \text{~~~~~~~~}target ${\cal T}$ \\
  \text{~~~~}\textbf{if} true \\
  \text{~~~~~~~~}Compare whether this node is ${\cal T}$;\\
  \text{~~~~~~~~}\textbf{if} true\\
  \text{~~~~~~~~~~~~}Remove ${\cal T}$ and forward the packet to next hop with its\\
  \text{~~~~~~~~~~~~~~~~}destination $d$;\\
  \text{~~~~~~~~}\textbf{else} \\
  \text{~~~~~~~~~~~~}Forward the packet to next hop with its destination ${\cal T}$;\\
  \text{~~~~}\textbf{else}\\
  \text{~~~~~~~~}Search its local cache \\
  \text{~~~~~~~~}\textbf{if} an entry $<a,b>$ exists\\
  \text{~~~~~~~~~~~~}\textbf{if} this node and $d$ are at the same side of $ab$\\
  \text{~~~~~~~~~~~~~~~~}Conduct GPSR;\\
  \text{~~~~~~~~~~~~}\textbf{if} this node and $d$ are at opposite sides of $ab$\\
  \text{~~~~~~~~~~~~~~~~}\textbf{if} $d$ is in $ramn$\\
  \text{~~~~~~~~~~~~~~~~~~~~}Write $a$ as tentative target ${\cal T}$ to the packet;\\
  \text{~~~~~~~~~~~~~~~~~~~~}Forward packet to next hop with destination ${\cal T}$;\\
  \text{~~~~~~~~~~~~~~~~}\textbf{if} $d$ is in $nmbt$\\
  \text{~~~~~~~~~~~~~~~~~~~~}Write $b$ as tentative target ${\cal T}$ to the packet;\\
  \text{~~~~~~~~~~~~~~~~~~~~}Forward packet to next hop with destination ${\cal T}$;\\
  \text{~~~~~~~~~~~~~~~~}\textbf{else}\\
  \text{~~~~~~~~~~~~~~~~~~~~}Conduct GPSR;\\
  \text{~~~~~~~~}\textbf{else}\\
  \text{~~~~~~~~~~~~}Conduct GPSR.\\
  
 }

\protect\caption{HDAR Forwarding Algorithm}
\protect\label{forwardfig}
\end{figure}

























 








==> Jianjun_template/figures/HDAR/introduction.tex <==
\section{Introduction}
\label{intro}


Geographic routing is a simple, scalable  and efficient routing strategy in wireless networks. It has been considered as the most promising 
routing scheme in ad-hoc networks. In such a scheme, the location information for nodes is available 
either through GPS or using virtual coordinates~\cite{ex11}. And it is assumed that each node knows its own location 
and the locations of its neighbors. The source node knows the location of the destination node and encapsulates 
it in each data packet. In the basic greedy forwarding approach, a node sends data packets to one of its neighbors 
who is closest to the destination until the packets reach the destination node. This mechanism can minimize the hops 
from the source to the destination. However, there existing a challenge often faced in geographic greedy routing 
is ``local minimum problem", in which the greedy forwarding process is blocked at a node that does not have a closer 
neighbor to the destination, even though there is a path from the source to destination in the network. The occurrence 
of hole can be caused by many factors in wireless ad hoc networks, such  as the jamming hole incurred by 
jam communication, the sparse deployment, the physical obstacles and power exhaustion~\cite{ex24}.

To overcome the local minimum issue, Greedy Perimeter Stateless Routing (GPSR)~\cite{ex13}, Greedy-Face-Greedy(GFG)~\cite{ex28}, 
and Greedy-Other-Adaptive-Face Routing(GOAFR)~\cite{ex29} are proposed. When a forwarding packet gets stuck at a local 
minimum node, it will start a perimeter routing phase where the packet will be forwarded along the perimeter 
of the hole,  until it reaches a node that can find one of its neighbors that is closer to the destination than 
itself. After that,the forwarding mode returns to greedy. The face routing family schemes can guarantee 
delivery. However,they often cause long detour path in the perimeter routing, although the shorter path exists.

To avoid the long detour path, recent work tries to detect the hole and the nodes located on the hole's boundary 
in advance, then these nodes advertise the hole information to some other nodes~\cite{ex22}~\cite{ex30}. 
So the future routing path can be adaptive in the presence of the hole. 

Our algorithms HDAR in this paper focus on defining and detecting holes in ad hoc network, representing holes and building routes around the holes. The contributions of this paper are threefold.
First, we come up with a heuristic algorithm to detect a hole quickly and easily.
% The hole can be detected in advance. 
And the hole can be identified only by one time calculation. 
%Our hole detecting algorithm results low false negative and low false positive. 
Second, we provide a very concise format to represent the hole. A hole is represented only by a segment.
Third, we develop an approach to make part of the nodes located on the hole's boundary announce to the nodes 
in the vicinity of the hole. 
We found the best tradeoff between the cost of hole information announcement and benefit for future routing. 
Simulation shows that compared with GPSR, HDAR reduces the length of routing path
by 12.4\% and forwarding hops by 13.2\% for all the paths in
tested areas. And the length of long detour paths around the hole can be reduced 61.2\%. 
%only
%38.8\% long and 35.4\% 
The number of hops can be reduced 64.6\% compared with GPSR. Simulation also indicates that the computational complexity of HDAR 
is only 16.6\% that of HAGR.

The rest of the paper is organized as follows. Section~\ref{related}
discusses related work. Section~\ref{Algorithms} proposes a novel method
for detecting holes and presents a new adaptive routing algorithm. We evaluate the
proposed schemes by simulations and describe the performance results in Section~\ref{evaluation}. 
Section~\ref{discussion} further discusses the hole detection and related methods. Section~\ref{conclusion} concludes the paper.
The deduction of the hole announcement size is introduced in the appendix.






==> Jianjun_template/figures/HDAR/maincontents.tex <==
\input{introduction.tex}
\input{overview.tex}
% \input{shadedarea.tex}
% \input{algorithm.tex}
\input{hdar.tex}
\input{simulation.tex}
\input{discussion.tex}
\input{conclusion.tex}
%\input{appendix.tex}


==> Jianjun_template/figures/HDAR/overview.tex <==
\section{Related Work}
\label{related}



The first geographic routing protocol is based on simple greedy forwarding. In this approach, 
each node forwards packets to one of its neighbors who is closest to the destination node until 
the packets arrive the destination. This scheme is efficient. However, it fails due to the ``local minimum problem".

To mitigate ``local minimum problem", compass routing~\cite{ex16} was proposed as the first face routing, 
in which the packet is forwarded along the face until greedy is workable in a node. However, 
compass routing cannot guarantee packet delivery in all geographic networks. Several routing 
algorithms in face routing family have been developed. By combining greedy and face routing, Karp and Kung proposed the
Greedy Perimeter Stateless Routing (GPSR) algorithm~\cite{ex13}.
It consists of the greedy forwarding mode and the perimeter forwarding mode, which is applied in the regions where
the greedy forwarding does not work. An enhanced algorithm, called Adaptive Face Routing (AFR), uses an eclipse
to restrict the search area during routing so that in the worst
case, the total routing cost is no worse than a constant factor
of the cost for the optimal route~\cite{ex17}. The latest addition to
the face routing family is Path Vector Face Routing(GPVFR)~\cite{ex18}, which improves
routing efficiency by exploiting local face information.
The protocols in face routing family can avoid the hole. However, they often cause long detour path.


A new idea was proposed recently, which is to detect the hole in advance, then the nodes located 
on the hole advertise the hole information to other nodes. The hole information will benefit nodes who receive it for their future routing. 
Qing gave 
a mathematical definition of hole~\cite{ex22}. He defined a hole to be a simple region enclosed by a polygon 
cycle which contains all the nodes where local minimum can appear. He brought forth the ``get stuck" concept and 
proposed the hole detection mechanism that
once a packet  following geographic greedy forwarding gets stuck at a node, the node must be on the boundary of a hole.
%Based on his hole definition, 
%when a packet gets stuck at a node following geographic greedy forwarding, this node must be 
%a stuck node 
%on the boundary of a hole. By marking all the boundaries of holes, the routes to get 
%stuck packets out of the local minimum can be found.  The stuck node can simply forward the packet 
%to one of its neighbors that shares the same boundary. 
Also related is HAGR~\cite{ex30}. HAGR investigated the 
nodes incident to a close loop in a geographical graph. For a vertex $u$, if the 
angle between two adjacent edges with respect to this vertex is larger than an angle threshold, 
then vertex $u$ considers it is located on a potential hole. To further determine if it is located on a hole, 
$u$ calculates the diameter of the loop. It locates the bisector that equally splits the angle and uses 
it as a reference line. Then node $u$ finds out the leftmost node and the rightmost node furthest from the 
bisector. The distance between the leftmost node and the rightmost node is the diameter of the hole. 
If the diameter is greater than the diameter threshold and the angle is bigger than the angle threshold, 
$u$ is regarded as sitting on a hole. Once a node is detected on  a hole, it advertises the hole information 
to its neighbors. Upon receiving the hole information, its neighbor recalculates the angle and diameter 
based on its location. If both of them are bigger than their thresholds, then the neighbor considers it is 
on a hole and it continues to advertises the hole information, otherwise it stops advertisement. 
Base on the hole detecting, HAGR divides the network plane into three regions, and the nodes in different 
regions conduct different forwarding strategies. The idea of HAGR is novel. However, the hole detecting 
approach is time-consuming since a node has to calculate the values of two metrics. And the hole advertisement is 
expensive because once a node receives the hole information, it has to recalculate two values and 
compare them with their corresponding thresholds. In addition,  the diameter threshold is an absolute value and it has to be adjusted according to 
the nodes' transmission range or the network deployment, otherwise false negative or false positive may occur.  
Moreover, the forwarding strategies are too complicated.







==> Jianjun_template/figures/HDAR/shadedarea.tex <==
\section{Shaded Area Detection}
\label{shadedarea}
In this section, we describe our method to detect and calculate the shaded areas. We assume that all the ad hoc nodes are distributed 
in a two dimension plane. Every node has the same transmission range. All the nodes are static. 
That is, mobility is not considered.

\subsection{Problem overview}


Fig.~\ref{fig1} indicates two examples of greedy path and detour path caused by a hole. Suppose node $S$ is the source node 
and $D_1$ and $D_2$ are two destination nodes respectively. 
When $S$ intends to send packets to $D_1$, it can find an efficient path by greedy forwarding. 




However, void areas(or holes) may exist in the network plane. A void area is an
area that has no active nodes. A routing path based on
geolocations may be blocked from moving closer to the destination due to the lack of relaying nodes to cross the void.
 In wireless 
ad hoc network, the holes are caused by various reasons~\cite{ex24}. 
For instance, the malicious nodes can jam
the communication to form Jamming Holes or they can
overwhelm regions  by denial of service attacks that cause Black Holes or Worm Holes.
In addition, if the nodes' signal is not long enough to cover everywhere in the network plane, the
Coverage Holes may exist. Moreover, there are Routing Holes. These holes
can be formed either due to voids in nodes deployment or because of failure of nodes due to various reasons such as 
malfunctioning, battery depletion or structure collapse physically destroying the nodes.
When greedy forwarding encounters a hole, it will not be available. For instance, when $S$ intends to send packets to $D_2$, it begins to use greedy forwarding 
mode. When the packets reach node $P$, $P$ is closer to $D_2$ than any of its neighbors but $P$ cannot reach $D_2$ by 
greedy forwarding. 
We say $P$ is a local minimal node. If $P$ changes the forwarding mode to perimeter, the packets will be forwarded along a 
long detour path until the packets arrive B, where the forwarding mode is changed to greedy. The reason that the path is 
detour is that $D_2$ is shaded by the hole but the source doesn't know it. So 
we would like to find the shaded area $T$ in advance and inform this district to $S$. Then $S$ could send the packets 
to the tentative target node $B$ directly if it wants to send packets to $D_2$ in $T$. And then node $B$ relays the packets 
to $D_2$ by greedy forwarding. So the main approach in this paper is that when a source node S sends packets to a destination node, if there is a hole that blocks
the routing path, the source calculates the destination area that is shaded by the hole, then saves the local minimal node
 and a key intermediate node from which the forwarding mode comes back to greedy to its cache. 
 When packets are forwarded via S to any nodes located in the shaded area in the future, S will forward them
to the key intermediate node as tentative target by greedy mode, and then the intermediate node relays to next intermediate node or 
destination node by greedy mode
until the packets arrive the destination. The long detour path can be avoided by this way.

\begin{figure}[!htp]
\begin{center}
\includegraphics[width=6.0cm]{figure1.eps}
\end{center}
\caption{Greedy path and detour path}
\label{fig1}
\end{figure}

There are two problems: one is how to figure out the shaded areas, another is how to find the tentative target nodes?

\subsection{Shaded areas}

%$Definition$: Landmark\\*
We call a node landmark as the following description: Suppose $S$ is a source node and $D$ is a destination node. $S$ is sending packets to $D$ by greedy mode or face mode. 
The packets are forwarded by greedy mode from $S$. Suppose there is a hole $M$ and the packets arrive a local minimal node $P$. 
Then the packets are forwarded by face mode along  the perimeter of $M$. If
there is a node $B$ satisfies: from $B$ to $D$, 
the packets are forwarded only by greedy mode and before B the forwarding mode is perimeter, then we call node $B$ the landmark node from $S$ to $D$.
The landmark looks like the point where the packets escape from the hole's restriction and come back to greedy mode.

The locations of 
the local minimal node $P$ and landmark $B$ must be learned by the source node $S$ to calculate the shaded area. We use three nodes $S$,$B$
and $P$ to represent a shaded destination area. These three nodes indicate the area semi-enclosed by ray $SB$, ray $SP$ and the hole's
perimeter from $B$ to point $F$ which is line $SP$ and the hole's intersection(Fig.~\ref{fig2}).

We add additional fields to a packet's header to let source node S learn $P$ and $B$ when
S sends packets to $D$ in case there is a hole that causes a detour path.
%If the source can learn about that the destination is shaded in case it's hidden behind a hole, the routing path will be shorter since 
%the source would send packets to the landmark. 
Nodes $S$,$D$ and $B${'}$s$ relative locations may vary depending on different hole shapes. So the steps to calculate the 
destination area are slightly different based on their relative locations. 
Basically, there are three types of hole's shapes that may affect how the source calculates the shaded destination areas. 
We distinguish the three types from two aspects, one is the quantitative relationship between  $\angle$ $BDS$ and $\frac{\pi}{2}$, 
another is  whether there is a greedy path from the source to the landmark. 

The first type of hole's shape is as Fig.~\ref{fig2}, where  $\angle$ $BDS$  is less than $\frac{\pi}{2}$ and there is a greedy path  
from $S$ to $B$. The method to find the shaded destination area is straightforward: 
$S$ logically connects $S$ and $P$, suppose $SP$ intersects the hole $M$ at two points and the one other than $P$ is $F$. 
Ray $SF$ extends to an arbitrary point $C$. 
$S$ logically connects $S$ and $B$. Suppose ray $SB$ extends to an arbitrary point $E$.
%Draw line $BE$ in parallel with line $SD$. 
Then the area semi-enclosed by $EB$, the perimeter of $M$ from $B$ to $F$ and $FC$ is the      
shaded destination area $T$. Hence, 
if $S$ wants to send packets to any destination node in $T$, the destination  is hidden behind the hole. To avoid a detour 
path, $S$ sends the packets to $B$ first, and $B$ will then relay them to $D$. Both of the two paths are greedy paths. 


\begin{figure}[!htp]
\begin{center}
\includegraphics[width=8.0cm]{figure2.eps}
\end{center}
\caption{The shaded area when angle BDS is less than $\frac{\pi}{2}$ and path SB is greedy}
%\caption{$\angle $BDS$ \leq$ $\frac{\pi}{2}$ }
%\caption{The shaded area $\frac{\pi}{2}$ }
\label{fig2}
\end{figure}

In scenario 2(Fig.~\ref{fig3}), $\angle$ $BDS$ is less than $\frac{\pi}{2}$.
% while $\angle$ $BSD$ may be greater or than $\frac{\pi}{2}$.
From $S$ to $B$, 
there's no greedy path exists. The steps to find the shaded destination area is the same as scenario one. However, 
to find a routing path in this  circumstance  is different from situation 1. We will discuss it later in this paper.

\begin{figure}[!htp]
\begin{center}
\includegraphics[width=8.0cm]{figure3.eps}
\end{center}
\caption{The shaded area when angle BDS is less than $\frac{\pi}{2}$ and path SB is not greedy}
\label{fig3}
\end{figure}

$\angle$ $BDS$ is greater than $\frac{\pi}{2}$ and there's no greedy path from $S$ to $B$ in the third scenario(Fig.~\ref{fig4})..   
To find the shaded destination areas, $B$ is considered as a tentative destination node, when packets are sent from $S$ to $B$, 
we find another landmark recursively, then we count this landmark as a tentative destination node, and continue to  find landmarks recursively 
until no
 landmark exists. Suppose the last landmark is $B^{'}$, $S$ connects $B^{'}$ and extends it to an arbitrary point $E$.
 Then the area semi-enclosed by $EB^{'}$ , the perimeter of $M$ from $B^{'}$  to $F$ and $FC$  is the shaded destination area $T$.
 %(exclusive $B^{'}$).
 
 
 \begin{figure}[!htp]
\begin{center}
\includegraphics[width=8.0cm]{figure4.eps}
\end{center}
\caption{The shaded area when angle BDS is greater than $\frac{\pi}{2}$ and path SB is not greedy}
\label{fig4}
\end{figure}
 
\begin{comment}
 The steps to find the shaded areas are described in algorithm 1.
In this algorithm, line 5 to line 7 indicates the scenarios of Fig.~\ref{fig2} and Fig.~\ref{fig3}. And line 8 to line 15
illustrates the circumstance in Fig.~\ref{fig4}. This algorithm illustrates the primary method
 to figure out a shaded destination area.  However, a node may generate multiple $<$ $shaded\_des\_area$, $landmark$ $>$
 entries which may share areas or landmarks. We will merge them to reduce spaces and provide efficient lookup. 
 So $BE$ or  $FC$ may not be the boundary line of a shaded area associated with landmark $B$ after the merge. 
 This will be discussed later in this paper.
\end{comment} 
 
Shaded Area Calculation Algorithm in Fig.~\ref{algfig}.
describes how the current node S calculates the shaded area in case there is a hole blocking packets forwarding.
Suppose the lanbdmark node is B. If $\angle$ $BDS$ is less than $\frac{\pi}{2}$, we extend line SB and line SP to E and C
respectively(Fig.~\ref{fig2}), then the area enclosed by EB, the hole perimeter from E to F and FC is shaded area.
However, S does not know the hole's concrete location, so we extend this theoretical area to EBPC as the shaded area since no active nodes in the hole.
If $\angle$ $BDS$ is greater than $\frac{\pi}{2}$, that means we have to recursively find the landmark which is nearest to the source and then
figure out the shaded area(Fig.~\ref{fig4}).This algorithm illustrates the primary method
 to figure out a shaded destination area.  However, a node may generate multiple $<$ $shaded\_des\_area$, $landmark$ $>$
 entries which may share areas or landmarks. We will merge them to reduce spaces and provide efficient lookup. 
 So $BE$ or  $FC$ may not be the boundary line of a shaded area associated with landmark $B$ after the merge. 
 This will be discussed later in this paper.
 \\
 

 


%oribigal algorithm, looks like a global one.
\begin{comment}
\begin{algorithm}[bt]
\begin{algorithmic}[1]
\caption{{\em  Shaded Destination Area}}
\label{algorithm1}
\STATE Logically connects $S$ and $P$. suppose $SP$ intersects the hole $M$ at two points, the one other than $P$ is $F$. $SF$
extends to an arbitrary point $C$.
\STATE $S$ sends packets to $D$ by greedy or face mode 
\IF{there is a landmark node $B$ in the routing path}
\STATE{$D$ informs  $B${'}$s$ location to $S$}
\IF{$\angle $BDS$ \leq$ $\frac{\pi}{2}$ }
\STATE{Connect $SB$ and extends it to $E$}
\STATE{the area semi-enclosed by $EB$, the perimeter of $M$ from $B$ to $F$ and $FC$ is the shaded destination area $T$}
\ELSE 
\STATE{$D^{'} \leftarrow B$}
\STATE{$D^{'}$ informs $S$ to send packets to $D^{'}$}
\WHILE{a landmark node $B^{'}$  from S to $D^{'}$  exists}
\STATE{$D^{'} \leftarrow B^{'}$}
\STATE{$D^{'}$ informs $S$ to send packets to $D^{'}$}
\ENDWHILE
\STATE{Connect $SB^{'}$ and extends it to $E$}
\STATE{the area semi-enclosed by $EB^{'}$, the perimeter of $M$ from $B^{'}$ to $F$ and $FC$ is the shaded destination area $T$}
\ENDIF
\ENDIF
\end{algorithmic}
\end{algorithm}
\end{comment}


\begin{figure}[hbt]
\baselineskip=10.2pt

{\scriptsize
  \noindent\underline{\bf S initiates sending a packet to destination node} \\
  \text{~~~~}S forwards the packet by greedy or face mode; \\
  %\text{~~~~~~~~}hdjshdjhd\\
  \\
  
  \noindent\underline{\bf When the destination node receives the data packet from S} \\
  \text{~~~~}Ckecks the packet's header; \\
  \text{~~~~}\textbf{if} local minimal P and landmark B exists \\
  \text{~~~~~~~~}Sends a $landmark\_exist\_msg$ to S containing the locations of B and P;\\ 
  \text{~~~~}\textbf{else}
  \text{~~~~}Sends ACK to S;
  \\
  
  \noindent\underline{\bf When S receives $landmark\_exist\_msg$} \\
  \text{~~~~}Marks the message sender as node D; \\
  \text{~~~~}\textbf{if} it doesn't save any local minimal node \\
  \text{~~~~~~~~}Saves P;\\
  \text{~~~~}Compares $\angle$ $BDS$ and $\frac{\pi}{2}$; \\
  \text{~~~~}\textbf{if} $\angle $BDS$ \leq$ $\frac{\pi}{2}$ \\
  \text{~~~~~~~~}Extends line SB to any point E;\\
  \text{~~~~~~~~}Extends line SP to any point C;\\
  \text{~~~~~~~~}Consider EBPC as shaded area;\\
  \text{~~~~}\textbf{else}\\
  \text{~~~~~~~~}Counts B as the packet's destination node in its header;\\
  \text{~~~~~~~~}Sends the data packet according to its destination in its header;\\
    
  
}

\protect\caption{Shaded Area Calculation Algorithm}
\protect\label{algfig}
\end{figure}


\begin{comment}
--When S initiates to send a data packet to destination node extracted from the packet's header
       S forwards the packet by greedy or face mode
       
--When the destination node receives the data packet from S
       Ckecks the packet's header
       \textbf{if} landmark B exists(P must exist)
            Sends a landmark_exist_msg to S containing B's location and P's location
       \textbf{else} sends ACK to S
                     
            
--When S receives landmark_exist_msg                  
       Marks the message sender as node D
       Compares \angle BDS and pi/2
          \textbf{if} <=pi/2
               Extends line SB to any point E
               Extends line SP to any point C
               Considers EBPC as shaded area
          \textbf{else}
               Counts B as the packet's destination node in its header
               Sends the data packet according to its destination in its header
               
    
              
          
\end{comment}

 


















==> Jianjun_template/figures/HDAR/simulation.tex <==
\section{Performance Evaluation}
\label{evaluation}



Our simulations were performed by using the easim3D wireless network simulator~\cite{ex27}, 
which is to simulate IEEE 802.11 radios and typically for location based routing algorithms. We
use a noiseless immobile radio network environment. In the
simulations, nodes with a transmission radius of 20 meters
are deployed in an interest area of 400mX400m.


\begin{comment}
%The first part is to compare the computational 
%complexity of HARG and our algorithm HDAR. 
\end{comment}
We generated networks with the number of nodes varied 
from 50 to 300. For a certain number, 50 networks were generated randomly. And the 
holes were generated automatically in each network. 

Our experiments include two parts. 
The first part is to compare GPSR and HDAR.
\begin{comment}
For each network, we first 
implemented HARG. Since HARG has not been simulated yet in the paper~\cite{ex30}, 
we select $5\pi/6$ as the hole detection threshold and 60 meters as the diameter threshold. 
In both HARG and HDAR, we investigated the number of computation times of hole detection. 
In HDAR, the hole information is only calculated by a few nodes located on the hole and other 
nodes are advertised the hole. While in HARG, a number of nodes have to calculate to determine 
the existing of a hole. The numbers of calculation times were reported to evaluate the computational complexity. 
Fig.~\ref{complexityfig} illustrates that the computational complexity of HDAR is much less than that of HARG.
\begin{figure}
\begin{center}
\includegraphics[width=7.0cm]{comtimes.eps}
\end{center}
\vspace{-0.1in}
\caption{The computational complexity.}
\label{complexityfig}
\end{figure}
\end{comment}
%We compare HDAR and GPSR in the second part of our experimentation. 
We implemented GPSR that is 
previously implemented by Karp and Kung~\cite{ex13}. 
%in the same networks generated in part 1. 
We compare GPSR and HDAR by two metrics, the length of routing paths 
and the number of hops.

Fig.~\ref{avepathfig} indicates the average length of paths when the number of nodes changes from 50 to 300.
The average length in HDAR is 12.4\% shorter than that of GPSR.
Fig.~\ref{hopsfig} shows the average number of hops in HDAR is 13.2\% less than that of GPSR.

\begin{figure}
\begin{center}
\includegraphics[width=7.0cm]{avepath.eps}
\end{center}
\vspace{-0.1in}
\caption{The average length of paths.}
\label{avepathfig}
\end{figure}

\begin{figure}
\begin{center}
\includegraphics[width=7.0cm]{avehops.eps}
\end{center}
\vspace{-0.1in}
\caption{The average number of hops.}
\label{hopsfig}
\end{figure}

In the statistics results of  Fig.~\ref{avepathfig} and Fig.~\ref{hopsfig}, the results report both the greedy path and 
the path in the vicinity of holes. So HDAR's effect to the path near the holes cannot be emphasized. To demonstrate HDAR's effect,
we tipically marked the paths that benefit from the hole information as ``hole paths" and recorded the pairs of source and destination nodes.
We also investigated the paths generated by GPSR with the same pairs of source and
destination nodes. Then we compared the paths benefit from hole information in HDAR
with the paths derived from GPSR.
%Then for the same pairs of source and destination nodes, we compare HDAR with GPSR
%still from the length of paths and number of hops perspectives.


The performance of HDAR and GPSR to the hole paths are reported in Fig.~\ref{holepathfig} and  Fig.~\ref{holehopfig}.
HDAR has much shorter paths and fewer hops compared with GPSR.
For the hole path paths, the average length of HDAR is only 38.8\% that of GPSR and the number of hops is only 35.4\%.
The two figures indicate that that HDAR reduces the long detour paths around holes significantly.







\begin{figure}
\begin{center}
\includegraphics[width=7.0cm]{holepath.eps}
\end{center}
\vspace{-0.1in}
\caption{The average length of hole paths.}
\label{holepathfig}
\end{figure}

\begin{figure}
\begin{center}
\includegraphics[width=7.0cm]{holehop.eps}
\end{center}
\vspace{-0.1in}
\caption{The average number of hops of hole paths.}
\label{holehopfig}
\end{figure}




The second part is to compare the computational 
complexity of HARG and our algorithm HDAR. 
We used the same networks in part 1.
% we first implemented HARG. 
Since HARG has not been simulated yet in the paper~\cite{ex30}, 
we selected $5\pi/6$ as the hole detection threshold and 60 meters as the diameter threshold. 
In both HARG and HDAR, we investigated the number of computation times of hole detection. 
In HDAR, the hole information is only calculated by a few nodes located on the hole and other 
nodes are advertised the hole information. While in HARG, a number of nodes have to calculate to determine 
the existing of a hole. The numbers of calculation times were reported to evaluate the computational complexity. 
Fig.~\ref{complexityfig} illustrates that the computational complexity of HDAR is much less than that of HARG.
\begin{figure}
\begin{center}
\includegraphics[width=7.0cm]{comtimes.eps}
\end{center}
\vspace{-0.1in}
\caption{The computational complexity.}
\label{complexityfig}
\end{figure}




















==> Jianjun_template/figures/SFBB/Makefile <==
#---------------------------------------------------------------------------
#  Makefile for latex documents with enhancements to make notes and slides.
#  You must use my macros.tex file if you want to utilize the enhancements.
#     Copyright (c) Jim Griffioen, 1997
#
#  Targets include:
#       init:   type 'make init' before doing anything
#	config:	reset the configuration to "student bw slides"
#       sg:     change the group ownership on RCS files (use after running ci)
#	all:	make the dvi file
#	ps:	make postscript file
#	pdf:	make pdf file
#	html:	make an html version (broken down by subsection)
#       html-nosplit: same as html, but create a single html file
#	bib:	make the bibliography and then .dvi file
#	gv:	make postscript file and ghostview it
#	acro:	make pdf file and acroread it
#	x:	run xdvi on the .dvi file
#	me:	configure for me
#	student: configure for student
#	notes:	configure for notes
#	slides:	configure for slides 
#       bw:	configure for black and white output
#	color:	configure for color output
#	portrait: configure for portrait orientation
#	landscape: configure for landscape orientation
#	2up:	make postscipt with 2 slides per page (plus note area)
#	4up:	make postscipt with 4 slides per page (no note area)
#	webnotes: make tar file with .ps, 2up, 4up, and html for class web page
#	clean:	remove all generated files
#	cleanlatex:  only remove the .dvi, .aux, .bbl, .blg, .log files
#	cleanhtml:  remove the generated html directory
#---------------------------------------------------------------------------

# Define the LaTex file filenames
PAPER=  main

ALLTEXFILES=	${PAPER}.tex \
		maincontents.tex \
		abstract.tex \
		conclusion.tex \
		definition.tex \
		evaluation.tex \
		introduction.tex \
		sfbb.tex \
		overview.tex \
		

# Name of figure files - these must be generated files
# because 'make clean' will delete them.
# Do not include non-generated figs here.
GENERATED_FIGS= 

# Names of xfig files used to generate the above .ps files
# Note, this variable is only used to checkout the xfig files
# from the RCS directory
FIG_FILES= 

# Image files (e.g., GIFs or JPGs) to be used directly in HTML docs
IMAGES=	

# Movie files (e.g., Quicktime, AVI, MPEGS) to be used directly in HTML docs
ANIMS=	

# Name of figure files that are not generated
OTHER_FIGS=	

# Name of the Unix group to set the RCS file ownership to
GROUP= netfac

#---------------------------------------------------------------------------
# You should not need to modify anything below this point
#---------------------------------------------------------------------------

#---------------------------------------------------------------------------
# Makefile code needed by all makefiles
#
# This section assumes that the following makefile variables have already
# been defined above
#    PAPER=
#    ALLTEXFILES=
#    GENERATED_FIGS=
#    FIG_FILES=
#    IMAGES=
#    ANIMS=	
#    OTHER_FIGS=
#    GROUP=
#---------------------------------------------------------------------------

# Set TEXINPUTS to find my tex macrosfiles
TEXINPUTS= .:../macros:../../macros:/homes/griff/lib/macros:

#---------------------------------------------------------------------------
# Define the names of the programs to use
#---------------------------------------------------------------------------

# Programs
GRAP=		grap
TPIC=		tpic
FIG2PS=		fig2dev -Lps -m 0.7
FIG2PIC=	fig2dev -Ltpic -m 0.7
LATEX=		latex
BIBTEX=		bibtex
DVI_TO_PS=	dvips -Pdownload35 -t letter
TBL=		tbl
XDVI=		xdvi
RM=		rm
GREP=		grep
GS=		gv
PDFVIEWER=	acroread
LPR=		lpr
CONVERT=	convert
L2H=		latex2html
PS2PDF=		ps2pdf -dPDFSETTINGS=/printer -dCompatibilityLevel=1.3 -dMaxSubsetPct=100 -dSubsetFonts=true -dEmbedAllFonts=true


# name of the config file - defined in macros.tex
CONFIGFILE= config.tex

# name of the latex2html init file
LATEX2HTML_INIT= /homes/griff/.latex2html_init

# printer to use
PRINTER= lp
PRINTER_OPT= -P${PRINTER}


#---------------------------------------------------------------------------
# Rules for Making
#---------------------------------------------------------------------------
.SUFFIXES: .tex .dvi .fig .ps .detex .g .tbl .pic .gif .jpg .bmp .tif .tiff .tex,v .fig,v .pdf
.tex.detex: 	; $(DETEX) $*.tex > $*.detex
.tex.dvi: 	; $(LATEX) $* 
.fig.pic:	; $(FIG2PIC) -Ltpic $<  |  $(GREP) -v ".baseline" > $*.pic
.fig.ps:	; $(FIG2PS) -Lps $< $*.ps
.gif.ps:	; $(CONVERT) $*.gif $*.ps
.jpg.ps:	; $(CONVERT) $*.jpg $*.ps
.bmp.ps:	; $(CONVERT) $*.bmp $*.ps
.tif.ps:	; $(CONVERT) $*.tif $*.ps
.tiff.ps:	; $(CONVERT) $*.tiff $*.ps
.pic.tex:	; $(TPIC) $*.pic > $*.tex
.g.pic:		; $(GRAP) $*.g | $(GREP) -v ".lf" > $*.pic
.g.tex:		; $(GRAP) $*.g | $(GREP) -v ".lf" > $*.pic ; $(TPIC) $*.pic
.tbl.pic:	; $(TBL) $*.tbl > $*.pic
.dvi.ps:	; $(DVI_TO_PS) -o $*.ps $*.dvi 
.ps.pdf:	; $(PS2PDF) $*.ps $*.pdf
.tex,v.tex:	; co $*.tex
.fig,v.fig:	; co $*.fig
.jpg,v.jpg:	; co $*.jpg
.gif,v.gif:	; co $*.gif
.bmp,v.bmp:	; co $*.bmp
.tiff,v.tiff:	; co $*.tiff
.tif,v.tif:	; co $*.tif

# Different Make options

all: ${PAPER}.dvi ${PAPER}.ps

${PAPER}.dvi: ${ALLTEXFILES} ${FIG_FILES} ${IMAGES} ${ANIMS} ${GENERATED_FIGS}
	$(LATEX) ${PAPER}

setgrp: 
	chgrp $(GROUP) RCS/*
sg: 
	chgrp $(GROUP) RCS/*

generated_figs: ${GENERATED_FIGS}

print: ${PAPER}.dvi

ps: ${PAPER}.ps

pdf: ${PAPER}.pdf

${PAPER}.ps: ${PAPER}.dvi

${PAPER}.pdf: ${PAPER}.ps

x: ${PAPER}.dvi
	$(XDVI) ${PAPER}.dvi &

gv: ps
	$(GS) ${PAPER}.ps &

gs: ps
	$(GS) ${PAPER}.ps &

acro: pdf
	$(PDFVIEWER) ${PAPER}.pdf &

bib: ${ALLTEXFILES} ${PAPER}.ps
	echo "#!/bin/sh" > .makbib
	echo $(LATEX) ${PAPER} >> .makbib
	echo $(BIBTEX) ${PAPER} >> .makbib
	echo $(LATEX) ${PAPER} >> .makbib
	echo $(LATEX) ${PAPER} >> .makbib
	chmod a+x .makbib
	./.makbib
	rm .makbib

me:
	cat $(CONFIGFILE) | sed "s/studenttrue/studentfalse/" > .tmp
	cp .tmp $(CONFIGFILE); rm .tmp
	cat $(CONFIGFILE) | sed "s/instructorfalse/instructortrue/" > .tmp
	cp .tmp $(CONFIGFILE); rm .tmp
instructor:
	cat $(CONFIGFILE) | sed "s/studenttrue/studentfalse/" > .tmp
	cp .tmp $(CONFIGFILE); rm .tmp
	cat $(CONFIGFILE) | sed "s/instructorfalse/instructortrue/" > .tmp
	cp .tmp $(CONFIGFILE); rm .tmp
student:
	cat $(CONFIGFILE) | sed "s/studentfalse/studenttrue/" > .tmp
	cp .tmp $(CONFIGFILE); rm .tmp
	cat $(CONFIGFILE) | sed "s/instructortrue/instructorfalse/" > .tmp
	cp .tmp $(CONFIGFILE); rm .tmp
slides:
	cat $(CONFIGFILE) | sed "s/slidesfalse/slidestrue/" > .tmp
	cp .tmp $(CONFIGFILE); rm .tmp
	cat $(CONFIGFILE) | sed "s/notestrue/notesfalse/" > .tmp
	cp .tmp $(CONFIGFILE); rm .tmp
notes:
	cat $(CONFIGFILE) | sed "s/slidestrue/slidesfalse/" > .tmp
	cp .tmp $(CONFIGFILE); rm .tmp
	cat $(CONFIGFILE) | sed "s/notesfalse/notestrue/" > .tmp
	cp .tmp $(CONFIGFILE); rm .tmp
color:
	cat $(CONFIGFILE) | sed "s/wantcolorfalse/wantcolortrue/" > .tmp
	cp .tmp $(CONFIGFILE); rm .tmp
bw:
	cat $(CONFIGFILE) | sed "s/wantcolortrue/wantcolorfalse/" > .tmp
	cp .tmp $(CONFIGFILE); rm .tmp
portrait:
	cat $(CONFIGFILE) | sed "s/landscapetrue/landscapefalse/" > .tmp
	cp .tmp $(CONFIGFILE); rm .tmp
landscape:
	cat $(CONFIGFILE) | sed "s/landscapefalse/landscapetrue/" > .tmp
	cp .tmp $(CONFIGFILE); rm .tmp
init:	config
config:
	/bin/echo '\\slidestrue' > $(CONFIGFILE)
	/bin/echo '\\notesfalse' >> $(CONFIGFILE)
	/bin/echo '\\instructorfalse' >> $(CONFIGFILE)
	/bin/echo '\\studenttrue' >> $(CONFIGFILE)
	/bin/echo '\\wantcolortrue' >> $(CONFIGFILE)
	/bin/echo '\\landscapefalse' >> $(CONFIGFILE)

html-split: $(PAPER).dvi
	$(L2H) -split 8 -bottom_navigation -info "" -local_icons \
	-init_file $(LATEX2HTML_INIT) $(PAPER).tex
	@echo copying $(IMAGES) $(ANIMS) into the $(PAPER) directory
	cp $(IMAGES) $(ANIMS) $(PAPER)

html: $(PAPER).dvi
	$(L2H) -split 0 -no_navigation -info "" -local_icons \
	-init_file $(LATEX2HTML_INIT) $(PAPER).tex
	@echo copying $(IMAGES) $(ANIMS) into the $(PAPER) directory
	cp $(IMAGES) $(ANIMS) $(PAPER)

html-nosplit: $(PAPER).dvi
	$(L2H) -split 0 -no_navigation -info "" -local_icons \
	-init_file $(LATEX2HTML_INIT) $(PAPER).tex
	@echo copying $(IMAGES) $(ANIMS) into the $(PAPER) directory
	cp $(IMAGES) $(ANIMS) $(PAPER)

html-noimages: $(PAPER).dvi
	$(L2H) -split 0 -no_images -no_navigation -info "" $(PAPER).tex
	@echo copying $(IMAGES) $(ANIMS) into the $(PAPER) directory
	cp $(IMAGES) $(ANIMS) $(PAPER)

htmlln:
	ln -s /homes/griff/lib/macros/html.sty.foremergencies html.sty

2up: ps
	2up -p${PAPER}-2pp.ps ${PAPER}.ps

4up: ps
	mpage -P -4 ${PAPER}.ps > ${PAPER}-4pp.ps

webnotes: 2up 4up html tar

tar:
	tar -vcf - ${PAPER}.ps ${PAPER}-2pp.ps ${PAPER}-4pp.ps ${PAPER} \
	| gzip > webnotes.tgz

clean: cleanlatex cleanfigs cleanps cleanhtml cleanpdf

cleanlatex:
	$(RM) -f *.aux *.bbl *.blg *.log *.dvi

cleanhtml:
	$(RM) -rf ${PAPER}

cleanfigs:
	$(RM) -f ${GENERATED_FIGS}

cleanps:
	$(RM) -f ${PAPER}.ps

cleanpdf:
	$(RM) -f ${PAPER}.pdf

ppp5:
	rsh ppp5 rm pap.ps pap.ps.gz
	cat ${PAPER}.ps | gzip > pap.ps.gz
	rcp pap.ps.gz ppp5:
	rsh ppp5 gunzip pap.ps.gz
	rm pap.ps.gz

ppp6:
	rsh ppp6 rm pap.ps pap.ps.gz
	cat ${PAPER}.ps | gzip > pap.ps.gz
	rcp pap.ps.gz ppp6:
	rsh ppp6 gunzip pap.ps.gz
	rm pap.ps.gz

ppp9:
	rsh 204.198.76.89 rm pap.ps pap.ps.gz
	cat ${PAPER}.ps | gzip > pap.ps.gz
	rcp pap.ps.gz 204.198.76.89:
	rsh 204.198.76.89 gunzip pap.ps.gz
	rm pap.ps.gz



==> Jianjun_template/figures/SFBB/conclusion.tex <==
\section{Conclusion}
\label{conclusion}

In this paper, we presented a new message broadcasting algorithm for vehicular networks.
In this algorithm, a message sender can select the best node among its neighbors that
re-broadcast the message fastest to other nodes. 
% The novelty of the approach is that each 
Each node only
keeps values of two parameters to record its moving trend. 
Together with the current velocity of each node, we can determine which node is the best candidate.
% Then the moving trend is used to select the best re-broadcasting node.
The simulations demonstrate that our approach can improve 
the delivery ratio and decrease the end-to-end delay over traditional farthest distance based algorithms.


==> Jianjun_template/figures/SFBB/definition.tex <==
\newcommand{\bibdir}{./}

\newcommand{\msgrange}{potential range}
\newcommand{\msgranges}{\msgrange s}
\newcommand{\closestneighbors}{$m$-width neighborhood}

\newcommand{\newunstruct}{new unstructured}



==> Jianjun_template/figures/SFBB/introduction.tex <==
\section{Introduction}
\label{intro}

Recent advances in wireless technologies have made Inter-Vehicle Communications possible 
in mobile Ad-Hoc networks (MANET), thus generating a new type of mobile network known as
Vehicular Ad-Hoc Network (VANET)~\cite{ex14}~\cite{ex24}. VANET has attracted considerable attentions from both the research community and the automotive industry. Many automobile manufacturers have started
planning to build communication devices into their vehicles for purposes of security, convenience and comfort. 
%In addition, the increasing importance of VANET has been recognized
%by the governmental organizations. The Federal Communications Commission (FCC) has allocated particular spectrum for Inter-Vehicle Communications.
With the development of VANETs, many attractive applications have emerged. 
On-board active systems can assist the drivers in avoiding collisions~\cite{ex16}. 
Safety systems can intelligently
disseminate road information~\cite{ex22}~\cite{ex25}, such as accidents, 
real-time traffic congestion, or condition of the road surface. 
Broadcasting schemes can also inform other vehicles of
approaching of police vehicles so that they yield to police vehicles~\cite{ex15}.


Message dissemination is essential in support of the applications of VANET. Researchers are developing broadcasting approaches to disseminate messages to other vehicles. 
The design of effective
vehicular broadcasting approaches poses a number of challenges.  Similar to MANET, VANET has no fixed infrastructure and instead relies on ordinary nodes to perform routing of messages. 
However, VANETs behave in different ways than traditional MANETs. The mobility constraints and high dynamic are unique characteristics of VANETs. 
Velocities are also restricted because of speed limits, traffic control mechanisms such as stop sign and traffic light, and scenarios of the road.
Furthermore, VANETs encounter
a major routing issue, i.e., the broadcast storm problem. The broadcast storm problem
occurs when mobile nodes send messages by flooding, causing frequent link layer contention with other nearby broadcasting
nodes and resulting in packet loss due to collisions.
Therefore, it is extremely difficult to design a sound message broadcasting approach, especially the one  that can
broadcast messages to other vehicles as fast as possible.

Current approaches focus on employing distance-based mechanisms. In these schemes, the sender node tries to select the farthest node in the broadcasting direction and assign it the duty of forwarding messages. 
However, these approaches may not select the best candidate that can forward the message to other nodes fastest.
In this paper, we develop
a statistical filtering based broadcasting algorithm. In this algorithm, each node maintains the acceleration and the variance of acceleration that can represent its historical mobility status. In addition,
each node can predict its future mobility trend by considering the two parameters and its current velocity. In the broadcasting process, the sender disseminates a message to all its neighbors in the broadcasting direction. Then it selects the fastest candidate based on considering its neighbors' future mobility and then designates this candidate to re-broadcast the message.
%The best re-broadcasting node can be selected because the metric to select the best node is the nodes' future mobilities.
Because each node only needs to maintain two parameters,    
the overhead  is low. Our simulation results indicate that  our approach can significantly decrease the end-to-end delay and improve
the message delivery ratio, compared with existing approaches.

The rest of the paper is organized as follows.
Section~\ref{related} discusses the related research on this topic. Section~\ref{sfbb} proposes a novel method to broadcast messages to other vehicles as fast as possible.
We evaluate the proposed schemes by simulations and describe the performance results
in Section~\ref{evaluation}.
Section~\ref{conclusion} concludes the paper.




==> Jianjun_template/figures/SFBB/maincontents.tex <==
\input{introduction.tex}
\input{overview.tex}
% \input{shadedarea.tex}
% \input{algorithm.tex}
\input{sfbb.tex}
\input{simulation.tex}
\input{conclusion.tex}
%\newpage


==> Jianjun_template/figures/SFBB/overview.tex <==
\section{Related Work}
\label{related}

This section reviews the work on the message broadcast protocols of Vehicular Networks.
Unlike other format of MANETs, applications developed for VANET have a very specific and clear goal of providing
an intelligent and safe transport system. Emergency warning for public safety is one of many applications that is
highly time-critical and requires a more intelligent broadcast mechanism than just blind flooding.
In~\cite{ex3}, the authors proposed a spatially aware packet routing algorithm to disseminate the message in VANETs.
This algorithm predicts the permanent topology holes. Then, the geographic forwarding is conducted
when the messages are disseminated to other nodes. This approach guarantees that the message will be broadcast to other nodes.
However, it costs too
much because the void areas need to be detected ahead. In addition, the location may change frequently in the VANET. Thus the scenario at a particular moment
is not the same as other time.

A. Amoroso et al proposed a broadcasting algorithm for VANET called FROV~\cite{ex4}.
% ``The Farther Relay and Oracle for VANET''~\cite {ex4}.
This
algorithm is applied in the scenario that cars have heterogeneous transmission ranges. In addition, the transmission of a car can vary while traveling, due to
changes of environmental conditions, such as the humidity of the air, rain, snow and fog. Moreover, topological conditions, such as tunnels, sharp curves, surrounding trees and
buildings, could further influence transmission ranges. The main idea of FROV is 
that the node selected to re-broadcast a message is the one whose re-transmission range spans further than
other nodes. To accomplish this task, FROV considers both
the position and the transmission range, in the direction of
the broadcast, for all the receivers of a message. This algorithm can handle the scenarios with extreme weather or poor conditions, but it does not
consider the mobility status of the vehicles that is essential in VANETs.

A multi-hop broadcast protocol for inter-vehicle communication was proposed in~\cite{ex5}.
This protocol assigns the duty of
forwarding and acknowledging the broadcast packet to only
one vehicle by dividing the road portion inside the transmission range into segments and choosing the vehicle in the
farthest non-empty segment without apriori topology information. When there is an intersection in the path of the
message dissemination, new directional broadcasts are initiated by the repeaters located at the intersections.
This protocol only considers the longest distance factor when selecting the best re-broadcasting node.

An approach that considers mobilities of vehicles was proposed in~\cite{ex6}. In this algorithm, vehicles are divided into several
clusters. Each cluster header maintains the moving status and density of the vehicles in its cluster.
This approach takes mobility into consideration, but it is very difficult to maintain
clusters in VANETs.

%Towards Efficient Routing in Vehicular Ad Hoc Networks.













==> Jianjun_template/figures/SFBB/sfbb.tex <==
%%%% note:
%   recursion discussed in ITGR routing section, may need a graph
%   combining entries in separate section one graph should be enough
%%%%%

\section{Kalman Filtering Based Broadcasting Protocol}
\label{sfbb}

\subsection{The Basic Idea}
% \subsection{Problem overview}

We start this section with a simple example to illustrate the basic idea of our approach.
% In this section, we describe our method to detect and calculate the shaded areas.
We assume that all the vehicles (nodes) are distributed in a two dimensional space and they are in the moving status.
% Every node has the same transmission range.
Each node has the same transmission range. In addition, errors of measurement for the mobility exist because of
environmental conditions~\cite{ex4}.

\begin{figure}[!htp]
\begin{center}
\includegraphics[width=8.0cm]{car1.eps}
\end{center}
\caption{The basic broadcasting scenario}
\label{fig1}
\end{figure}

Fig.~\ref{fig1} gives an example to show how the sender
$A$ should select one of its neighbors to re-broadcast its message.
After node $A$ broadcasts the message to all of its neighbors in the broadcasting direction,
$A$'s neighbors $C_1$, $C_2$ and $C_3$ receive this message. Node $A$ has to select one of them
to re-broadcast the message.
A simple strategy will let $A$ select the one that is the farthest away from $A$ in the broadcasting direction.
In this case, $A$ will select $C_1$.
However, this may not necessarily be the best choice.

% Let us assume that node $C_1$ is slowing down.

Let us assume that node $C_1$ is moving at a much lower speed than $C_2$ and $C_3$.
Further we assume the historical velocities up to this moment of
node $C_2$ are [..., 50, 55, 59, 63] (miles/hour), and the velocities of node $C_3$ are [..., 75, 71, 66, 64].
Our goal is to select a node that can re-broadcast the message fastest to other nodes.
Considering that $C_2$ and $C_3$ are moving much faster thatn $C_1$, they are obviously
better choices for carrying the message farther down the broadcast direction.
If we only consider the current speed, $A$ should choose $C_3$.
However, we want to select the one that can get out of the transmission range of $A$ and conduct the re-broadcasting first.
This can achieve the goal of the fastest re-broadcast of the message.
We can predict future velocities of these nodes based on their historical and current velocities, and then figure out which node is the first one that will get out of
$A$'s range. In this example, our strategy will let $A$ choose $C_2$.

\begin{comment}
Fig.~\ref{fig1} gives an example in which
$A$ is the message sender. Node $A$ broadcasts the message to all of its neighbors in the broadcasting direction.
$A's$ neighbors $C_1$, $C_2$ and $C_3$ receive this message. Then, $A$ will select one of them to re-broadcast the
messages. If $A$ selects the one that is the farthest away from $A$ in the broadcasting direction, $C_1$ is the option.
Now we assume that node $C_1$ is slowing down.
Considering the scope of coverage of re-broadcast, $C_2$ or $C_3$ are better choices and should be selected.
We assume the historical velocities up to this moment of
node $C_2$ are [...50,55,59,63] (miles/hour), and the velocities of node $C_3$ are [...75,71,66,64]. If we simply select the faster one, $C_3$ is
the choice. However, we want to select the one who can get out of the transmission range of $A$ and then conduct the re-broadcasting first.
We would compute the velocities of these nodes based on their historical and current velocities, and then figure out which one is the first one that will get out of
$A$'s range. In this example, the best choice should be $C_2$.
\end{comment}


\subsection{Kalman Filtering Based Mechanism}
The transmission range of the wireless network for vehicles
is normally 300-400 meters long. It is much longer than the width of the road containing  multiple lanes.
Thus we use a line to represent the road as in Fig.~\ref{fig2}. Here $l$ is a partial arc of the transmission range crossing the road. In addition, point $P$ is the intersection
of $l$ and the road.

\begin{figure}[!htp]
\begin{center}
\includegraphics[width=8.0cm]{car22.eps}
\end{center}
\caption{Simplified basic broadcasting scenario}
\label{fig2}
\end{figure}


We need to compute which node is the first one that can get out of $A$'s range.
The moving trend obviously must be considered.
%The naive method to find the moving trend is to let each node
%save all its history and current velocities, then each node can represent its moving trend by curve-fitting approach that approximates its mobility trend. Apparently, this method costs too much.
We come up with a model based on Kalman Filtering method~\cite{ex10}. In this model, each node only needs to maintain two parameters, its potential acceleration and
variance of acceleration, to represent its mobility trend. Then its future velocity can be computed.
Thus, node $A$ can figure out the best node to be assigned to conduct the re-broadcasting subsequently.


We observe the discrete moving status with every period $\Delta$$t$. Suppose we are investigating the nodes at current time $k$.
Node $A$ would like to find the node that will reach $P$ first and assign it as the re-broadcasting node.
We mark the transmission range of A as $R$, the velocity of node $C_i$ measured at time $k$ as $v_{i_k}$, and
%We would like to compute $c_i$'s potential ability about how fast it can get out of
 %A's range. We estimate $v_{ik+1}$ as $c_i$'s potential ability.
  the distance from A to $C_i$ as $|AC_i|$. Then the time to
reach $P$ is $T_i=(R-|AC_i|)/$$|$$\hat{v_{i_k}}-v_A|$. Here $\hat{v_{i_k}}$ is the predicted velocity of $C_i$ at time $k$.
The prediction is based on considering both $C_i$'s historical and current mobility status. In our approach,
 we predict $C_i$'s velocity for time $k+1$ to compute $T_i$.
 Once we know each $\hat{v_{i_k}}$, we will figure out the node
 with the smallest $T_i$. So the task is to compute $\hat{v_{i_k}}$. % which will be achieved by predicting the velocity of time $k+1$ at time $k$.
%The prediction of its velocity of time $k+1$ is important. For example, if two node $c_1$ and $c_2$ have the history velocities $[50,55,59,63]$
 %and $[76,73,66,63]$ respectively, we predict that $c_1$ will be faster than  $c_2$ at next time by their moving trends.
 %Because the node $c_i$ periodically measures and records its velocity every time slot $\Delta$$t$,

 The naive method of predicting the velocity at time $k+1$ is as follows. Let node $C_i$ save
all its historical and current (time $k$) velocities $v_{i_0}$, $v_{i_1}$, ...,$v_{i_k}$.
Then it can predict its velocity for time $k+1$ by the curve-fitting method that approximates
its moving trend. The problem with this method is that it costs too much. So we devise a model based on stochastic
filtering approach, particularly, Kalman Filtering method. In our model, each node only needs
to maintain values of two parameters, the potential acceleration and the variance of acceleration
at time $k-1$ and measure the status at time $k$.



%We would like to predict the velocity of next time by predicting the acceleration $a$.
We define the following notations to represent the mobility status for node $C_i$ in Table 1. Note that all the notations of
acceleration and velocity are vectors.

\begin{table}[htp]
\caption{Notations for the Mobility Status}
\centering
\begin{tabular}{|c|c|}
%\hline
%\multicolumn{2}{|c|}{Notations for the  Mobility Status} \\
\hline
Notation & Meaning \\\hline
$v_{i_k}$ & The measured velocity at time $k$. \\\hline
$\hat{v_{i_k}}$ & The velocity predicted at time $k$. \\\hline
$a_{i_k}$ & The acceleration measured  at time $k$.\\\hline
$\hat{a_{i_k}^-}$ & The acceleration at time $k$ evolved \\
~~~~ & from time $k-1$.\\\hline
$\hat{a_{i_k}}$ & The potential acceleration at time $k$. \\\hline
 $p_{i_k}$ & The variance of acceleration updated \\
 ~~~~ & at time $k$.\\\hline
  $p_{i_k}^-$ & The variance of acceleration at time $k$ \\
  ~~~~ & evolved from time $k-1$.\\\hline
 $Q$ & The error or noise in the process.\\\hline
  $Kg_{i_k}$ & The blending factor at time $k$.\\
\hline
\end{tabular}
\label{table11}
\end{table}

%begin the additional content for the job talk
\noindent Input: At time $k$, node $C_i$ maintains\\
$v_{i_{k-1}}$, $\hat{a_{i_{k-1}}}$, and $p_{{i_k-1}}$. \\
$C_i$ also measures $v_{i_k}$.\\
Output: $C_i$ outputs its potential \\
%velocity $v_{i_{k+1}}$.\\
acceleration $\hat{a_{i_k}}$.\\
At time $k$, $C_i$  computes $a_{i_k}$.\\
$C_i$ updates $\hat{a_{i_k}^-}$ and $p_{i_k}^-$ in order to keep its historical moving trend to predict its future velocity.\\
$C_i$ also computes the blending factor $Kg_{i_k}$,
which indicates how much the acceleration changes from last time to current time.\\
$C_i$ computes its potential acceleration
$\hat{a_{i_k}}$. This acceleration will be used to predict its velocity for time $k+1$.\\
$C_i$ computes the velocity predicted for time $k+1$.\\
%end the content for the job talk

At time $k$, $C_i$  measures its velocity $v_{i_k}$. And then it computes $a_{i_k}$ as its measured acceleration  by
% $a_{i_k}$=$(v_{i_k}-v_{i_{k-1}})$/$\Delta$$t$ ~~ (1)\\
\[a_{i_k}=(v_{i_k}-v_{i_{k-1}})/\Delta t\]
Node $C_i$ updates $\hat{a_{i_k}^-}$ and $p_{i_k}^-$ in order to keep its historical moving trend to predict its future velocity.
% $\hat{a_{i_k}^-}$=$\hat{a_{i_{k-1}}}$ ~~(2)\\
\[\hat{a_{i_k}^-}=\hat{a_{i_{k-1}}} \]
\[p_{i_k}^-=p_{{i_k-1}}+Q  \]
Node $C_i$ also computes the blending factor $Kg_{i_k}$,
which indicates how much the acceleration changes from last time to current time.\\
\[Kg_{i_k}=p_{i_k}^-(p_{i_k}^-+Q)^{-1}=p_{i_k}^-/(p_{i_k}^-+Q) \]
% $Kg_{i_k}$=$p_{i_k}^-(p_{i_k}^-+Q)^{-1}$=$p_{i_k}^-/(p_{i_k}^-+Q)$ ~~(4)\\
Once $C_i$ obtains the blending factor $Kg_{i_k}$ and the evolved acceleration $\hat{a_{i_k}^-}$, it knows how much the acceleration changes and the
evolved acceleration. Additionally, $C_i$ considers the measured acceleration $a_{i_k}$. Then it computes its potential acceleration
$\hat{a_{i_k}}$. This acceleration will be used to predict its velocity for time $k+1$.
\[\hat{a_{i_k}}=\hat{a_{i_k}^-}+Kg_{i_k}(a_{i_k}-\hat{a_{i_k}^-}) \]
% $\hat{a_{i_k}}$=$\hat{a_{i_k}^-}$+$Kg_{i_k}(a_{i_k}-\hat{a_{i_k}^-})$ ~~(5)\\
$C_i$ updates the variance of acceleration for future utilization.
\[p_{i_k}=(1-Kg_{i_k})p_{i_k}^- \]
% $p_{i_k}$=(1-$Kg_{i_k}$)$p_{i_k}^-$ ~~(6)\\
Finally, the velocity predicted for time $k+1$ is
\[v_{i_{k+1}}=v_{i_k}+\hat{a_{i_k}}\Delta t \]
% $v_{i_{k+1}}=v_{i_k}+\hat{a_{i_k}}\Delta$$t$ ~~(7)\\
In the entire computation process at time $k$, $C_i$ only needs to measure its velocity $v_{i_k}$ and record two parameters
$\hat{a_{i_{k-1}}^-}$ and $p_{i_{k-1}}$. Then it can predict its velocity at time $k+1$ by the calculation.


\begin{comment}


\noindent Note that $\hat{v_{i_k}}$ will be obtained by the prediction of the velocity for time $k+1$.
And $\hat{a_{i_k}}$ will be obtained by the prediction of the acceleration for time $k+1$.\\


 $v_{i_k}$: the measured velocity at time $k$.\\
$\hat{v_{i_k}}$: the potential velocity at time $k$. It will be obtained by the prediction of the velocity for time $k+1$.\\
$a_{i_k}$: the acceleration measured by $(v_{i_k}-v_{i_{k-1}})/\Delta$$t$ at time $k$.\\
$\hat{a_{i_k}^-}$: the acceleration at time $k$ evolved from time $k-1$.\\
$\hat{a_{i_k}}$: the potential acceleration at time $k$. It will be obtained by the prediction of the acceleration for time $k+1$.\\
 $p_{i_k}$: the variance of acceleration updated at time $k$.\\
  $p_{i_k}^-$: the variance of acceleration at time $k$ evolved from time $k-1$.\\
 $Q$: the error or noise in the process.\\
  $Kg_{i_k}$: the blending factor at time $k$.\\


The idea of our approach is: at time $k$, node $c_i$ keeps the potential acceleration $\hat{a_{i_{k-1}}}$ and the variance of acceleration $p_{i_{k-1}}$ of previous time $k-1$, which was
calculated from time $k-2$.
The parameter $\hat{a_{i_{k-1}}}$ represents  $c_i$'s potential acceleration and $p_{i_{k-1}}$ represents how its acceleration changes. So the two parameters represent its moving trend. Then at time $k$, if node $c_i$ wants to predict its potential velocity at time $k+1$, it uses the two parameters of time $k-1$ to compute a
blending factor $Kg_{i_k}$. Further, it predicts its velocity at time $k+1$ by $Kg_{i_k}$ and  $a_{i_k}$.
In order to maintain the knowledge of its moving trend, node $c_i$ conducts the following update of every $\Delta$$t$:\\
$\hat{a_{i_k}^-}$=$\hat{a_{i_{k-1}}}$ ~~(1)\\
$p_{i_k}^-$=$p_{{i_k-1}}$+$Q$ ~~ (2)\\
$c_i$ also conducts the measurement update as follows:\\
$Kg_{i_k}$=$p_{i_k}^-(p_{i_k}^-+Q)^{-1}$=$p_{i_k}^-/(p_{i_k}^-+Q)$ ~~(3)\\
$\hat{a_{i_k}}$=$\hat{a_{i_k}^-}$+$Kg_{i_k}(a_{i_k}-\hat{a_{i_k}^-})$ ~~(4)\\
$e_{i_k}$=$|$$\hat{a_{i_k}^-}$-$\hat{a_{i_k}}$$|$=$|$$\hat{a_{i_{k-1}}}$-$\hat{a_{i_k}}$$|$ ~~(5)\\
%$p_{i_k}=E[e_{i_k}e_{i_k}^T]$ ~~(6)\\
$p_{i_k}$=(1-$Kg_{i_k}$)$p_{i_k}^-$ ~~(6)\\
%$\hat{a}$

\noindent At time $k$, node $c_i$ keeps the velocity $v_{i_{k-1}}$, variance $p_{i_{k-1}}$ and the potential acceleration $\hat{a_{i_{k-1}}^-}$ of time $k-1$.
$c_i$ can measure its velocity $v_{i_k}$ and compute the acceleration $a_{i_k}$ by $(v_{i_k}-v_{i_{k-1}})/\Delta$$t$. So the potential acceleration $\hat{a_{i_k}}$ at time $k$
can be computed by formula (4). Then the potential velocity at time $k+1$ can be achieved
by $v_{i_{k+1}}=v_{i_k}+\hat{a_{i_k}}\Delta$$t$. In this approach, $\hat{a_{i_{k-1}}^-}$ and $p_{i_{k-1}}$ represent  the changes of the moving status. Hence the historical mobility can be kept
only by the two parameters, which illustrate the moving trend of a node.
\end{comment}

The direction of the road may not be parallel or perpendicular
to the coordinate axes. Moreover, a vehicle may suddenly change its moving direction or speed. So we decompose
the velocity into two velocities parallel to the axes of the coordinate plane (Fig.~\ref{fig4})
to take care of the general scenarios.

\begin{figure}[!htp]
\begin{center}
\includegraphics[width=6.0cm]{m1020_4.eps}
\end{center}
\caption{Velocities of X and Y decomposition}
\label{fig4}
\end{figure}

In the general scenario, node $C_i$ computes its velocity $\hat{v_{i_{{k+1}_x}}}$  in  X direction and $\hat{v_{i_{{k+1}_y}}}$  in  Y direction at time $k+1$,
then computes $\hat{v_{i_{k+1}}}$=$\sqrt{ \hat{v_{i_{{k+1}_x}}}^{2}+\hat{v_{i_{{k+1}_y}}}^{2} }$. It further computes $T_i$ by $T_i=(R-|AC_i|)/$$|$$\hat{v_{i_{k+1}}}-v_A|$,
the time that node $C_i$ gets out of the range of $A$. Then $A$ can figure out the desired node $C_i$  with minimal $T_i$.


\begin{comment}


%In the scenario of Fig.~\ref{fig1}, we assume that the  moving direction of the vehicles and message broadcasting direction are identical.
%Moreover, the vehicles in opposite moving direction are not involved in the broadcasting process. In addition to this situation, there are some other scenarios. We list three of them in this paragraph and will discuss all in the Handle\_msg() algorithm.
%In Fig.~\ref{fig5}, from  $A$'s angle, the vehicle moving direction and message broadcasting direction are identical, and the vehicles in other moving direction are nothing to do with the broadcasting process.
In Fig.~\ref{fig5}, from  $A$'s angle, the vehicle moving direction and message broadcasting direction are identical, and the vehicles in both directions need to be
informed of the message. Another instance is
in Fig.~\ref{fig6}, from  $A$'s angle, the vehicle moving direction and message broadcasting direction are opposite, and the vehicles in other moving direction can help forward the broadcasting message, but they do not have to receive the message.
%A real world setting is, node $A$ was advertised a car accident message from $B$, and then $A$ is broadcasting the message to the node  $C$, $D$,...in its same moving direction. Then, $A$ selects one of the nodes from $E$, $F$...in its opposite moving direction to help  deliver  the message.
One more example is that the road is one way. The current broadcasting node can only select a node in its same moving direction to re-broadcast the message regardless whether the re-broadcasting direction is the same or the opposite direction of the mobility.

There are a number of factors that will affect how node $A$ selects the re-broadcasting node, including the type of the road (one way or two ways), the vehicles' moving direction, the message broadcasting direction, the areas of the
message receivers (the nodes in $A$'s same direction or opposite direction). %The combination of these factors will result a large number of scenarios. We only list three examples in this
We divide them into two categories by focusing on the selection of the re-broadcasting node. The first category is that
\end{comment}

From node $A$'s perspective, the moving direction of the vehicles and the message broadcasting direction can be identical or opposite.
When the moving direction and the broadcasting direction are identical (Fig.~\ref{fig5}), node $A$ broadcasts the message to its neighbores, and then selects the re-broadcasting node in the same moving direction based on the formulas
presented above.
% discussed in this paper.
%that can get out of $A$'s range in the same moving direction first. The selection criteria is based on formulas (1)-(7).
When the moving direction and the broadcasting direction are opposite (Fig.~\ref{fig6}),
%(the areas in its same direction, opposite direction or both).
node $A$ broadcasts the message to its neighbores, then it selects the re-broadcasting node from those
in the opposite moving direction that can get out of $A$'s range in the opposite moving direction first.

\begin{comment}
Otherwise, it selects a node (must be in the same moving direction) that can get out of $A$'s range in the opposite moving direction first.
Fig.~\ref{fig13} shows this scenario. In the one way road, $A$ selects node $E$, the slowest one behind it that can get out of $A$'s range in the opposite moving direction first. We can simply substitute the values of acceleration and velocity to the formulas (1)-(7) to compute the results because all parameters are vectors.
\end{comment}
%One more scenario is  that in addition to helping deliver the broadcasting message, the
%nodes in the opposite moving direction also need to be advised the message (Fig.~\ref{fig7}).

\begin{comment}
\begin{figure}[!htp]
\begin{center}
\includegraphics[width=8.0cm]{carcase_0.eps}
\end{center}
\caption{Case 0}
\label{fig45}
\end{figure}
\end{comment}

\begin{figure}[!htp]
\begin{center}
\includegraphics[width=8.0cm]{carcase_2.eps}
\end{center}
\caption{Moving direction and broadcasting direction are identical}
\label{fig5}
\end{figure}


\begin{figure}[!htp]
\begin{center}
\includegraphics[width=8.0cm]{carcase_3.eps}
\end{center}
\caption{Moving direction and broadcasting direction are opposite}
\label{fig6}
\end{figure}

%\begin{figure}[!htp]
%\begin{center}
%\includegraphics[width=8.0cm]{carcase_5.eps}
%\end{center}
%\caption{Scenario example 3}
%\label{fig13}
%\end{figure}

\begin{comment}
\begin{figure}[!htp]
\begin{center}
\includegraphics[width=8.0cm]{carcase_4.eps}
\end{center}
\caption{Case 4}
\label{fig7}
\end{figure}
\end{comment}

 \subsection{Algorithm Description}

%In our approach , at time $k$, each node updates and keeps its variance $p_{k-1}$ and the potential acceleration $\hat{a_{k}^-}$ of time $k-1$.
In the broadcasting process, the location of the initiator is included in the broadcasting message. Once a node receives a broadcasting message, it computes the distance to the
initiator. We can define a distance threshold. The messages are only broadcast within this threshold. If the distance is greater than the threshold, the node stops re-broadcasting. When
initiating a broadcasting message or upon receiving a re-broadcasting signal, a node calls the algorithm SFBB. The node handles different scenarios by the algorithm Handle\_msg.

\begin{comment}
Otherwise the node handles the following five cases.\\
Case 0: the broadcasting
direction and its moving direction are identical, and the nodes in its same moving direction don't need to be advised the broadcasting message, but the nodes in the opposite direction need. Then the node re-broadcasts
the message to its neighbors in its opposite moving direction and selects the re-broadcasting node in its same moving direction. In this case,
the re-broadcasting node only helps deliver the message (Fig.~\ref{fig45}).\\
Case 1: the broadcasting
direction and its moving direction are identical, and the nodes in opposite moving direction don't need to be advised the message. The node then re-broadcasts
the message to its neighbors in its same moving direction and selects the best candidate in its moving direction (Fig.~\ref{fig1}). \\
Case 2:
the broadcasting
direction and its moving direction are identical, and the nodes in its moving direction and opposite direction need to be advertised the message. Then the node re-broadcasts
the message to  its neighbors before it in its same moving direction and all its neighbors in its opposite moving direction, and then selects the best candidate from those in its same moving direction (Fig.~\ref{fig5}).  \\
Case 3: the broadcasting
direction and its moving direction are opposite, and the nodes in opposite moving don't need to be advertised the message. Then the node re-broadcasts
the message to  its neighbors behind  it in its moving direction, and then selects the best candidate from those in its
opposite moving direction (Fig.~\ref{fig6}).  \\
Case 4: the broadcasting
direction and its moving direction are opposite, and the nodes in opposite moving need to be advertised the message. Then the node re-broadcasts
the message to its neighbors behind  it in its moving direction and its neighbors in its opposite moving direction, and then selects the best candidate from those in its
opposite moving direction (Fig.~\ref{fig7}). \\
In our approach, each node periodically updates and keeps the acceleration variance, the potential acceleration and the velocity of the past time. When
initiating a broadcasting message or upon receiving a broadcasting message, a node handles it by the algorithm SFBB.

\end{comment}



\begin{figure}[hbt]
\baselineskip=10.2pt
% {\scriptsize
{\small
  \noindent\underline{\bf SFBB()} \\
  \text{~~~~}\textbf{if} it is the initiator\\
  \text{~~~~~~~~}  Call Handle\_msg.\\
  \text{~~~~}\textbf{elseif} the distance to the initiator is greater than the threshold \\
  \text{~~~~~~~~~~~~}Stop re-broadcasting; \\
  \text{~~~~}\textbf{else} Carry the message; \\
  \text{~~~~~~~~~~~~}Call Handle\_msg right after it gets out of the sender's\\
  \text{~~~~~~~~~~~~}   range.\\
   }

\protect\caption{SFBB algorithm}
\protect\label{routingfig}
\end{figure}


\begin{comment}

\begin{figure}[hbt]
\baselineskip=10.2pt
% {\scriptsize
{\small
  \noindent\underline{\bf  Handle\_msg()} \\
    \text{~~~~}  Switch (Receivers)\\
  \text{~~~~~~~~} case `Vehicles in the same moving direction' \\
  \text{~~~~~~~~~~~~} Broadcast the message to the vehicles in its same\\
   \text{~~~~~~~~~~~~}  moving direction; \\
    \text{~~~~~~~~~~~~}  Break; \\
  \text{~~~~~~~~} case `Vehicles in the opposite direction' \\
  \text{~~~~~~~~~~~~} Broadcast the message to the vehicles in its opposite\\
  \text{~~~~~~~~~~~~} moving direction; \\
  \text{~~~~~~~~~~~~}  Break; \\
  \text{~~~~~~~~~} case `Both directions' \\
  \text{~~~~~~~~~~~~} Broadcast the message to all the vehicles in its range; \\
  \text{~~~~~~~~~~~~}  Break; \\
  \text{~~~~}\textbf{if} moving direction and broadcasting are identical\\
  \text{~~~~~~} Select the node  in the moving direction  that can get out of its\\
  \text{~~~~~~} range firstly in the moving direction. \\
  \text{~~~~}\textbf{elseif} moving direction and broadcasting are different\\
  \text{~~~~~~}  \textbf{if} road type is two ways\\
  \text{~~~~~~~~~} Select the node from opposite lanes that can get out of its\\
  \text{~~~~~~~~~} range firstly opposite to the moving direction. \\
  \text{~~~~~~}  \textbf{else} Select the node from it moving direction that can get out\\
   \text{~~~~~~~~~~~~} of its range firstly opposite to the moving direction. \\
   \text{~~~~} Send a re-broadcasting signal to the node. \\


     }

\protect\caption{Handle\_msg algorithm}
\protect\label{routingfig1}
\end{figure}


\end{comment}



\begin{figure}[hbt]
\baselineskip=10.2pt
% {\scriptsize
{\small
  \noindent\underline{\bf  Handle\_msg()} \\
      \text{~~~} Broadcast the message to all the vehicles in its range; \\
      \text{~~~~}\textbf{if} moving direction and broadcasting are identical\\
  \text{~~~~~~} Select the node  in the moving direction  that can get out of its\\
  \text{~~~~~~} range first in the moving direction. \\
  \text{~~~~}\textbf{elseif} moving direction and broadcasting are different\\
   \text{~~~~~~~~~} Select the node from the opposite moving direction that can\\
  \text{~~~~~~~~~}  get out of its range first opposite to the moving direction. \\
    \text{~~~} Send a re-broadcasting signal to the node. \\

     }

\protect\caption{Handle\_msg algorithm}
\protect\label{routingfig1}
\end{figure}


\begin{comment}
{\small
  \noindent\underline{\bf SFBB()} \\
  \text{~~~~}\textbf{if} the distance to the initiator is greater than the threshold \\
  \text{~~~~~~~~}stop re-broadcasting; \\
  \text{~~~~}\textbf{else} carry the message; \\
  \text{~~~~~~~~~~~~}Handle the message according to the following five cases right after it gets out of the sender's range;\\
  \text{~~~~~~~~~~~~}Case 0: re-broadcast the message to its neighbors in its opposite moving direction;\\
  \text{~~~~~~~~~~~~~~~~}collect the moving status of its neighbors before it in its same moving direction; \\
  \text{~~~~~~~~~~~~~~~~}select and designate the best node to conduct re-broadcasting; \\
  \text{~~~~~~~~~~~~}Case 1: re-broadcast the message to its neighbors before it in its same moving direction;\\
  \text{~~~~~~~~~~~~~~~~}collect the moving status of its neighbors before it in its moving direction; \\
  \text{~~~~~~~~~~~~~~~~}select and designate the best node to conduct re-broadcasting; \\
  \text{~~~~~~~~~~~~}Case 2: re-broadcast
the message to  its neighbors before it in its same moving direction and all its neighbors in its opposite moving direction;\\
  \text{~~~~~~~~~~~~~~~~}collect the moving status of its neighbors before it in its moving direction; \\
  \text{~~~~~~~~~~~~~~~~}select and designate the best node to conduct re-broadcasting; \\
  \text{~~~~~~~~~~~~}Case 3: re-broadcast the message to  its neighbors behind  it in its moving direction;\\
  \text{~~~~~~~~~~~~~~~~}collect the moving status of its neighbors in its opposite moving direction; \\
  \text{~~~~~~~~~~~~~~~~}select and designate the best node to conduct re-broadcasting; \\
  \text{~~~~~~~~~~~~}Case 4: re-broadcast
the message to its neighbors behind  it in its moving direction and its neighbors in its opposite moving direction;\\
  \text{~~~~~~~~~~~~~~~~}collect the moving status of its neighbors in its opposite moving direction; \\
  \text{~~~~~~~~~~~~~~~~}select and designate the best node to conduct re-broadcasting; \\
 }
\end{comment}


==> Jianjun_template/figures/SFBB/simulation.tex <==
\section{Performance Evaluation}
\label{evaluation}


\begin{figure}
% \begin{figure}[!htp]
\begin{center}
\includegraphics[width=8.0cm]{g1.eps}
\end{center}
% \vspace{-0.1in}
\caption{The packet delivery ratio}
\label{fig15}
\end{figure}



\begin{figure}
% \begin{figure}[!htp]
\begin{center}
\includegraphics[width=8.0cm]{g22.eps}
\end{center}
% \vspace{-0.1in}
\caption{The end-to-end delay}
\label{fig16}
\end{figure}


\begin{figure}
% \begin{figure}[!htp]
% \vspace{-0.32in}
\begin{center}
\includegraphics[width=8.0cm]{g3.eps}
\end{center}
\vspace{-0.1in}
\caption{The packet delivery ratio}
\label{fig19}
\end{figure}

We conduct simulations using the GloMoSim wireless network simulator~\cite{ex27}.
We use the tool BonnMotion~\cite{ex28} to generate mobile nodes.
The mobility mode we use is ``ManhattanGrid," which can generate the
nodes distributed in the areas similar to roads or streets.
The size of the environment is 2000X2000 $m^2$.
The number of vehicles varies from 50  to 300 with an increment of 50. We set the average packet generation rate from 0.1 to 0.9 per second.
The packet generation rate represents the number of packets generated by a node per second.
The MAC protocol is 802.11.


Many broadcasting protocols are based on the idea that the current sender selects
the node that is farthest away from itself to conduct the re-broadcast task.
This method is called ``DIST'' in the comparison.
We compare our statistical filter based broadcast protocol ``SFBB'' with the ``DIST'' method
using two metrics.
% are considered in our simulation.
The first one is the package delivery ratio, which
is the ratio of the number of vehicles that receive the broadcasting message over the total number of vehicles.
The second metric is the end-to-end delay. 
It is the time elapsed from the packet generated until the packet reaches the receiver in the desired area.
%It is the time elapsed between the instant the packet enters the re-broadcasting node and
%the reception time of the packet by another node.
%To evaluate the two metrics, the number of nodes is varied from 50 to 300
%with an increment of 50. We also set the packet generation rate to vary from 0.1 up to 0.9 per second.





Fig.~\ref{fig15} shows the average packet delivery ratio when the number of nodes 
changes from 50 to 300 and the average packet generation rate is fixed at 0.5.
The delivery ratio decreases when the number of nodes increases.
This is 
because 802.11 protocol performs poorly with more nodes due to the
packet collision. We can see that the ratio generated by SFBB is 9.2\% higher than DIST overall because SFBB can broadcast
a message in a new place faster with less collision than DIST. 
% And less collision exists in the new place.




\begin{figure}
% \begin{figure}[!htp]
% \vspace{-0.82in}
\begin{center}
\includegraphics[width=8.0cm]{g44.eps}
\end{center}
\vspace{-0.1in}
\caption{The end-to-end delay}
\label{fig20}
\end{figure}



Fig.~\ref{fig16} shows the average end-to-end delay with the same configuration as Fig.~\ref{fig15}.
It illustrates the end-to-end delay of SFBB is 9.1\% lower than that of DIST overall.
This is because SFBB can select the
fastest one to re-broadcast the message.




Fig.~\ref{fig19} presents the packet delivery ratio when the packet generation rate varies from
0.1 to 0.9 and the number of nodes is fixed at 150. Similar to Fig.~\ref{fig15}, the ratio decreases when the value of the packet generation rate increases.
%  due to the collision of dense packets.
This figure indicates that the delivery ratio of SFBB is 9.4\% higher than DIST overall because
the re-broadcasting nodes selected by SFBB enter a new place with less collision
faster than DIST. Fig.~\ref{fig20} shows that the end-to-end delay of the two approaches. 
Again, SFBB has a small end-to-end delay than the DIST method. Overall SFBB is 9.0\% lower than DIST.




==> figures/HDAR/Makefile <==
#---------------------------------------------------------------------------
#  Makefile for latex documents with enhancements to make notes and slides.
#  You must use my macros.tex file if you want to utilize the enhancements.
#     Copyright (c) Jim Griffioen, 1997
#
#  Targets include:
#       init:   type 'make init' before doing anything
#	config:	reset the configuration to "student bw slides"
#       sg:     change the group ownership on RCS files (use after running ci)
#	all:	make the dvi file
#	ps:	make postscript file
#	pdf:	make pdf file
#	html:	make an html version (broken down by subsection)
#       html-nosplit: same as html, but create a single html file
#	bib:	make the bibliography and then .dvi file
#	gv:	make postscript file and ghostview it
#	acro:	make pdf file and acroread it
#	x:	run xdvi on the .dvi file
#	me:	configure for me
#	student: configure for student
#	notes:	configure for notes
#	slides:	configure for slides 
#       bw:	configure for black and white output
#	color:	configure for color output
#	portrait: configure for portrait orientation
#	landscape: configure for landscape orientation
#	2up:	make postscipt with 2 slides per page (plus note area)
#	4up:	make postscipt with 4 slides per page (no note area)
#	webnotes: make tar file with .ps, 2up, 4up, and html for class web page
#	clean:	remove all generated files
#	cleanlatex:  only remove the .dvi, .aux, .bbl, .blg, .log files
#	cleanhtml:  remove the generated html directory
#---------------------------------------------------------------------------

# Define the LaTex file filenames
PAPER=  main

ALLTEXFILES=	${PAPER}.tex \
		maincontents.tex \
		abstract.tex \
		conclusion.tex \
		definition.tex \
		evaluation.tex \
		introduction.tex \
		overview.tex \
		

# Name of figure files - these must be generated files
# because 'make clean' will delete them.
# Do not include non-generated figs here.
GENERATED_FIGS= 

# Names of xfig files used to generate the above .ps files
# Note, this variable is only used to checkout the xfig files
# from the RCS directory
FIG_FILES= 

# Image files (e.g., GIFs or JPGs) to be used directly in HTML docs
IMAGES=	

# Movie files (e.g., Quicktime, AVI, MPEGS) to be used directly in HTML docs
ANIMS=	

# Name of figure files that are not generated
OTHER_FIGS=	

# Name of the Unix group to set the RCS file ownership to
GROUP= netfac

#---------------------------------------------------------------------------
# You should not need to modify anything below this point
#---------------------------------------------------------------------------

#---------------------------------------------------------------------------
# Makefile code needed by all makefiles
#
# This section assumes that the following makefile variables have already
# been defined above
#    PAPER=
#    ALLTEXFILES=
#    GENERATED_FIGS=
#    FIG_FILES=
#    IMAGES=
#    ANIMS=	
#    OTHER_FIGS=
#    GROUP=
#---------------------------------------------------------------------------

# Set TEXINPUTS to find my tex macrosfiles
TEXINPUTS= .:../macros:../../macros:/homes/griff/lib/macros:

#---------------------------------------------------------------------------
# Define the names of the programs to use
#---------------------------------------------------------------------------

# Programs
GRAP=		grap
TPIC=		tpic
FIG2PS=		fig2dev -Lps -m 0.7
FIG2PIC=	fig2dev -Ltpic -m 0.7
LATEX=		latex
BIBTEX=		bibtex
DVI_TO_PS=	dvips -Z -t letter -P cmz
TBL=		tbl
XDVI=		xdvi
RM=		rm
GREP=		grep
GS=		gv
PDFVIEWER=	acroread
LPR=		lpr
CONVERT=	convert
L2H=		latex2html
PS2PDF=		ps2pdf


# name of the config file - defined in macros.tex
CONFIGFILE= config.tex

# name of the latex2html init file
LATEX2HTML_INIT= /homes/griff/.latex2html_init

# printer to use
PRINTER= lp
PRINTER_OPT= -P${PRINTER}


#---------------------------------------------------------------------------
# Rules for Making
#---------------------------------------------------------------------------
.SUFFIXES: .tex .dvi .fig .ps .detex .g .tbl .pic .gif .jpg .bmp .tif .tiff .tex,v .fig,v .pdf
.tex.detex: 	; $(DETEX) $*.tex > $*.detex
.tex.dvi: 	; $(LATEX) $* 
.fig.pic:	; $(FIG2PIC) -Ltpic $<  |  $(GREP) -v ".baseline" > $*.pic
.fig.ps:	; $(FIG2PS) -Lps $< $*.ps
.gif.ps:	; $(CONVERT) $*.gif $*.ps
.jpg.ps:	; $(CONVERT) $*.jpg $*.ps
.bmp.ps:	; $(CONVERT) $*.bmp $*.ps
.tif.ps:	; $(CONVERT) $*.tif $*.ps
.tiff.ps:	; $(CONVERT) $*.tiff $*.ps
.pic.tex:	; $(TPIC) $*.pic > $*.tex
.g.pic:		; $(GRAP) $*.g | $(GREP) -v ".lf" > $*.pic
.g.tex:		; $(GRAP) $*.g | $(GREP) -v ".lf" > $*.pic ; $(TPIC) $*.pic
.tbl.pic:	; $(TBL) $*.tbl > $*.pic
.dvi.ps:	; $(DVI_TO_PS) -o $*.ps $*.dvi 
.ps.pdf:	; $(PS2PDF) $*.ps $*.pdf
.tex,v.tex:	; co $*.tex
.fig,v.fig:	; co $*.fig
.jpg,v.jpg:	; co $*.jpg
.gif,v.gif:	; co $*.gif
.bmp,v.bmp:	; co $*.bmp
.tiff,v.tiff:	; co $*.tiff
.tif,v.tif:	; co $*.tif

# Different Make options

all: ${PAPER}.dvi ${PAPER}.ps

${PAPER}.dvi: ${ALLTEXFILES} ${FIG_FILES} ${IMAGES} ${ANIMS} ${GENERATED_FIGS}
	$(LATEX) ${PAPER}

setgrp: 
	chgrp $(GROUP) RCS/*
sg: 
	chgrp $(GROUP) RCS/*

generated_figs: ${GENERATED_FIGS}

print: ${PAPER}.dvi

ps: ${PAPER}.ps

pdf: ${PAPER}.pdf

${PAPER}.ps: ${PAPER}.dvi

${PAPER}.pdf: ${PAPER}.ps

x: ${PAPER}.dvi
	$(XDVI) ${PAPER}.dvi &

gv: ps
	$(GS) ${PAPER}.ps &

gs: ps
	$(GS) ${PAPER}.ps &

acro: pdf
	$(PDFVIEWER) ${PAPER}.pdf &

bib: ${ALLTEXFILES} ${PAPER}.ps
	echo "#!/bin/sh" > .makbib
	echo $(LATEX) ${PAPER} >> .makbib
	echo $(BIBTEX) ${PAPER} >> .makbib
	echo $(LATEX) ${PAPER} >> .makbib
	echo $(LATEX) ${PAPER} >> .makbib
	chmod a+x .makbib
	./.makbib
	rm .makbib

me:
	cat $(CONFIGFILE) | sed "s/studenttrue/studentfalse/" > .tmp
	cp .tmp $(CONFIGFILE); rm .tmp
	cat $(CONFIGFILE) | sed "s/instructorfalse/instructortrue/" > .tmp
	cp .tmp $(CONFIGFILE); rm .tmp
instructor:
	cat $(CONFIGFILE) | sed "s/studenttrue/studentfalse/" > .tmp
	cp .tmp $(CONFIGFILE); rm .tmp
	cat $(CONFIGFILE) | sed "s/instructorfalse/instructortrue/" > .tmp
	cp .tmp $(CONFIGFILE); rm .tmp
student:
	cat $(CONFIGFILE) | sed "s/studentfalse/studenttrue/" > .tmp
	cp .tmp $(CONFIGFILE); rm .tmp
	cat $(CONFIGFILE) | sed "s/instructortrue/instructorfalse/" > .tmp
	cp .tmp $(CONFIGFILE); rm .tmp
slides:
	cat $(CONFIGFILE) | sed "s/slidesfalse/slidestrue/" > .tmp
	cp .tmp $(CONFIGFILE); rm .tmp
	cat $(CONFIGFILE) | sed "s/notestrue/notesfalse/" > .tmp
	cp .tmp $(CONFIGFILE); rm .tmp
notes:
	cat $(CONFIGFILE) | sed "s/slidestrue/slidesfalse/" > .tmp
	cp .tmp $(CONFIGFILE); rm .tmp
	cat $(CONFIGFILE) | sed "s/notesfalse/notestrue/" > .tmp
	cp .tmp $(CONFIGFILE); rm .tmp
color:
	cat $(CONFIGFILE) | sed "s/wantcolorfalse/wantcolortrue/" > .tmp
	cp .tmp $(CONFIGFILE); rm .tmp
bw:
	cat $(CONFIGFILE) | sed "s/wantcolortrue/wantcolorfalse/" > .tmp
	cp .tmp $(CONFIGFILE); rm .tmp
portrait:
	cat $(CONFIGFILE) | sed "s/landscapetrue/landscapefalse/" > .tmp
	cp .tmp $(CONFIGFILE); rm .tmp
landscape:
	cat $(CONFIGFILE) | sed "s/landscapefalse/landscapetrue/" > .tmp
	cp .tmp $(CONFIGFILE); rm .tmp
init:	config
config:
	/bin/echo '\\slidestrue' > $(CONFIGFILE)
	/bin/echo '\\notesfalse' >> $(CONFIGFILE)
	/bin/echo '\\instructorfalse' >> $(CONFIGFILE)
	/bin/echo '\\studenttrue' >> $(CONFIGFILE)
	/bin/echo '\\wantcolortrue' >> $(CONFIGFILE)
	/bin/echo '\\landscapefalse' >> $(CONFIGFILE)

html-split: $(PAPER).dvi
	$(L2H) -split 8 -bottom_navigation -info "" -local_icons \
	-init_file $(LATEX2HTML_INIT) $(PAPER).tex
	@echo copying $(IMAGES) $(ANIMS) into the $(PAPER) directory
	cp $(IMAGES) $(ANIMS) $(PAPER)

html: $(PAPER).dvi
	$(L2H) -split 0 -no_navigation -info "" -local_icons \
	-init_file $(LATEX2HTML_INIT) $(PAPER).tex
	@echo copying $(IMAGES) $(ANIMS) into the $(PAPER) directory
	cp $(IMAGES) $(ANIMS) $(PAPER)

html-nosplit: $(PAPER).dvi
	$(L2H) -split 0 -no_navigation -info "" -local_icons \
	-init_file $(LATEX2HTML_INIT) $(PAPER).tex
	@echo copying $(IMAGES) $(ANIMS) into the $(PAPER) directory
	cp $(IMAGES) $(ANIMS) $(PAPER)

html-noimages: $(PAPER).dvi
	$(L2H) -split 0 -no_images -no_navigation -info "" $(PAPER).tex
	@echo copying $(IMAGES) $(ANIMS) into the $(PAPER) directory
	cp $(IMAGES) $(ANIMS) $(PAPER)

htmlln:
	ln -s /homes/griff/lib/macros/html.sty.foremergencies html.sty

2up: ps
	2up -p${PAPER}-2pp.ps ${PAPER}.ps

4up: ps
	mpage -P -4 ${PAPER}.ps > ${PAPER}-4pp.ps

webnotes: 2up 4up html tar

tar:
	tar -vcf - ${PAPER}.ps ${PAPER}-2pp.ps ${PAPER}-4pp.ps ${PAPER} \
	| gzip > webnotes.tgz

clean: cleanlatex cleanfigs cleanps cleanhtml cleanpdf

cleanlatex:
	$(RM) -f *.aux *.bbl *.blg *.log *.dvi

cleanhtml:
	$(RM) -rf ${PAPER}

cleanfigs:
	$(RM) -f ${GENERATED_FIGS}

cleanps:
	$(RM) -f ${PAPER}.ps

cleanpdf:
	$(RM) -f ${PAPER}.pdf

ppp5:
	rsh ppp5 rm pap.ps pap.ps.gz
	cat ${PAPER}.ps | gzip > pap.ps.gz
	rcp pap.ps.gz ppp5:
	rsh ppp5 gunzip pap.ps.gz
	rm pap.ps.gz

ppp6:
	rsh ppp6 rm pap.ps pap.ps.gz
	cat ${PAPER}.ps | gzip > pap.ps.gz
	rcp pap.ps.gz ppp6:
	rsh ppp6 gunzip pap.ps.gz
	rm pap.ps.gz

ppp9:
	rsh 204.198.76.89 rm pap.ps pap.ps.gz
	cat ${PAPER}.ps | gzip > pap.ps.gz
	rcp pap.ps.gz 204.198.76.89:
	rsh 204.198.76.89 gunzip pap.ps.gz
	rm pap.ps.gz



==> figures/HDAR/abstract.tex <==
In wireless ad-hoc networks, an important issue of Geographic Routing is ``local minimum" problem, which 
is caused by ``hole" that blocks the greedy forwarding process. Existing geographic
routing algorithms use perimeter routing strategies to find a long detour
path when such a situation occurs. To avoid the long detour path, recent research
focuses on detecting the hole in advance, then the nodes located on the boundary of the hole
advertise the hole information to the nodes near the hole. Hence the long detour 
path can be avoided in future routing. We propose a heuristic hole detecting algorithm which 
can identify the hole easily and quickly. In addition, we quantitatively figure out the areas
in the vicinity of the hole that need to be announced the hole information. With such information,
a new routing scheme was developed. Simulation results illustrate
that our approach can achieve better performance in terms of the average length and number of hops of routing 
paths. Simulation also shows that our approach introduces very small computational complexity.




==> figures/HDAR/algorithm.tex <==
\section{Intermediate Targets Geographic Routing (ITGR)}
\label{algorithm}
In this section, we describe our routing approach. We also discuss how to merge the entries that contain pairs of 
shaded area and associated landmark. 




\subsection{Intermediate Targets Routing outline}



%Algorithm 1 shows the approaches to find  the shaded destination area when there is a hole that blocks 
%the routing path from a source node $S$ to a destination node $D$.
%We further present our intermediate targets routing algorithm. 
In ITGR routing algorithm, when a source node $S$ intends to send packets to the destination 
node $D$, it looks up its local cache to see whether $<$ $shaded\_des\_area$, $landmark$ $>$ exists 
and whether $D$ is in this area. If $S$ finds this kind of entry in its cache, it will consider the landmark as its 
tentative target and forward the packets to next hop. Otherwise, the  node $S$ will perform greedy or 
perimeter routing to forward  packets with destination node $D$ to next hop. 
Once the packets reach the destination, the destination  checks whether there is a landmark in the routing path or not. 
If there is, the destination will inform the source node $S$ to calculate the shaded area and then $S$ will update  
its local cache by the fresh entry $<$ $shaded\_des\_area$, $landmark$ $>$ . Hence, if node $S$ forwards packets to any nodes in
a shaded area in the future, it will
extracte the corresponding landmark node from its local cache as a tentative target and then forward packets
to next hop.




\subsection{Determining nodes located in shaded areas}

For a destination node $D$, how can we determine if it is located in a certain shaded area?
Normally, the area is enclosed by rays and partial edges of the hole polygon. 
For instance, in Fig.~\ref{fig2}, 
the area is enclosed by ray $BE$, the hole's edges from $B$ to $F$ 
and ray $FC$. While $S$ does not know node $F${'}$s$ location,
 we need to find other point as reference to evaluate if a destination node is located in the shaded area or not. 
Since no active nodes in the hole,  we can simply determine if the destination is in the area $EBPC$.
 
Suppose that points $S$,$B$ and $P${'}$s$ coordinates are $S(x_s,y_s)$,$B(x_b,y_b)$ and $P(x_p,y_p)$ respectively. 
 If a destination node $G$ satisfies the following three conditions, it must be located in the shaded area:
 \begin{enumerate}
\item $G$ and $P$ are located on the same side of line $SB$;
\item $G$ and $B$ are located on the same side of line $SP$;
\item $G$ and $S$ are located on different sides of line $BP$.
\end{enumerate} 
 
To determine it, we write line $SB${'}$s$ function as: 
\begin{displaymath}
\frac{y-y_s}{y_b-y_s}=\frac{x-x_s}{x_b-x_s}
\end{displaymath}

It can be written as: \\*
$(y_b-y_s)x-(x_b-x_s)y+(x_by_s-x_sy_b)=0$     (1)

Suppose G's coordinates are $G$$(x_g,y_g)$. To determine if $G$ is in the shaded area, 
the first step is to determine if $G$ and $P$ are in the same side of line $SB$.
We substitute $x$ and $y$ in the left term of (1) by $x_g$ and $y_g$ and derive an expression: \\*
$(y_b-y_s)x_g-(x_b-x_s)y_g+(x_by_s-x_sy_b)$    (2)


We then substitute $x$ and $y$ in the left term of (1) by $P${'}$s$ coordinates $x_p$ and $y_p$ and derive another expression: \\*
$(y_b-y_s)x_p-(x_b-x_s)y_p+(x_by_s-x_sy_b)$     (3) \\*

If the symbols of (2) and (3) are identical, $G$ and $P$ are located in the same side of line $SB$, 
we can continue to determine if $G$ is in the shaded area $T$. Otherwise, $G$ cannot be in the shaded area. 

The second step is to determine if $G$ and $B$ are located in the same side of line $SP$.We write line $SP${'}$s$ equation:\\*
$(y_p-y_s)x-(x_p-x_s)y+(x_py_s-x_sy_p)=0$     (4)\\*

Then we substitute $x$ and $y$ in the left term of (4) by $G${'}$s$ coordinates and $B${'}$s$ coordinates and derive two expressions:\\*
$(y_p-y_s)x_g-(x_p-x_s)y_g+(x_py_s-x_sy_p)$      (5)\\*
$(y_p-y_s)x_b-(x_p-x_s)y_b+(x_py_s-x_sy_p)$       (6)

 
If (5) and (6) have different symbols, $G$ cannot be in the shaded area.Otherwise, $G$ and $B$ are located in the same side of 
line $SP$. We then
write the line $BP${'}$s$ equation and substitute $G$ and $S${'}$s$ coordinates to the left term of this equation 
and then got two expressions. 
If the two expressions have different symbols, $G$ and $S$ are located in two sides of 
line $BP$. That is, $G$ is in the shaded destination area. Hence if the destination node $G$ satisfies all the three conditions 
$S$ can conclude that $G$ is located in the shaded area. 



\subsection{Entries combination}
If a node $S$ sends multiple times packets to different destinations, many entries with the 
format $<$ $shaded\_des\_area$, $landmark$ $>$ might be 
generated and be intended to be saved in the node's cache. Among these entries, some landmarks may be identical and some 
shaded destination areas may be overlapped. 
We would like to merge them to save spaces and provide efficient entry lookup in the future. So once a node $S$ sends packets to a destination 
and generates a fresh entry $<$ $area\_SUV$, $B$ $>$, 
it looks up the entries in its local cache and update them.
There are two situations $S$ needs to deal with, one is that $S$ finds an entry in its cache with the same landmark $B$ as the new generated entry. 
Another is that
$S$ finds an entry in its cache whose landmark is not $B$ but whose destination area and $area\_SUV$ are overlap each other.
%to see if 
%there is an entry with the same landmark. If there exists one, then the node updates the entry in its cache by combining the new 
%generated shaded area and the area associated with this landmark that has been saved in its cache.
In the first situation, suppose $S$ finds an entry $<$ $area\_SU^{'}V^{'}$, $B$ $>$ existing in its cache, $S$ then updates
its entries according to the following cases:\\*
Case1: $SU^{'}V^{'}$ $\subset$ $SUV$, that is: $U$ and $V$ are in different sides of $SU^{'}$,
$U$ and $V$ are in different sides of $SV^{'}$.(Fig.~\ref{fig6}) \\*
This scenario can be represented by points' coordinates as follows: Suppose 
that points $S$,$U$, $V$,$U^{'}$ and $V^{'}${'}$s$ coordinates are $S(x_s,y_s)$,$U(x_u,y_u)$, 
$V(x_v,y_v)$,$U^{'}(x_{u^{'}},y_{u^{'}})$ and $V^{'}(x_{v^{'}},y_{v^{'}})$ respectively. \\*
Then line $SU^{'}${'}$s$ equation is: \\*
$(y_{u^{'}}-y_s)x-(x_{u^{'}}-x_s)y+(x_{u^{'}}y_s-x_sy_{u^{'}})=0$  (7)\\*
We substitute $U$ and $V${'}$s$ coordinates in the left term of (7) and derive two expressions: \\*
$(y_{u^{'}}-y_s)x_u-(x_{u^{'}}-x_s)y_u+(x_{u^{'}}y_s-x_sy_{u^{'}})$  (8) \\*
$(y_{u^{'}}-y_s)x_v-(x_{u^{'}}-x_s)y_v+(x_{u^{'}}y_s-x_sy_{u^{'}})$  (9) \\*
If (8) and (9) have different symbols, then $U$ and $V$ are located in different sides of $SU^{'}$.\\*
Line $SV^{'}${'}$s$ equation is:\\*
$(y_{v^{'}}-y_s)x-(x_{v^{'}}-x_s)y+(x_{v^{'}}y_s-x_sy_{v^{'}})=0$  (10)\\*
We substitute $U$ and $V${'}$s$ coordinates in the left term of (10) and derive two expressions: \\*
$(y_{v^{'}}-y_s)x_u-(x_{v^{'}}-x_s)y_u+(x_{v^{'}}y_s-x_sy_{v^{'}})$  (11) \\*
$(y_{v^{'}}-y_s)x_v-(x_{v^{'}}-x_s)y_v+(x_{v^{'}}y_s-x_sy_{v^{'}})$  (12) \\*
If (11) and (12) have different symbols, then $U$ and $V$ are located in different sides of $SV^{'}$.\\*
The update of this scenario is: $S$ removes $<$ $area\_SU^{'}V^{'}$, $B$ $>$ then insert $<$ $area\_SUV$, $B$ $>$. \\*

\begin{figure}[!htp]
\begin{center}
\includegraphics[width=8.0cm]{mer_1.eps}
\end{center}
\caption{The case when $SU^{'}V^{'}$ $\subset$ $SUV$.}
\label{fig6}
\end{figure}





Case2: $SUV$  $\subset$ $SU^{'}V^{'}$, that is: $U^{'}$ and $V^{'}$ are in different sides of $SU$,
$U^{'}$ and $V^{'}$ are in different sides of $SV$.(Fig.~\ref{fig7}) \\* Their relative locations can still be
represented by points' coordinates as case 1.
The coresponding update is: $S$ does nothing. \\*

\begin{figure}[!htp]
\begin{center}
\includegraphics[width=8.0cm]{mer_3.eps}
\end{center}
\caption{The case when $SUV$ $\subset$ $SU^{'}V^{'}$  .}
\label{fig7}
\end{figure}

Case3: The area of $SUV$ and $SU^{'}V^{'}$ are overlapped and $U$ and $V$ are in different sides of $SU^{'}$, 
$U$ and $V$ are in the same side of $SV^{'}$. (Fig.~\ref{fig8})
The update is: $S$ removes $<$ $area\_SU^{'}V^{'}$, $B$ $>$ then insert $<$ $area\_SUV^{'}$, $B$ $>$. \\*

\begin{figure}[!htp]
\begin{center}
\includegraphics[width=8.0cm]{mer_2.eps}
\end{center}
\caption{One case when $SUV$ and $SU^{'}V^{'}$ are overlapped. }
\label{fig8}
\end{figure}


Case4: The area of $SUV$ and $SU^{'}V^{'}$ are overlapped and $U^{'}$ and $V^{'}$ are in different sides of $SU$, 
$U^{'}$ and $V^{'}$ are in the same side of $SV$. (Fig.~\ref{fig9})
The update is: $S$ removes $<$ $area\_SU^{'}V^{'}$, $B$ $>$ then insert $<$ $area\_SU^{'}V$, $B$ $>$. \\*

\begin{figure}[!htp]
\begin{center}
\includegraphics[width=8.0cm]{mer_4.eps}
\end{center}
\caption{Another case when $SUV$ and $SU^{'}V^{'}$ are overlapped. }
\label{fig9}
\end{figure}

Case5: The area of $SUV$ and $SU^{'}V^{'}$ are disjoint.The update is just to insert $<$ $area\_SUV^{'}$, $B$ $>$. \\*
In the above cases, we use the nodes' relative locations to determine two areas' inclusion relation. This method  is
avaliable for the areas caused by a hole. However, it may not avaliable for general cases of Computational Geometry.


The second situation is that  S generate a new entry 
$<$ $area\_SUV$, $B$ $>$, it looks up its local cache and 
finds an entry $<$ $area\_SU^{'}V^{'}$, $B^{'}$ $>$. $area\_SUV$ and $area\_SU^{'}V^{'}$
are overlapped. For instance, in Fig.~\ref{fig10}, when $S$ sends packets to $D$, its generates an area enclosed by
$EB$, the hole perimeter from $B$ to $F$ and line $FC$(the extension of $SP$), which is represented by $SBP$ and associated with landmark $B$. When
$S$ sends packets to node $D^{'}$ later, it generates an area represented as $SB^{'}P^{'}$ and associated with landmark $B^{'}$.
A naive update is to simply insert the new generated entry to $S${'}$s$ cache. However, the new entry and the existing entry share the area
$EBF^{'}C^{'}$. Hence, if $S$ wants to send packets to a node $G$ located in the shared area, $S$ will be confused how to figure 
out the intermediate target. So we must keep all the areas stored in a certain node to be disjoint. 
In this scenario, The area $EBF^{'}C^{'}$ is associated with two landmarks $B$ and $B^{'}$,
the paths from $B$ to $G$ and from $B^{'}$ to $G$ are both greedy. The distance from  $B^{'}$ to $G$ is farer away than that from 
$B$ to $G$. We mark $B^{'}$=$argMax(distance(B,G),distance(B^{'},G))$.
We would like to let area $EBF^{'}C^{'}$ only be associated with
$B^{'}$ since if $S$ wants to send packets to a node $G$ in area $EBF^{'}C^{'}$ in the future, the tentative target $B^{'}$ will
cause less potential recursively  tentative target finding than $B$.
In general case, we mark the fresh generated entry is $<$ $area\_SUV$, $B$ $>$, $S$ looks up its entry and finds an entry $<$ $area\_SU^{'}V^{'}$, $B^{'}$ $>$,
$area\_SUV$ and $area\_SU^{'}V^{'}$ are overlapped. There are four cases to update $S{'}$$s$ entries.\\*
\begin{figure}[!htp]
\begin{center}
\includegraphics[width=7.0cm]{overlap_1.eps}
\end{center}
\caption{The case when $SUV$ and $SU^{'}V^{'}$ with different landmarks are overlapped. }
\label{fig10}
\end{figure}



Case 1: $SU^{'}V^{'}$ $\subset$ $SUV$, that is: $U$ and $V$ are in different sides of $SU^{'}$,
$U$ and $V$ are in different sides of $SV^{'}$(Fig.~\ref{fig11}). \\*
The update is: \\*
If $B$ is $argMax(distance(B,G),distance(B^{'},G))$,
$S$  removes $<$ $area\_SU^{'}V^{'}$, $B^{'}$ $>$ and then
   inserts $<$ $area\_SUV$, $B$ $>$. \\*
If $B^{'}$ is $argMax(distance(B,G),distance(B^{'},G))$,$S$ inserts $<$ $area\_SUU^{'}$, $B$ $>$ and inserts $<$ $area\_SVV^{'}$, $B$ $>$. \\*  
$S$ does this update because once an area is the overlap of two areas, $S$ makes it be associated with the landmark that is
farer away from an arbitratry  node in the shaded common area for less recursive tentative targets finding in the future.    

\begin{figure}[!htp]
\begin{center}
\includegraphics[width=4.0cm]{overope_1.eps}
\end{center}
\caption{The case when $SU^{'}V^{'}$ $\subset$ $SUV$.}
\label{fig11}
\end{figure}


Case2: $SUV$  $\subset$ $SU^{'}V^{'}$, that is: $U^{'}$ and $V^{'}$ are in different sides of $SU$,
$U^{'}$ and $V^{'}$ are in different sides of $SV$.(Fig.~\ref{fig12}) \\*
The update is:\\ If $B$ is $argMax(distance(B,G),distance(B^{'},G))$, $S$  removes $<$ $area\_SU^{'}V^{'}$, $B^{'}$ $>$, then
inserts $<$ $area\_SUV$, $B$ $>$, $<$ $area\_SU^{'}U$, $B^{'}$ $>$ and $<$ $area\_SV^{'}V$, $B^{'}$ $>$.\\*
If $B^{'}$ is $argMax(distance(B,G),distance(B^{'},G))$, $S$ does nothing.

\begin{figure}[!htp]
\begin{center}
\includegraphics[width=4.0cm]{overope_2.eps}
\end{center}
\caption{The case when $SUV$ $\subset$ $SU^{'}V^{'}$ .}
\label{fig12}
\end{figure}


Case3: The area of $SUV$ and $SU^{'}V^{'}$ are overlapped and $U$ and $V$ are in different sides of $SU^{'}$, 
$U$ and $V$ are in the same side of $SV^{'}$. (Fig.~\ref{fig13})
The update is: 
If $B$ is $argMax(distance(B,G),distance(B^{'},G))$,$S$  removes $<$ $area\_SU^{'}V^{'}$, $B^{'}$ $>$ and then
inserts $<$ $area\_SUV$, $B$ $>$ and $<$ $area\_SVV^{'}$, $B^{'}$ $>$. \\*
If $B^{'}$ is $argMax(distance(B,G),distance(B^{'},G))$,then $S$ inserts $<$ $area\_SUU^{'}$, $B$ $>$.
\begin{figure}[!htp]
\begin{center}
\includegraphics[width=4.0cm]{overope_3.eps}
\end{center}
\caption{One case when $SUV$ and $SU^{'}V^{'}$ are overlapped.}
\label{fig13}
\end{figure}



Case4: The area of $SUV$ and $SU^{'}V^{'}$ are overlapped and $U^{'}$ and $V^{'}$ are in different sides of $SU$, 
$U^{'}$ and $V^{'}$ are in the same side of $SV$. (Fig.~\ref{fig14})
The update is: 
If $B$ is $argMax(distance(B,G),distance(B^{'},G))$,$S$  removes $<$ $area\_SU^{'}V^{'}$, $B^{'}$ $>$ and then
inserts $<$ $area\_SUV$, $B$ $>$ and $<$ $area\_SU^{'}U$, $B^{'}$ $>$. \\*
If $B^{'}$ is $argMax(distance(B,G),distance(B^{'},G))$,then $S$ inserts $<$ $area\_SV^{'}V$, $B$ $>$.
\begin{figure}[!htp]
\begin{center}
\includegraphics[width=4.0cm]{overope_4.eps}
\end{center}
\caption{Another case when $SUV$ and $SU^{'}V^{'}$ are overlapped.}
\label{fig14}
\end{figure}










 


\begin{comment}
\begin{algorithm}[bt] 
\begin{algorithmic}[1] 
\caption{{\em Intermediate Targets Routing}}
\label{algorithm2}
\WHILE{packets have not arrived destination D}
\STATE{$S$ looks up its local cache to see if any $<$ $shaded\_des\_area$, $landmark$ $>$ exists 
and if its forwarding packets{'}$s$ destination $D^{'}$ is in the shaded destination area}
\IF{$S$ finds $D^{'}$ is in a shaded destination area in an entry}
\STATE{$S$ counts the corresponding landmark node $B$ as tentative target $D^{'}$ and forwards packets to next hop $S_1$}
\STATE{$S \leftarrow S_1$}
\ENDIF
\IF{$S$ finds no such entry}
\STATE{$S$ forwards packets with destination $D^{'}$ by GPSR to next hop $S_1$}
\STATE{$S \leftarrow S_1$}
\ENDIF
\ENDWHILE
\IF{packets arrive $D$}
\STATE{$D$ check if there the path is detour}
\IF{the path is detour}
\STATE{$D$ informs $S$ the  landmark and local minimal node $P$}
\STATE{$S$ calculates the shaded destination area and  updates its local cache}
\ENDIF
\ENDIF
\IF{the  packets never arrives the destination after a certain TTL}
\STATE{the packets are discarded and the source node reports $D$ is unreachable.}
\ENDIF


\end{algorithmic}
\end{algorithm}
\end{comment}



\subsection{ITGR routing scheme}

\begin{figure}[hbt]
\baselineskip=10.2pt

{\scriptsize
  \noindent\underline{\bf S initiates sending a packet to destination node D} \\
  \text{~~~~}Looks up its local cache to see whether any $<$ $shaded\_des\_area$, $landmark$ $>$ exists 
and whether $D$ is in the shaded destination area; \\
  \text{~~~~}\textbf{if} finds $D$ is in a shaded destination area \\
  \text{~~~~~~~~}Counts the corresponding landmark node $B$ as tentative target $D^{'}$;\\
  \text{~~~~}forwards packets to next hop;\\
  \text{~~~~}S is waiting to receive ACK after sending the packet;\\
  \text{~~~~}\textbf{if} didn't receive an ACK after a certain TTL\\
  \text{~~~~~~~~}Reports that data sending fails;
  \\
  
  \noindent\underline{\bf When a node receives the data packet} \\
  \text{~~~~}Extracts the destination node from the packet's header; \\
  \text{~~~~}\textbf{if} this node is the destination node D\\
  \text{~~~~~~~~}Checks whether local minimal P and landmark B exists\\
  \text{~~~~~~~~}\textbf{if} they exist\\
  \text{~~~~~~~~~~~~}Sends an ACK and a $landmark\_exist\_msg$ to source containing the locations of B and P\\ 
  \text{~~~~~~~~}\textbf{else} sends an ACK to the source\\
  \text{~~~~}\textbf{else} looks up its local cache to see whether any $<$ $shaded\_des\_area$, $landmark$ $>$ exists 
and whether its forwarding packets{'}$s$ destination node is in the shaded destination area; \\
  \text{~~~~~~~~}\textbf{if} finds the destination node is in a shaded destination area \\
  \text{~~~~~~~~~~~~}Counts the corresponding landmark node $B$ as tentative target $D^{'}$;\\
  \text{~~~~~~~~}Forwards packets to next hop;\\
  \\
  
  \noindent\underline{\bf When a node receives $landmark\_exist\_msg$} \\
  \text{~~~~}Calculates the shaded area by the method in Shaded Area Calculation Algorithm; \\
  \text{~~~~}Updates its local cache; \\
  
  
}

\protect\caption{Intermediate Targets Routing Algorithm}
\protect\label{routingfig}
\end{figure}







The algorithm in Fig.~\ref{routingfig} describes the routing scheme when $S$ sends packets to $D$. 
%Suppose the packets record the landmark if the path is detour then the destination will know it. 
In this algorithm, the source node
$S$ looks up its local cache to see if any $<$ $shaded\_des\_area$, $landmark$ $>$ exists 
and if its forwarding packets' destination $D$ is in the shaded destination area. If 
$S$ finds $D$ is in a shaded destination area in an entry, $S$ will count 
the corresponding landmark node $B$ as tentative target $D^{'}$  and forwards packets to next hop node, say $S_1$,
then $S_1$ will begin the entry lookup and forward packets to next hop. If $S$ finds no such entry, 
$S$ forwards packets with destination $D^{'}$ by GPSR to next hop $S_1$, $S_1$ will begin the entry lookup 
and forwrding  operations. 
%So at the beginning when $S$ attempts to forward
%packets, the $D^{'}$ in the algorithm is the final  destination node $D$. But once an entry is found, the $D^{'}$
%will be replaced  by a landmark node. 
%In any step, if the packets are forwarded to the fixed destination $D$,line 1 to line 8 will be done.
The algorithm contains two aspects, one is to select an intermediate node as tentative target to 
conduct the ITGR routing algorithm, another is to calculate the $<$ $shaded\_des\_area$, $landmark$ $>$
entry and save it to a node's cache.Both of them can be peformed  recursively.

The recursion mostly happen in the scenario such  that $\angle$ $BSD$ $\geq$ $\frac{\pi}{2}$ and
$\angle$ $BDS$ $<$ $\frac{\pi}{2}$(Fig.~\ref{fig3}) or the situation that $\angle$ $BSD$ $<$ $\frac{\pi}{2}$ 
and $\angle$ $BDS$ $\geq$ $\frac{\pi}{2}$(Fig.~\ref{fig4}). Fig.~\ref{fig5} is an instance to generate the
$<$shaded\_des\_area, landmark$>$ 
entry recursively. The first time when $S$ 
wants to send packet to $D$, it generates and saves the entry $<$ $area\_SBP$, $B$ $>$  to its cache. 
When $S$ selects $B$ as its intermediate target for routing, it will meets local minimal node $P^{'}$ and generate an entry
$<$ $area\_SB^{'}P^{'}$, $B^{'}$ $>$, then $S$ will update its cache.

\begin{figure} [!htp]
\begin{center}
\includegraphics[width=8.0cm]{figure5.eps}
%\includegraphics[width=8.0cm]{path2.eps}
%\includegraphics[width=8.0cm]{hops.eps}
\end{center}
\caption{Recursively generate shaded areas and recursively conduct ITGR}
\label{fig5}
\end{figure}

Intermediate targets routing algorithm can be recursively conducted as well. Suppose the pairs of entries 
$<$ $area\_SP^{'}P$, $B$ $>$ and $<$ $area\_SB^{'}P^{'}$, $B^{'}$ $>$ have been stored in S's local cache after updating(Fig.~\ref{fig5}). 
When S is forwarding packets whose destination is $D^{'}$,
 it looks up its local cache and finds that 
$D^{'}$  is in the shaded area $SP^{'}P$ and $B$ is the landmark,so $S$ counts $B$ it 
intermediate target. Then $S$ tries to send the packet to $B$, it looks up 
it local cache and finds node $B$ is in the shaded area $SB^{'}P^{'}$ and $B^{'}$ is the landmark, so $S$ counts 
$B^{'}$ its intermediate target, then tries to send packet to $B^{'}$ by greedy routing. Then from $B^{'}$ to $B$, 
the path is generated by greedy forwarding; 
from $B$ to $D^{'}$ , the path is greedy forwarding as well. This recursive routing makes the routing path is constructed by 
a series of sub-paths, which are all greedy forwarding paths.










==> figures/HDAR/conclusion.tex <==
\section{Conclusion}
\label{conclusion}

In this paper, we presented a heuristic algorithm that detects the hole. 
The hole can be represented concisely and announced to the nodes nearby that
potentially incur detour paths by face routing. The node benefited from 
the hole information can adaptively adjust the forwarding hop to avoid long detour path.
The novelty of the approach is that a single node can detect the hole
efficiently and then the nodes near the hole can benefit from it. 
The experiments indicate that our approach results in significant shorter 
routing path and fewer hops than an existing geographic routing algorithm. And it only
causes few computational complexities.



==> figures/HDAR/definition.tex <==
\newcommand{\bibdir}{./}

\newcommand{\msgrange}{potential range}
\newcommand{\msgranges}{\msgrange s}
\newcommand{\closestneighbors}{$m$-width neighborhood}

\newcommand{\newunstruct}{new unstructured}



==> figures/HDAR/discussion.tex <==
\section{Discussion}
\label{discussion}
In this section, we will discuss the method how to figure out the value of $\delta$, the 
situations  that will cause false positive or false negative when detecting holes and two
types of special circumstances about the hole representation.


\subsection{Derivation of the threshold}
\begin{comment}
In this paper, we define that a hole is a kind of polygon. In this kind of polygon, 
there exists a node p that is a vertex and satisfies that: a node d among the polygon's vertices can 
be found, p is closer to d than any of its neighbors but p cannot reach d directly. P is called local 
minimum node. Our hole detection algorithm is to detect such polygon that containing at least one local 
minimum node. 
\end{comment}
%We consider it is a hole. 

In geographic routing, when a hole exists, there will be a detour path. So we attempt 
to detect a hole by finding a detour path. The ``detour" path is defined as the routing path 
between two nodes that is much longer than their Euclidean distance in this paper. In order to quantitatively represent the 
``much longer", we introduce a threshold $\delta$ that is $length\_pro()/dist\_euc()$. To determine the value of $\delta$, 
we first attempt a polygon like a circle(Fig.~\ref{dis1fig}) in which $\delta$ is $\pi/2=1.57$. However, the circle is not a hole, 
so we will investigate $\delta>1.57$.
\begin{figure}[!htp]
\begin{center}
\includegraphics[width=4.0cm]{dis1.eps}
\end{center}
\caption{A circle is not a hole}
\label{dis1fig}
\end{figure}

We then increase the value of $\delta$. Suppose triangle $abp$ is a regular triangle(Fig.~\ref{dis2fig}), the length of each edge is 1, 
and the transmission range is slightly less than 1, such as 0.9. Then we move a to $a^{'}$ and let both $a^{'}p$ and $a^{'}b$ be equal to the 
transmission range. Then from $p$ to $b$, a path $p \rightarrow a' \rightarrow b$ exists and it is a slight detour path. 
But the triangle is not a hole since none of the three nodes is a local minimum node. In this circumstance,
the value of $\delta$ is approximate equal to 2.

\begin{figure}[!htp]
\begin{center}
\includegraphics[width=4.0cm]{dis2.eps}
\end{center}
\caption{A regular triangle is not a hole}
\label{dis2fig}
\end{figure}

Then we increase the value of $\delta$ to the one that is slightly larger than 2.
We found that $\delta$ =2.25 is a good choice for small false positive and small false negative
by experimental attempts.


\subsection{Discussion of false positive and false negative}
The false negative  and false positive may occur during the hole detection. 
The false negative occurs when the Euclidean distance from a source node to the destination node is close to the
transmission range and the detour path is slightly larger than the Euclidean distance.
%, such as the detour is one more hop than the Euclidean distance. 
For instance, in 
Fig.~\ref{dis3fig}, the transmission range is 0.9,$\mid pd \mid$=0.95, $\mid ad \mid$=$\mid bd \mid$=1,$\mid ed \mid$=$\mid df \mid$=0.9
and $\mid ap \mid$=$\mid pb \mid$=0.9. Then $p$ is a local minimum node and the polygon $paedfb$ is a hole. However, HDAR 
does not detect it is a hole. The false negative is introduced by a very special circumstance that the detour path is
about one hop distance longer than the Euclidean distance. If the detour is longer, then $\delta$ will be greater than
2.25 and the polygon will be considered as  a hole. If the Euclidean distance from $p$ to $d$ is much larger than the transmission
range, the polygon is a long and narrow area. The $\delta$ will be less than 2.25 from $p$'s point of view. But node $e$ or $f$ 
will detect the long and narrow polygon is a hole. The false negative in Fig.~\ref{dis3fig} will not affect the routing too much
because the detour is not too long, normally one hop.


\begin{figure}[!htp]
\begin{center}
\includegraphics[width=4.0cm]{dis3.eps}
\end{center}
\caption{False negative when detecting hole by HDAR}
\label{dis3fig}
\end{figure}

False positive occurs when Euclidean distance from a source node to the destination node is slightly larger than the
transmission range and the detour path is at least three hops long, and each hop is close to the transmission range.
 For instance, in 
Fig.~\ref{dis4fig}, the transmission range is 0.9,$\mid pd \mid$=1, $\mid ed \mid$=0.95,
and $\mid ep \mid$=$\mid ea \mid$=$\mid ad \mid$=$\mid dc \mid$=$\mid cb \mid$=0.9. Where 
 $p$ is not a local minimum node and then the polygon $peadcb$ is not a hole by hole's original definition. 
 However, HDAR 
detects it is a hole. And node $e$ and $p$ will advertise the hole information to an area $epk$. 
The area to be announced is not big
since only a few nodes(two nodes in this example) announce the hole information. If there are more nodes located in any edge such as 
$ea$ or $ep$, then the polygon is a true hole. Although this is a ``pseudo hole" detected by HDAR, the nodes in $epk$ will benefit from the hole information. 
For example, if $s$ wants to send
a packet to $d$, $s$ will send the packet to a directly(green path) instead of detour from $p$(red paths). The false positive 
will occur in very special situations. And the further hole announcement to a small area is not an expensive  task. But the nodes in this 
area will benefit from the hole information.


\begin{figure}[!htp]
\begin{center}
\includegraphics[width=6.0cm]{dis4.eps}
\end{center}
\caption{False positive when detecting hole by HDAR}
\label{dis4fig}
\end{figure}


\subsection{Further discussion of the hole representation}

The hole is represented by a segment that connects the most remote two nodes of the hole in this paper.
However, there may be a second segment that is a little shorter than the segment standing for the hole
and they are almost perpendicular. We will discuss how this situation affects the future routing by two
types of hole shapes. 

In the first type, the shape of hole is a convex polygon(Fig.~\ref{app1fig}). $ef$ represents the hole. There is a second 
segment $ch$ that is a little shorter than $ef$. We fit this polygon by a circle. When node $a$ intends to send a packet to node
$d$, who is on the same side of $a$ relative to $ef$, only GPSR can be used in our routing protocol. Since $a$ and $d$
 are located on the
boundary of a circle, $a$ can always find another node $b$ or $c$ or $g$ that is closer to $d$ as its next hop. So greedy forwarding
is available. In this circumstance, no matter which segment representing the hole will not affect the future routing.






\begin{figure}[!htp]
\begin{center}
\includegraphics[width=8.0cm]{app1.eps}
\end{center}
\caption{The polygon is fitted as a circle}
\label{app1fig}
\end{figure}



The hole is concave in the second type(Fig.~\ref{app2fig}). $ef$ represents the hole. There is a second 
segment $ch$ that is a little shorter than $ef$. We fit this polygon by a 3-regular tree in Poincare disk~\cite{ex31}. 
It can be considered as two sets of hyperbola. They divided the plane into four regions I,II,III and IV by
arc $fh$,$fc$, $ce$ and $eh$ excluding the hole. We illustrate that the possible detour will not be too much by an example node $a$.
When $a$ located in region III wants to send a packet to node $b$, $a$
 finds that $e$ is the tentative target and
the path is constructed by $ae$ and $eb$, both are greedy. When $a$ sends a packet to $g$, since $a$ and $g$
 are on the same side of segment $ef$, $a$ uses greedy to reach $k$, then from $k$ to $c$ by face routing and from $c$ to $g$ by greedy. 
When $a$ sends a packet to $d$, $a$ considers
$f$ as tentative target. Then the path will be constructed by $aj$,$jc$,$cf$ and $fd$, where $jc$
 is face routing path. So no matter what regions 
the source and destination nodes are located, there is at most one piece of face routing path included in one region. And it will not be 
two long. 



\begin{figure}[!htp]
\begin{center}
\includegraphics[width=8.0cm]{app3.eps}
\end{center}
\caption{The polygon is fitted as hyperbolas}
\label{app2fig}
\end{figure}










==> figures/HDAR/evaluation.tex <==
\section{Performance Evaluation}
\label{evaluation}

We conduct our performance evaluation using a
noiseless immobile radio network environment, where the nodes are
distributed in a given area and may each have a different
transmission range and bandwidth. 
Since what we are interested in is to
compare our results with the outputs generated by other allocation
approaches, we convert this network to a weight graph G=(V,E) where
the weight represents the bandwidth. 
We set the number of users to be 30 and 
let the number of channels vary from 25 to 50 with increment 5. 
We set the probability
that an edge exists between any pair of user and channel nodes to be 0.2 
and the edge weight is uniformly distributed from
1 to 9.
For each 
% pair of user number and channel number, 
configuration, 
we 
% randomly 
generate 10 graphs and
conduct the experiment 10 times based on the graphs. 
We calculate the average value from the experiments as the result 
for each configuration.

We use two metrics to evaluate the performance.
One is
%  system utilization, i.e., 
the sum bandwidth of all users by the allocation.
The other is the allocation ratio of the number of users 
who are allocated with at least one channel 
over the number of users who are competing for the spectrum pool.

We compare our solution with three other approaches. The first one 
is NMSB
(Non-collaborative-Max-Sum-Bandwidth). In each step, this approach
picks the vertex with the highest bandwidth and assigns it to its
associated user. Then the algorithm remove the edges that interfere
with this user until all the channels are allocated. The second one
is 
CMSB (Collaborative-Max-Sum-Bandwidth). This approach picks up
the vertex with the highest label, defined as the bandwidth of a
channel 
divided by the number of users interfering with each other with 
regard to this channel. The process is repeated until all channels
have been allocated. The
third approach is MINSTARVE, which tries to allocate the
channels to the users who have not been allocated before. In
this approach, each user has a priority. The user's priority is
decreased by one if the user is allocated with a channel. The
algorithm takes care of higher priority users first.

\begin{figure}[!htp]
\begin{center}
\includegraphics[width=8.0cm]{Fig8.eps}
\end{center}
\caption{Sum bandwidth of allocated channels} \label{fig11} 
\end{figure}

In Fig.~\ref{fig11}, we evaluate the sum bandwidth of these approaches.
The number of channels changes from 25 to 50. The results show
that our approach can achieve near optimal sum bandwidth, similar to 
NMSB.
Both NMSB and our approach are about 10\% to 25\% higher than
the other two approaches.


\begin{figure}[!htp]
\begin{center}
\includegraphics[width=8.0cm]{Fig9.eps}
\end{center}
\caption{Allocation ratios} 
\label{fig12} 
\end{figure}

In Fig.~\ref{fig12}, 
% has the identical network setting as fig 11. But what we concern is 
we evaluate the allocation ratio of the four approaches.
It shows that our algorithm can reach near 100\%
allocation ratio. MINSTARVE is close to 80\%, while the other two
range from 40\% to 70\%. It illustrates that our mechanism can 
better avoid starvation. 

% Combined by the two figures, we can see that Bipartite-graph based
% approach can guarantee as many as possible users to be benefit from
% spectrum and achieve large sum bandwidth as well.


==> figures/HDAR/hdar.tex <==
\section{Hole Detecting and Adaptive Routing}
\label{Algorithms}

\subsection{Hole Detection Algorithm}
In HDAR, a node $p$ begins to detect whether it is located on a hole only if the angle between its two 
adjacent edges is greater than 120 degrees~\cite{ex22}.
% This is because if there is no angle between 
%two adjacent edges respect to $p$ that is bigger than 120 degrees, $p$ can not be a local minimum node. 
$p$ initiates a probe message and writes its location to this message. Then $p$ sends the message to its 
leftmost node respect to the angle. Where the leftmost node is defined as: $p$ faces the area formed by the two rays of 
this angle, then $p$ uses the angle's bisector line to conduct anti-clockwise sweeping, the leftmost node is the first one that met
by the sweeping line. Upon receiving the probe message, $p$'s leftmost neighbor node writes 
its location into the message and passes it to its leftmost neighbor, here the leftmost or rightmost neighbor is defined similarly. The probe message will finally come back 
to node $p$ from $p$'s rightmost neighbor respect to the initial invested angle~\cite{ex22}~\cite{ex30}. 
When the probe message circulates, 
it collects the locations of the nodes on its way. So node $p$ knows all the nodes' locations on the way.


$p$ then begins to investigate the nodes on the way ordered clockwisely. For each node on the way, $p$ computes the length of their probe path $length\_pro()$ 
and their Euclidean distance $dist\_euc()$. For a node $x$, $length\_pro(p, x)/dist\_euc(p, x)$ is defined as hole detection ratio $p$ 
to $x$.
If there exists a node $v$, the hole detection ratio $p$ to whom is larger than a predefined threshold $\delta$, that is,\\
 \text{~~~~~~~~}$length\_pro(p, v)/dist\_euc(p, v)$ $>$ $\delta$ \text{~~~~~~~~}(1) \\
is satisfied, 
then $p$ is considered sitting on a hole. The value of $\delta$ affects the hole detection results. Too big value of $\delta$ introduces 
false negative and too small value of $\delta$ causes false positive. We derived that  $\delta$=2.25 is a good choice to detect 
most holes that will block greedy forwarding.
Fig.~\ref{hdarfig1}  is an example for hole detection. Node $p$ initiates the hole probe message. $p$ collects the nodes' 
locations during the message circulates the loop. Then $p$ finds that there exists a node $v$, 
satisfying $length\_pro(p, v)/dist\_euc(p, v)$ $>$ 2.25 , $p$ is considered sitting on a hole.

\begin{figure}[!htp]
\begin{center}
\includegraphics[width=6.0cm]{fig1.eps}
\end{center}
\caption{P initiates the probe message and it circulates the loop}
\label{hdarfig1}
\end{figure}


The hole that was detected is a polygon. Note that some nodes located on the polygon measure they are 
located on a hole, but other nodes may not consider they are on a hole. For instance, 
in Fig.~\ref{hdarfig1}, node $g$, $p$ and $h$  consider they are on a hole since there exist nodes on the polygon's
boundary to let them satisfy the hole definition (1). However, 
the vertexes $a$ and $b$ at the hole polygon found by $p$ don't consider they are on a hole because $a$ or $b$'s greedy
forwarding will not be blocked
%  does not have to generate detour routing path in future routing due to 
by the polygon. 
%That is, the polygon has minor effect to $a$ or $b$ for their  routing paths.

The node located on the polygon may detect the hole repeatedly, thus a lot of overhead will be generated. 
%In order to reduce the overhead, asynchronous detection is introduced. That is, one will send out the probe 
Fortunately, the overhead can be reduced because of the 802.11 MAC layer random backoff mechanism. In this mechanism,
one will not send out a packet 
%its probe message 
if it overhears an RTS sent to other node.
%that another node in its transmission is sending out a probe message.
Instead, it will wait for a period and then begin to send out its packet only when it hears the CTS plus a period. 
% asynchronous detection is introduced. That is, one will send out the probe 
%message and others will receive it  before sending out theirs. 
We use this mechanism that once a node hears a probe message, it would not schedule a probe message although it has 
not sent out its probe message yet.
% when a probe message comes to it. 
However, a node sitting on the polygon may only 
receive partial of the nodes' information based on this mechanism if the received probe does not start from this node. 
In order to make each node know the locations of all the nodes on the polygon, the probe initiating node sends two probe 
messages clockwise and anti-clockwise at the same time.(shown in Fig.~\ref{hdarfig1}). So each node on the polygon can obtain
the whole information of the polygon. Since the probe message is sent  by both clockwise and anti-clockwise directions,
there will be two probe paths, we choose the longer as the length of the probe path to calculate the hole detection ratio. 

The probe message initiating algorithm is described as Fig.~\ref{initiatefig}.


\begin{figure}[hbt]
\baselineskip=10.2pt
{\small
  \noindent\underline{\bf Probe\_msg\_initiating()} \\
  %\text{~~~~}\textbf{if} receives a probe message \\
  \text{~~~~}\textbf{if} doesn't receive a probe message \\
  %\text{~~~~~~~~}cancel probe\_initiate message; \\
  %\text{~~~~~~~~}\textbf{else} search whether it has an angle between two adjacent edges \\
  \text{~~~~~~~~}\textbf Search whether it has an angle between two adjacent edges \\
  \text{~~~~~~~~}larger than 120 degrees; \\
  \text{~~~~~~~~}\textbf{if} true \\
  \text{~~~~~~~~~~~~}Initiate a probe message; \\
  \text{~~~~~~~~~~~~}Write its location to this message; \\
  \text{~~~~~~~~~~~~}Send it to its left node and right node of the angle.\\
  %\text{~~~~~~~~}\textbf{else}\\
  %\text{~~~~~~~~~~~~}cancel probe\_initiate message. \\
 }

\protect\caption{Probe Message Initiating Algorithm}
\protect\label{initiatefig}
\end{figure}


 The probe message receiving algorithm is described as Fig.~\ref{receivefig}. In this algorithm,
upon receiving a probe message, a node determines whether it is the message initiate node. If it is,
the node will calculate the hole detection ratio when both probe massages come back.  If the node is not the 
message initiate node, it will write its location to the message and forward the message.


\begin{figure}[hbt]
\baselineskip=10.2pt
{\small
  \noindent\underline{\bf Probe\_msg\_receiving()} \\
  \text{~~~~}Compare its location with the message initiator's location to \\
  \text{~~~~}determine whether it is the message initiator \\
  \text{~~~~}\textbf{if} it is the initiator \\
  \text{~~~~~~~~}Search whether the two probe message from  \\
  \text{~~~~~~~~}different directions both reached it; \\
  \text{~~~~~~~~}\textbf{if} true \\
  \text{~~~~~~~~~~~~}Calculate the hole detection ratio \\
  \text{~~~~~~~~}\textbf{else} \\
  \text{~~~~~~~~~~~~}Wait for the second probe message; \\
  \text{~~~~}\textbf{else} \\
  \text{~~~~~~~~}Write its location;\\
  \text{~~~~~~~~}Forward the message to its left or right neighbor\\
  \text{~~~~~~~~}according to the forwarding direction.\\
 }

\protect\caption{Probe Message Receiving Algorithm}
\protect\label{receivefig}
\end{figure}







The probe initiator must have an angle between two adjacent edges with respect to it that is larger than 120 degrees. 
However, such an angle is necessary but not sufficient condition to determine the initiator is a local minimum node, 
but this does not affect our hole detection results since the initial node being regarded as  a local minimum is independent on the fact
that the node detects a hole. A relative destination is needed to determine a local minimum but our hole detection
algorithm does not need a specific destination.
 The objective of the hole probe message is to find a hole, but not to determine if 
the probe initiator is a local minimum node. 

The probe initiator who finds a hole finally may be or may not be 
a local minimum node. In Fig.~\ref{hdarfig1}, node $p$ initiates the hole probe message and finds that it is 
located on a hole. It is a local minimum node if it sends a packet to nodes in the vicinity of node d. In Fig.~\ref{hdarfig2}, node p 
initiates a hole probe message and detects the hole, but $p$ is not a local minimum node. The hole information 
will be announced to the nodes in a certain area and these nodes will be benefited from the hole announcement for future routing. 
%This situation occurs when there is a hole, but the hole probe message is initiated by a node that is not a local minimum node. 


In Fig.~\ref{hdarfig3}, $p$ is a local minimum node. $p$ initiates a hole probe message but it cannot detect the hole 
because the length of 
the probe path from $p$ to any node on the polygon over their Euclidean distance is approximate to 1. However, the hole can be 
detected by another node such as $n$ and the hole information will be announced to areas($ekf$ and $e^{'}k^{'}f^{'}$) containing 
the nodes which will be benefited 
from the hole information in future routing. This phenomenon that a true local minimum node $p$ cannot detect a hole 
occurs when the polygon is long and narrow then the initiator's 
routing will not be blocked by the polygon. So this detecting result has very minor effect to $p$'s forwarding.
Nevertheless, the hole will be detected by another node who suffers from the hole. 
%The hole detected by other node has very minor effect to p's forwarding. And by 
%our determining condition, the ratio of the length of p's probe path to any node in the hole over the Euclidean distance is 
%close to 1. 
%So the effect of this polygon to node $p$ and the hole detection ratio defined in this paper are consistent.


\begin{figure}[!htp]
\begin{center}
\includegraphics[width=6.0cm]{initiator2.eps}
\end{center}
\caption{P is not a local minimum but finds the hole}
\label{hdarfig2}
\end{figure}


\begin{figure}[!htp]
\begin{center}
\includegraphics[width=6.0cm]{initiator3.eps}
\end{center}
\caption{P is a local minimum but does not find the hole}
\label{hdarfig3}
\end{figure}

\subsection{Shape-Free Hole Representation}
The hole that is detected is a polygon. The representation of a polygon is a sequence of vertexes. 
However, in geographic routing, we don't have to care all the nodes on the polygon because most of 
them have minor effect to determine the routing paths. What we concern are the nodes that will block the 
greedy forwarding.
In our model, since $p$ has already obtained all the nodes' locations on the polygon(Fig.~\ref{hdarfig2}), 
$p$ calculates the two nodes whose Euclidean distance is most remote. The segment connecting these 
two nodes looks like a board that blocks the greedy forwarding. For instance, segment $ab$ in Fig.~\ref{hdarfig2} is 
the board that blocks the greedy forwarding. Then the hole is represented as $<a,b>$. 
No matter what the shape of the hole is, what we concern is 
the segment connecting the two most remote nodes.


\subsection{Determining the Shaded Area}
That the greedy forwarding is blocked by the board $<a,b>$ is because some potential  destination nodes 
are hidden behind the board, and the source nodes located in a certain area that is in the opposite 
side to the hidden destinations are not aware of them. In the basic routing approach, a source 
node just conducts the greedy forwarding until it fails due to the local minimum node, where the greedy 
forwarding changes to face forwarding. Thus the detour paths are generated. If the possible destination nodes 
hidden behind the board can be figured out in advance and be announced to the source nodes in the certain area, 
the length of the routing paths can be dramatically reduced. We determine the possible destination area(shaded area)
as follows: Draw line $ar$ perpendicular to segment $ab$, $r$ and $p$ are at the opposite sides of $ab$. Also draw line $bt$ 
perpendicular to line $ab$, $t$ and $p$ are at  the opposite sides of ab. Then the area $rabt$ is the shaded area(Fig.~\ref{hdarfig4}). 



\subsection{Hole Announcement}
The nodes in area $rabt$ are the possible destination nodes associated with some source nodes. 
We would like to figure out an area containing these source nodes that will be announced 
the hole information in the opposite side of $rabt$(Fig.~\ref{hdarfig4}). The hole information will help 
the nodes adaptively adjust the next forwarding hops to avoid detour routing paths. 
In order to determine the hole announcement area, the announcement breadth and depth 
need to be figured out. We first find node $e$ and node $f$ at the same side as node $p$ 
relative to segment $ab$ that are the left and right nodes furthest away from each other and satisfy the hole 
detection condition (1). Let $c$ be the midpoint of segment $ef$. Draw segment $ck$ perpendicular 
to $ef$. Then the triangle $efk$ is the area that should 
be announced the hole information. Note that hole announcement area is larger, 
more nodes will be advertised the hole information and the future routing path will be shorter. 
However, the area is larger, more overheads will be introduced. 
So there is a tradeoff between the benefit to the future routing path and the overhead. 
The optimal values of the hole information announcement size that can both shorten 
the future routing path and reduce the overhead need to be found. The announcement 
breadth is selected as segment $ef$ since $e$ and $f$ are most remote nodes on the hole's boundary
located on the same side of $p$ satisfying the hole detection condition.
%is the leftmost node that satisfies the 
%hole detection condition and $f$ is the rightmost node that satisfies the hole detection 
%condition. 
So the announcement depth determines the size of the area. 
We let the length of $ec$ be $l$ and
% approximate the length of $ef$ to be $L$. And we 
mark $\angle cek$ to be $\alpha$.
Assume that the nodes are distributed in the plane uniformly. So the number of the nodes in $\bigtriangleup$ekf
can be represented by the area of $\bigtriangleup$ekf:\\
\text{~~~~~~~~}$\frac{1}{2}$$\cdot$$2l$$\cdot$$l$$\tan\alpha$$=$$l^{2}$$\tan\alpha$,$\alpha\in\lbrack0,\frac{\pi}{2}\rbrack$ \\
For node $s$, if it intends to send a packet to node $d$ by HDAR routing protocol, the path includes the sub-paths $s \rightarrow k$,
$k \rightarrow e$, $e \rightarrow a$ and $a \rightarrow d$. The last two sub-paths are fixed, 
but $s \rightarrow k$ and $k \rightarrow e$ depend on $\alpha$. Let the length of $sc$ be $h$, 
we approximately represent the length of path $sk$ by $h-\mid kc\mid=h-l$$\tan\alpha$,
and the length of path $k \rightarrow e$ by $\mid ke\mid$ since the routing path generated by HDAR 
will be along $ke$. Here  $\mid ke\mid$ is $\frac{l}{\cos\alpha}$. Hence from $s$ to $e$, the length of paths is:\\
\text{~~~~~~~~}$(h-l$$\tan\alpha)+\frac{l}{\cos\alpha}$     \\
We want to find an $\alpha$ that can try to minimize both the area of $\bigtriangleup$ekf and the length of routing path.
The optimal value to minimize both is depended on $\alpha$. We deduced that the best solution is that when $\alpha$ is 1.05. 
We approximate the length of $ef(2l)$ to be $\mid ab\mid$. Then the optimal length of the depth ck 
is $\tan\alpha$*$\frac{1}{2}\mid ef\mid$, that is: $0.87*\mid ab\mid$. The details will be discussed in the appendix. 

The nodes on the arc $ef$ begin to advertise the hole information $<a,b>$ to their neighbors. 
In order to avoid duplicate messages, once a node in 
the area has received the hole information, it simply discards the duplicate. 
After the  advertisement of hole's information, each node in the area $efk$ knows that any possible 
destination node in area $rabt$ is hidden behind the the board $<a,b>$(The red nodes and boundary nodes from $e$ to $f$
in Fig.~\ref{hdarfig4}) .

\begin{figure}[!htp]
\begin{center}
\includegraphics[width=6.0cm]{main.eps}
\end{center}
\caption{Hole Announcement}
\label{hdarfig4}
\end{figure}





\subsection{Adaptive routing}
After the announcement, each node in the triangle $ekf$ knows that there is a hole $<a,b>$ that blocks the greedy 
forwarding to any destination node in area $rabt$. So the nodes in triangle $ekf$ can adaptively adjust the routing 
path. In the network plane, once a node $s$ intends to send a packet with destination $d$, it first looks up its local 
cache to see whether it has a hole information entry $<a,b>$. If there is no such entry in its local cache, it just 
conducts GPSR. Else if there is a hole information entry $<a,b>$ but $s$ and $d$ are located at the same side of segment 
$ab$, $s$ just conducts GPSR. If $s$ and $d$ are located on the opposite sides of $ab$ but $d$ is not in the shaded area $rabt$, 
$s$ just conducts GPSR. Else $d$ must be in the area $rabt$. In this situation, $s$ wants to consider $a$ or $b$ as its tentative 
target and then writes $a$ or $b$ to the packet's head as a tentative target. In order to make $s$ determine which one  
should be the tentative target, let $m$ be the midpoint of segment $ab$, $mn$ is perpendicular to segment $ab$ and 
$n$ is at the opposite side of $ab$ compared with $s$. Then if $d$ is 
located in area $ramn$, $s$ writes $a$ to the packet's head as its tentative target. If $d$ is located in area $nmbt$, 
$s$ writes $b$ to the packet's head 
as its tentative target. When the packet reaches $a$ or $b$, the tentative target will continue  
sending the packet to the destination node $d$.

When a node is forwarding a packet to its next hop, it calls $HDAR\_forwarding()$ described in Fig.~\ref{forwardfig}.

\begin{figure}[hbt]
\baselineskip=10.2pt
{\small
  \noindent\underline{\bf HDAR\_forwarding()} \\
  \text{~~~~}Look at the forwarding packet whether this node has a tentative \\
  \text{~~~~~~~~}target ${\cal T}$ \\
  \text{~~~~}\textbf{if} true \\
  \text{~~~~~~~~}Compare whether this node is ${\cal T}$;\\
  \text{~~~~~~~~}\textbf{if} true\\
  \text{~~~~~~~~~~~~}Remove ${\cal T}$ and forward the packet to next hop with its\\
  \text{~~~~~~~~~~~~~~~~}destination $d$;\\
  \text{~~~~~~~~}\textbf{else} \\
  \text{~~~~~~~~~~~~}Forward the packet to next hop with its destination ${\cal T}$;\\
  \text{~~~~}\textbf{else}\\
  \text{~~~~~~~~}Search its local cache \\
  \text{~~~~~~~~}\textbf{if} an entry $<a,b>$ exists\\
  \text{~~~~~~~~~~~~}\textbf{if} this node and $d$ are at the same side of $ab$\\
  \text{~~~~~~~~~~~~~~~~}Conduct GPSR;\\
  \text{~~~~~~~~~~~~}\textbf{if} this node and $d$ are at opposite sides of $ab$\\
  \text{~~~~~~~~~~~~~~~~}\textbf{if} $d$ is in $ramn$\\
  \text{~~~~~~~~~~~~~~~~~~~~}Write $a$ as tentative target ${\cal T}$ to the packet;\\
  \text{~~~~~~~~~~~~~~~~~~~~}Forward packet to next hop with destination ${\cal T}$;\\
  \text{~~~~~~~~~~~~~~~~}\textbf{if} $d$ is in $nmbt$\\
  \text{~~~~~~~~~~~~~~~~~~~~}Write $b$ as tentative target ${\cal T}$ to the packet;\\
  \text{~~~~~~~~~~~~~~~~~~~~}Forward packet to next hop with destination ${\cal T}$;\\
  \text{~~~~~~~~~~~~~~~~}\textbf{else}\\
  \text{~~~~~~~~~~~~~~~~~~~~}Conduct GPSR;\\
  \text{~~~~~~~~}\textbf{else}\\
  \text{~~~~~~~~~~~~}Conduct GPSR.\\
  
 }

\protect\caption{HDAR Forwarding Algorithm}
\protect\label{forwardfig}
\end{figure}

























 








==> figures/HDAR/introduction.tex <==
\section{Introduction}
\label{intro}


Geographic routing is a simple, scalable  and efficient routing strategy in wireless networks. It has been considered as the most promising 
routing scheme in ad-hoc networks. In such a scheme, the location information for nodes is available 
either through GPS or using virtual coordinates~\cite{ex11}. And it is assumed that each node knows its own location 
and the locations of its neighbors. The source node knows the location of the destination node and encapsulates 
it in each data packet. In the basic greedy forwarding approach, a node sends data packets to one of its neighbors 
who is closest to the destination until the packets reach the destination node. This mechanism can minimize the hops 
from the source to the destination. However, there existing a challenge often faced in geographic greedy routing 
is ``local minimum problem", in which the greedy forwarding process is blocked at a node that does not have a closer 
neighbor to the destination, even though there is a path from the source to destination in the network. The occurrence 
of hole can be caused by many factors in wireless ad hoc networks, such  as the jamming hole incurred by 
jam communication, the sparse deployment, the physical obstacles and power exhaustion~\cite{ex24}.

To overcome the local minimum issue, Greedy Perimeter Stateless Routing (GPSR)~\cite{ex13}, Greedy-Face-Greedy(GFG)~\cite{ex28}, 
and Greedy-Other-Adaptive-Face Routing(GOAFR)~\cite{ex29} are proposed. When a forwarding packet gets stuck at a local 
minimum node, it will start a perimeter routing phase where the packet will be forwarded along the perimeter 
of the hole,  until it reaches a node that can find one of its neighbors that is closer to the destination than 
itself. After that,the forwarding mode returns to greedy. The face routing family schemes can guarantee 
delivery. However,they often cause long detour path in the perimeter routing, although the shorter path exists.

To avoid the long detour path, recent work tries to detect the hole and the nodes located on the hole's boundary 
in advance, then these nodes advertise the hole information to some other nodes~\cite{ex22}~\cite{ex30}. 
So the future routing path can be adaptive in the presence of the hole. 

Our algorithms HDAR in this paper focus on defining and detecting holes in ad hoc network, representing holes and building routes around the holes. The contributions of this paper are threefold.
First, we come up with a heuristic algorithm to detect a hole quickly and easily.
% The hole can be detected in advance. 
And the hole can be identified only by one time calculation. 
%Our hole detecting algorithm results low false negative and low false positive. 
Second, we provide a very concise format to represent the hole. A hole is represented only by a segment.
Third, we develop an approach to make part of the nodes located on the hole's boundary announce to the nodes 
in the vicinity of the hole. 
We found the best tradeoff between the cost of hole information announcement and benefit for future routing. 
Simulation shows that compared with GPSR, HDAR reduces the length of routing path
by 12.4\% and forwarding hops by 13.2\% for all the paths in
tested areas. And the length of long detour paths around the hole can be reduced 61.2\%. 
%only
%38.8\% long and 35.4\% 
The number of hops can be reduced 64.6\% compared with GPSR. Simulation also indicates that the computational complexity of HDAR 
is only 16.6\% that of HAGR.

The rest of the paper is organized as follows. Section~\ref{related}
discusses related work. Section~\ref{Algorithms} proposes a novel method
for detecting holes and presents a new adaptive routing algorithm. We evaluate the
proposed schemes by simulations and describe the performance results in Section~\ref{evaluation}. 
Section~\ref{discussion} further discusses the hole detection and related methods. Section~\ref{conclusion} concludes the paper.
The deduction of the hole announcement size is introduced in the appendix.






==> figures/HDAR/maincontents.tex <==
\input{introduction.tex}
\input{overview.tex}
% \input{shadedarea.tex}
% \input{algorithm.tex}
\input{hdar.tex}
\input{simulation.tex}
\input{discussion.tex}
\input{conclusion.tex}
%\input{appendix.tex}


==> figures/HDAR/overview.tex <==
\section{Related Work}
\label{related}



The first geographic routing protocol is based on simple greedy forwarding. In this approach, 
each node forwards packets to one of its neighbors who is closest to the destination node until 
the packets arrive the destination. This scheme is efficient. However, it fails due to the ``local minimum problem".

To mitigate ``local minimum problem", compass routing~\cite{ex16} was proposed as the first face routing, 
in which the packet is forwarded along the face until greedy is workable in a node. However, 
compass routing cannot guarantee packet delivery in all geographic networks. Several routing 
algorithms in face routing family have been developed. By combining greedy and face routing, Karp and Kung proposed the
Greedy Perimeter Stateless Routing (GPSR) algorithm~\cite{ex13}.
It consists of the greedy forwarding mode and the perimeter forwarding mode, which is applied in the regions where
the greedy forwarding does not work. An enhanced algorithm, called Adaptive Face Routing (AFR), uses an eclipse
to restrict the search area during routing so that in the worst
case, the total routing cost is no worse than a constant factor
of the cost for the optimal route~\cite{ex17}. The latest addition to
the face routing family is Path Vector Face Routing(GPVFR)~\cite{ex18}, which improves
routing efficiency by exploiting local face information.
The protocols in face routing family can avoid the hole. However, they often cause long detour path.


A new idea was proposed recently, which is to detect the hole in advance, then the nodes located 
on the hole advertise the hole information to other nodes. The hole information will benefit nodes who receive it for their future routing. 
Qing gave 
a mathematical definition of hole~\cite{ex22}. He defined a hole to be a simple region enclosed by a polygon 
cycle which contains all the nodes where local minimum can appear. He brought forth the ``get stuck" concept and 
proposed the hole detection mechanism that
once a packet  following geographic greedy forwarding gets stuck at a node, the node must be on the boundary of a hole.
%Based on his hole definition, 
%when a packet gets stuck at a node following geographic greedy forwarding, this node must be 
%a stuck node 
%on the boundary of a hole. By marking all the boundaries of holes, the routes to get 
%stuck packets out of the local minimum can be found.  The stuck node can simply forward the packet 
%to one of its neighbors that shares the same boundary. 
Also related is HAGR~\cite{ex30}. HAGR investigated the 
nodes incident to a close loop in a geographical graph. For a vertex $u$, if the 
angle between two adjacent edges with respect to this vertex is larger than an angle threshold, 
then vertex $u$ considers it is located on a potential hole. To further determine if it is located on a hole, 
$u$ calculates the diameter of the loop. It locates the bisector that equally splits the angle and uses 
it as a reference line. Then node $u$ finds out the leftmost node and the rightmost node furthest from the 
bisector. The distance between the leftmost node and the rightmost node is the diameter of the hole. 
If the diameter is greater than the diameter threshold and the angle is bigger than the angle threshold, 
$u$ is regarded as sitting on a hole. Once a node is detected on  a hole, it advertises the hole information 
to its neighbors. Upon receiving the hole information, its neighbor recalculates the angle and diameter 
based on its location. If both of them are bigger than their thresholds, then the neighbor considers it is 
on a hole and it continues to advertises the hole information, otherwise it stops advertisement. 
Base on the hole detecting, HAGR divides the network plane into three regions, and the nodes in different 
regions conduct different forwarding strategies. The idea of HAGR is novel. However, the hole detecting 
approach is time-consuming since a node has to calculate the values of two metrics. And the hole advertisement is 
expensive because once a node receives the hole information, it has to recalculate two values and 
compare them with their corresponding thresholds. In addition,  the diameter threshold is an absolute value and it has to be adjusted according to 
the nodes' transmission range or the network deployment, otherwise false negative or false positive may occur.  
Moreover, the forwarding strategies are too complicated.







==> figures/HDAR/shadedarea.tex <==
\section{Shaded Area Detection}
\label{shadedarea}
In this section, we describe our method to detect and calculate the shaded areas. We assume that all the ad hoc nodes are distributed 
in a two dimension plane. Every node has the same transmission range. All the nodes are static. 
That is, mobility is not considered.

\subsection{Problem overview}


Fig.~\ref{fig1} indicates two examples of greedy path and detour path caused by a hole. Suppose node $S$ is the source node 
and $D_1$ and $D_2$ are two destination nodes respectively. 
When $S$ intends to send packets to $D_1$, it can find an efficient path by greedy forwarding. 




However, void areas(or holes) may exist in the network plane. A void area is an
area that has no active nodes. A routing path based on
geolocations may be blocked from moving closer to the destination due to the lack of relaying nodes to cross the void.
 In wireless 
ad hoc network, the holes are caused by various reasons~\cite{ex24}. 
For instance, the malicious nodes can jam
the communication to form Jamming Holes or they can
overwhelm regions  by denial of service attacks that cause Black Holes or Worm Holes.
In addition, if the nodes' signal is not long enough to cover everywhere in the network plane, the
Coverage Holes may exist. Moreover, there are Routing Holes. These holes
can be formed either due to voids in nodes deployment or because of failure of nodes due to various reasons such as 
malfunctioning, battery depletion or structure collapse physically destroying the nodes.
When greedy forwarding encounters a hole, it will not be available. For instance, when $S$ intends to send packets to $D_2$, it begins to use greedy forwarding 
mode. When the packets reach node $P$, $P$ is closer to $D_2$ than any of its neighbors but $P$ cannot reach $D_2$ by 
greedy forwarding. 
We say $P$ is a local minimal node. If $P$ changes the forwarding mode to perimeter, the packets will be forwarded along a 
long detour path until the packets arrive B, where the forwarding mode is changed to greedy. The reason that the path is 
detour is that $D_2$ is shaded by the hole but the source doesn't know it. So 
we would like to find the shaded area $T$ in advance and inform this district to $S$. Then $S$ could send the packets 
to the tentative target node $B$ directly if it wants to send packets to $D_2$ in $T$. And then node $B$ relays the packets 
to $D_2$ by greedy forwarding. So the main approach in this paper is that when a source node S sends packets to a destination node, if there is a hole that blocks
the routing path, the source calculates the destination area that is shaded by the hole, then saves the local minimal node
 and a key intermediate node from which the forwarding mode comes back to greedy to its cache. 
 When packets are forwarded via S to any nodes located in the shaded area in the future, S will forward them
to the key intermediate node as tentative target by greedy mode, and then the intermediate node relays to next intermediate node or 
destination node by greedy mode
until the packets arrive the destination. The long detour path can be avoided by this way.

\begin{figure}[!htp]
\begin{center}
\includegraphics[width=6.0cm]{figure1.eps}
\end{center}
\caption{Greedy path and detour path}
\label{fig1}
\end{figure}

There are two problems: one is how to figure out the shaded areas, another is how to find the tentative target nodes?

\subsection{Shaded areas}

%$Definition$: Landmark\\*
We call a node landmark as the following description: Suppose $S$ is a source node and $D$ is a destination node. $S$ is sending packets to $D$ by greedy mode or face mode. 
The packets are forwarded by greedy mode from $S$. Suppose there is a hole $M$ and the packets arrive a local minimal node $P$. 
Then the packets are forwarded by face mode along  the perimeter of $M$. If
there is a node $B$ satisfies: from $B$ to $D$, 
the packets are forwarded only by greedy mode and before B the forwarding mode is perimeter, then we call node $B$ the landmark node from $S$ to $D$.
The landmark looks like the point where the packets escape from the hole's restriction and come back to greedy mode.

The locations of 
the local minimal node $P$ and landmark $B$ must be learned by the source node $S$ to calculate the shaded area. We use three nodes $S$,$B$
and $P$ to represent a shaded destination area. These three nodes indicate the area semi-enclosed by ray $SB$, ray $SP$ and the hole's
perimeter from $B$ to point $F$ which is line $SP$ and the hole's intersection(Fig.~\ref{fig2}).

We add additional fields to a packet's header to let source node S learn $P$ and $B$ when
S sends packets to $D$ in case there is a hole that causes a detour path.
%If the source can learn about that the destination is shaded in case it's hidden behind a hole, the routing path will be shorter since 
%the source would send packets to the landmark. 
Nodes $S$,$D$ and $B${'}$s$ relative locations may vary depending on different hole shapes. So the steps to calculate the 
destination area are slightly different based on their relative locations. 
Basically, there are three types of hole's shapes that may affect how the source calculates the shaded destination areas. 
We distinguish the three types from two aspects, one is the quantitative relationship between  $\angle$ $BDS$ and $\frac{\pi}{2}$, 
another is  whether there is a greedy path from the source to the landmark. 

The first type of hole's shape is as Fig.~\ref{fig2}, where  $\angle$ $BDS$  is less than $\frac{\pi}{2}$ and there is a greedy path  
from $S$ to $B$. The method to find the shaded destination area is straightforward: 
$S$ logically connects $S$ and $P$, suppose $SP$ intersects the hole $M$ at two points and the one other than $P$ is $F$. 
Ray $SF$ extends to an arbitrary point $C$. 
$S$ logically connects $S$ and $B$. Suppose ray $SB$ extends to an arbitrary point $E$.
%Draw line $BE$ in parallel with line $SD$. 
Then the area semi-enclosed by $EB$, the perimeter of $M$ from $B$ to $F$ and $FC$ is the      
shaded destination area $T$. Hence, 
if $S$ wants to send packets to any destination node in $T$, the destination  is hidden behind the hole. To avoid a detour 
path, $S$ sends the packets to $B$ first, and $B$ will then relay them to $D$. Both of the two paths are greedy paths. 


\begin{figure}[!htp]
\begin{center}
\includegraphics[width=8.0cm]{figure2.eps}
\end{center}
\caption{The shaded area when angle BDS is less than $\frac{\pi}{2}$ and path SB is greedy}
%\caption{$\angle $BDS$ \leq$ $\frac{\pi}{2}$ }
%\caption{The shaded area $\frac{\pi}{2}$ }
\label{fig2}
\end{figure}

In scenario 2(Fig.~\ref{fig3}), $\angle$ $BDS$ is less than $\frac{\pi}{2}$.
% while $\angle$ $BSD$ may be greater or than $\frac{\pi}{2}$.
From $S$ to $B$, 
there's no greedy path exists. The steps to find the shaded destination area is the same as scenario one. However, 
to find a routing path in this  circumstance  is different from situation 1. We will discuss it later in this paper.

\begin{figure}[!htp]
\begin{center}
\includegraphics[width=8.0cm]{figure3.eps}
\end{center}
\caption{The shaded area when angle BDS is less than $\frac{\pi}{2}$ and path SB is not greedy}
\label{fig3}
\end{figure}

$\angle$ $BDS$ is greater than $\frac{\pi}{2}$ and there's no greedy path from $S$ to $B$ in the third scenario(Fig.~\ref{fig4})..   
To find the shaded destination areas, $B$ is considered as a tentative destination node, when packets are sent from $S$ to $B$, 
we find another landmark recursively, then we count this landmark as a tentative destination node, and continue to  find landmarks recursively 
until no
 landmark exists. Suppose the last landmark is $B^{'}$, $S$ connects $B^{'}$ and extends it to an arbitrary point $E$.
 Then the area semi-enclosed by $EB^{'}$ , the perimeter of $M$ from $B^{'}$  to $F$ and $FC$  is the shaded destination area $T$.
 %(exclusive $B^{'}$).
 
 
 \begin{figure}[!htp]
\begin{center}
\includegraphics[width=8.0cm]{figure4.eps}
\end{center}
\caption{The shaded area when angle BDS is greater than $\frac{\pi}{2}$ and path SB is not greedy}
\label{fig4}
\end{figure}
 
\begin{comment}
 The steps to find the shaded areas are described in algorithm 1.
In this algorithm, line 5 to line 7 indicates the scenarios of Fig.~\ref{fig2} and Fig.~\ref{fig3}. And line 8 to line 15
illustrates the circumstance in Fig.~\ref{fig4}. This algorithm illustrates the primary method
 to figure out a shaded destination area.  However, a node may generate multiple $<$ $shaded\_des\_area$, $landmark$ $>$
 entries which may share areas or landmarks. We will merge them to reduce spaces and provide efficient lookup. 
 So $BE$ or  $FC$ may not be the boundary line of a shaded area associated with landmark $B$ after the merge. 
 This will be discussed later in this paper.
\end{comment} 
 
Shaded Area Calculation Algorithm in Fig.~\ref{algfig}.
describes how the current node S calculates the shaded area in case there is a hole blocking packets forwarding.
Suppose the lanbdmark node is B. If $\angle$ $BDS$ is less than $\frac{\pi}{2}$, we extend line SB and line SP to E and C
respectively(Fig.~\ref{fig2}), then the area enclosed by EB, the hole perimeter from E to F and FC is shaded area.
However, S does not know the hole's concrete location, so we extend this theoretical area to EBPC as the shaded area since no active nodes in the hole.
If $\angle$ $BDS$ is greater than $\frac{\pi}{2}$, that means we have to recursively find the landmark which is nearest to the source and then
figure out the shaded area(Fig.~\ref{fig4}).This algorithm illustrates the primary method
 to figure out a shaded destination area.  However, a node may generate multiple $<$ $shaded\_des\_area$, $landmark$ $>$
 entries which may share areas or landmarks. We will merge them to reduce spaces and provide efficient lookup. 
 So $BE$ or  $FC$ may not be the boundary line of a shaded area associated with landmark $B$ after the merge. 
 This will be discussed later in this paper.
 \\
 

 


%oribigal algorithm, looks like a global one.
\begin{comment}
\begin{algorithm}[bt]
\begin{algorithmic}[1]
\caption{{\em  Shaded Destination Area}}
\label{algorithm1}
\STATE Logically connects $S$ and $P$. suppose $SP$ intersects the hole $M$ at two points, the one other than $P$ is $F$. $SF$
extends to an arbitrary point $C$.
\STATE $S$ sends packets to $D$ by greedy or face mode 
\IF{there is a landmark node $B$ in the routing path}
\STATE{$D$ informs  $B${'}$s$ location to $S$}
\IF{$\angle $BDS$ \leq$ $\frac{\pi}{2}$ }
\STATE{Connect $SB$ and extends it to $E$}
\STATE{the area semi-enclosed by $EB$, the perimeter of $M$ from $B$ to $F$ and $FC$ is the shaded destination area $T$}
\ELSE 
\STATE{$D^{'} \leftarrow B$}
\STATE{$D^{'}$ informs $S$ to send packets to $D^{'}$}
\WHILE{a landmark node $B^{'}$  from S to $D^{'}$  exists}
\STATE{$D^{'} \leftarrow B^{'}$}
\STATE{$D^{'}$ informs $S$ to send packets to $D^{'}$}
\ENDWHILE
\STATE{Connect $SB^{'}$ and extends it to $E$}
\STATE{the area semi-enclosed by $EB^{'}$, the perimeter of $M$ from $B^{'}$ to $F$ and $FC$ is the shaded destination area $T$}
\ENDIF
\ENDIF
\end{algorithmic}
\end{algorithm}
\end{comment}


\begin{figure}[hbt]
\baselineskip=10.2pt

{\scriptsize
  \noindent\underline{\bf S initiates sending a packet to destination node} \\
  \text{~~~~}S forwards the packet by greedy or face mode; \\
  %\text{~~~~~~~~}hdjshdjhd\\
  \\
  
  \noindent\underline{\bf When the destination node receives the data packet from S} \\
  \text{~~~~}Ckecks the packet's header; \\
  \text{~~~~}\textbf{if} local minimal P and landmark B exists \\
  \text{~~~~~~~~}Sends a $landmark\_exist\_msg$ to S containing the locations of B and P;\\ 
  \text{~~~~}\textbf{else}
  \text{~~~~}Sends ACK to S;
  \\
  
  \noindent\underline{\bf When S receives $landmark\_exist\_msg$} \\
  \text{~~~~}Marks the message sender as node D; \\
  \text{~~~~}\textbf{if} it doesn't save any local minimal node \\
  \text{~~~~~~~~}Saves P;\\
  \text{~~~~}Compares $\angle$ $BDS$ and $\frac{\pi}{2}$; \\
  \text{~~~~}\textbf{if} $\angle $BDS$ \leq$ $\frac{\pi}{2}$ \\
  \text{~~~~~~~~}Extends line SB to any point E;\\
  \text{~~~~~~~~}Extends line SP to any point C;\\
  \text{~~~~~~~~}Consider EBPC as shaded area;\\
  \text{~~~~}\textbf{else}\\
  \text{~~~~~~~~}Counts B as the packet's destination node in its header;\\
  \text{~~~~~~~~}Sends the data packet according to its destination in its header;\\
    
  
}

\protect\caption{Shaded Area Calculation Algorithm}
\protect\label{algfig}
\end{figure}


\begin{comment}
--When S initiates to send a data packet to destination node extracted from the packet's header
       S forwards the packet by greedy or face mode
       
--When the destination node receives the data packet from S
       Ckecks the packet's header
       \textbf{if} landmark B exists(P must exist)
            Sends a landmark_exist_msg to S containing B's location and P's location
       \textbf{else} sends ACK to S
                     
            
--When S receives landmark_exist_msg                  
       Marks the message sender as node D
       Compares \angle BDS and pi/2
          \textbf{if} <=pi/2
               Extends line SB to any point E
               Extends line SP to any point C
               Considers EBPC as shaded area
          \textbf{else}
               Counts B as the packet's destination node in its header
               Sends the data packet according to its destination in its header
               
    
              
          
\end{comment}

 


















==> figures/HDAR/simulation.tex <==
\section{Performance Evaluation}
\label{evaluation}



Our simulations were performed by using the easim3D wireless network simulator~\cite{ex27}, 
which is to simulate IEEE 802.11 radios and typically for location based routing algorithms. We
use a noiseless immobile radio network environment. In the
simulations, nodes with a transmission radius of 20 meters
are deployed in an interest area of 400mX400m.


\begin{comment}
%The first part is to compare the computational 
%complexity of HARG and our algorithm HDAR. 
\end{comment}
We generated networks with the number of nodes varied 
from 50 to 300. For a certain number, 50 networks were generated randomly. And the 
holes were generated automatically in each network. 

Our experiments include two parts. 
The first part is to compare GPSR and HDAR.
\begin{comment}
For each network, we first 
implemented HARG. Since HARG has not been simulated yet in the paper~\cite{ex30}, 
we select $5\pi/6$ as the hole detection threshold and 60 meters as the diameter threshold. 
In both HARG and HDAR, we investigated the number of computation times of hole detection. 
In HDAR, the hole information is only calculated by a few nodes located on the hole and other 
nodes are advertised the hole. While in HARG, a number of nodes have to calculate to determine 
the existing of a hole. The numbers of calculation times were reported to evaluate the computational complexity. 
Fig.~\ref{complexityfig} illustrates that the computational complexity of HDAR is much less than that of HARG.
\begin{figure}
\begin{center}
\includegraphics[width=7.0cm]{comtimes.eps}
\end{center}
\vspace{-0.1in}
\caption{The computational complexity.}
\label{complexityfig}
\end{figure}
\end{comment}
%We compare HDAR and GPSR in the second part of our experimentation. 
We implemented GPSR that is 
previously implemented by Karp and Kung~\cite{ex13}. 
%in the same networks generated in part 1. 
We compare GPSR and HDAR by two metrics, the length of routing paths 
and the number of hops.

Fig.~\ref{avepathfig} indicates the average length of paths when the number of nodes changes from 50 to 300.
The average length in HDAR is 12.4\% shorter than that of GPSR.
Fig.~\ref{hopsfig} shows the average number of hops in HDAR is 13.2\% less than that of GPSR.

\begin{figure}
\begin{center}
\includegraphics[width=7.0cm]{avepath.eps}
\end{center}
\vspace{-0.1in}
\caption{The average length of paths.}
\label{avepathfig}
\end{figure}

\begin{figure}
\begin{center}
\includegraphics[width=7.0cm]{avehops.eps}
\end{center}
\vspace{-0.1in}
\caption{The average number of hops.}
\label{hopsfig}
\end{figure}

In the statistics results of  Fig.~\ref{avepathfig} and Fig.~\ref{hopsfig}, the results report both the greedy path and 
the path in the vicinity of holes. So HDAR's effect to the path near the holes cannot be emphasized. To demonstrate HDAR's effect,
we tipically marked the paths that benefit from the hole information as ``hole paths" and recorded the pairs of source and destination nodes.
We also investigated the paths generated by GPSR with the same pairs of source and
destination nodes. Then we compared the paths benefit from hole information in HDAR
with the paths derived from GPSR.
%Then for the same pairs of source and destination nodes, we compare HDAR with GPSR
%still from the length of paths and number of hops perspectives.


The performance of HDAR and GPSR to the hole paths are reported in Fig.~\ref{holepathfig} and  Fig.~\ref{holehopfig}.
HDAR has much shorter paths and fewer hops compared with GPSR.
For the hole path paths, the average length of HDAR is only 38.8\% that of GPSR and the number of hops is only 35.4\%.
The two figures indicate that that HDAR reduces the long detour paths around holes significantly.







\begin{figure}
\begin{center}
\includegraphics[width=7.0cm]{holepath.eps}
\end{center}
\vspace{-0.1in}
\caption{The average length of hole paths.}
\label{holepathfig}
\end{figure}

\begin{figure}
\begin{center}
\includegraphics[width=7.0cm]{holehop.eps}
\end{center}
\vspace{-0.1in}
\caption{The average number of hops of hole paths.}
\label{holehopfig}
\end{figure}




The second part is to compare the computational 
complexity of HARG and our algorithm HDAR. 
We used the same networks in part 1.
% we first implemented HARG. 
Since HARG has not been simulated yet in the paper~\cite{ex30}, 
we selected $5\pi/6$ as the hole detection threshold and 60 meters as the diameter threshold. 
In both HARG and HDAR, we investigated the number of computation times of hole detection. 
In HDAR, the hole information is only calculated by a few nodes located on the hole and other 
nodes are advertised the hole information. While in HARG, a number of nodes have to calculate to determine 
the existing of a hole. The numbers of calculation times were reported to evaluate the computational complexity. 
Fig.~\ref{complexityfig} illustrates that the computational complexity of HDAR is much less than that of HARG.
\begin{figure}
\begin{center}
\includegraphics[width=7.0cm]{comtimes.eps}
\end{center}
\vspace{-0.1in}
\caption{The computational complexity.}
\label{complexityfig}
\end{figure}




















==> figures/SFBB/Makefile <==
#---------------------------------------------------------------------------
#  Makefile for latex documents with enhancements to make notes and slides.
#  You must use my macros.tex file if you want to utilize the enhancements.
#     Copyright (c) Jim Griffioen, 1997
#
#  Targets include:
#       init:   type 'make init' before doing anything
#	config:	reset the configuration to "student bw slides"
#       sg:     change the group ownership on RCS files (use after running ci)
#	all:	make the dvi file
#	ps:	make postscript file
#	pdf:	make pdf file
#	html:	make an html version (broken down by subsection)
#       html-nosplit: same as html, but create a single html file
#	bib:	make the bibliography and then .dvi file
#	gv:	make postscript file and ghostview it
#	acro:	make pdf file and acroread it
#	x:	run xdvi on the .dvi file
#	me:	configure for me
#	student: configure for student
#	notes:	configure for notes
#	slides:	configure for slides 
#       bw:	configure for black and white output
#	color:	configure for color output
#	portrait: configure for portrait orientation
#	landscape: configure for landscape orientation
#	2up:	make postscipt with 2 slides per page (plus note area)
#	4up:	make postscipt with 4 slides per page (no note area)
#	webnotes: make tar file with .ps, 2up, 4up, and html for class web page
#	clean:	remove all generated files
#	cleanlatex:  only remove the .dvi, .aux, .bbl, .blg, .log files
#	cleanhtml:  remove the generated html directory
#---------------------------------------------------------------------------

# Define the LaTex file filenames
PAPER=  main

ALLTEXFILES=	${PAPER}.tex \
		maincontents.tex \
		abstract.tex \
		conclusion.tex \
		definition.tex \
		evaluation.tex \
		introduction.tex \
		sfbb.tex \
		overview.tex \
		

# Name of figure files - these must be generated files
# because 'make clean' will delete them.
# Do not include non-generated figs here.
GENERATED_FIGS= 

# Names of xfig files used to generate the above .ps files
# Note, this variable is only used to checkout the xfig files
# from the RCS directory
FIG_FILES= 

# Image files (e.g., GIFs or JPGs) to be used directly in HTML docs
IMAGES=	

# Movie files (e.g., Quicktime, AVI, MPEGS) to be used directly in HTML docs
ANIMS=	

# Name of figure files that are not generated
OTHER_FIGS=	

# Name of the Unix group to set the RCS file ownership to
GROUP= netfac

#---------------------------------------------------------------------------
# You should not need to modify anything below this point
#---------------------------------------------------------------------------

#---------------------------------------------------------------------------
# Makefile code needed by all makefiles
#
# This section assumes that the following makefile variables have already
# been defined above
#    PAPER=
#    ALLTEXFILES=
#    GENERATED_FIGS=
#    FIG_FILES=
#    IMAGES=
#    ANIMS=	
#    OTHER_FIGS=
#    GROUP=
#---------------------------------------------------------------------------

# Set TEXINPUTS to find my tex macrosfiles
TEXINPUTS= .:../macros:../../macros:/homes/griff/lib/macros:

#---------------------------------------------------------------------------
# Define the names of the programs to use
#---------------------------------------------------------------------------

# Programs
GRAP=		grap
TPIC=		tpic
FIG2PS=		fig2dev -Lps -m 0.7
FIG2PIC=	fig2dev -Ltpic -m 0.7
LATEX=		latex
BIBTEX=		bibtex
DVI_TO_PS=	dvips -Pdownload35 -t letter
TBL=		tbl
XDVI=		xdvi
RM=		rm
GREP=		grep
GS=		gv
PDFVIEWER=	acroread
LPR=		lpr
CONVERT=	convert
L2H=		latex2html
PS2PDF=		ps2pdf -dPDFSETTINGS=/printer -dCompatibilityLevel=1.3 -dMaxSubsetPct=100 -dSubsetFonts=true -dEmbedAllFonts=true


# name of the config file - defined in macros.tex
CONFIGFILE= config.tex

# name of the latex2html init file
LATEX2HTML_INIT= /homes/griff/.latex2html_init

# printer to use
PRINTER= lp
PRINTER_OPT= -P${PRINTER}


#---------------------------------------------------------------------------
# Rules for Making
#---------------------------------------------------------------------------
.SUFFIXES: .tex .dvi .fig .ps .detex .g .tbl .pic .gif .jpg .bmp .tif .tiff .tex,v .fig,v .pdf
.tex.detex: 	; $(DETEX) $*.tex > $*.detex
.tex.dvi: 	; $(LATEX) $* 
.fig.pic:	; $(FIG2PIC) -Ltpic $<  |  $(GREP) -v ".baseline" > $*.pic
.fig.ps:	; $(FIG2PS) -Lps $< $*.ps
.gif.ps:	; $(CONVERT) $*.gif $*.ps
.jpg.ps:	; $(CONVERT) $*.jpg $*.ps
.bmp.ps:	; $(CONVERT) $*.bmp $*.ps
.tif.ps:	; $(CONVERT) $*.tif $*.ps
.tiff.ps:	; $(CONVERT) $*.tiff $*.ps
.pic.tex:	; $(TPIC) $*.pic > $*.tex
.g.pic:		; $(GRAP) $*.g | $(GREP) -v ".lf" > $*.pic
.g.tex:		; $(GRAP) $*.g | $(GREP) -v ".lf" > $*.pic ; $(TPIC) $*.pic
.tbl.pic:	; $(TBL) $*.tbl > $*.pic
.dvi.ps:	; $(DVI_TO_PS) -o $*.ps $*.dvi 
.ps.pdf:	; $(PS2PDF) $*.ps $*.pdf
.tex,v.tex:	; co $*.tex
.fig,v.fig:	; co $*.fig
.jpg,v.jpg:	; co $*.jpg
.gif,v.gif:	; co $*.gif
.bmp,v.bmp:	; co $*.bmp
.tiff,v.tiff:	; co $*.tiff
.tif,v.tif:	; co $*.tif

# Different Make options

all: ${PAPER}.dvi ${PAPER}.ps

${PAPER}.dvi: ${ALLTEXFILES} ${FIG_FILES} ${IMAGES} ${ANIMS} ${GENERATED_FIGS}
	$(LATEX) ${PAPER}

setgrp: 
	chgrp $(GROUP) RCS/*
sg: 
	chgrp $(GROUP) RCS/*

generated_figs: ${GENERATED_FIGS}

print: ${PAPER}.dvi

ps: ${PAPER}.ps

pdf: ${PAPER}.pdf

${PAPER}.ps: ${PAPER}.dvi

${PAPER}.pdf: ${PAPER}.ps

x: ${PAPER}.dvi
	$(XDVI) ${PAPER}.dvi &

gv: ps
	$(GS) ${PAPER}.ps &

gs: ps
	$(GS) ${PAPER}.ps &

acro: pdf
	$(PDFVIEWER) ${PAPER}.pdf &

bib: ${ALLTEXFILES} ${PAPER}.ps
	echo "#!/bin/sh" > .makbib
	echo $(LATEX) ${PAPER} >> .makbib
	echo $(BIBTEX) ${PAPER} >> .makbib
	echo $(LATEX) ${PAPER} >> .makbib
	echo $(LATEX) ${PAPER} >> .makbib
	chmod a+x .makbib
	./.makbib
	rm .makbib

me:
	cat $(CONFIGFILE) | sed "s/studenttrue/studentfalse/" > .tmp
	cp .tmp $(CONFIGFILE); rm .tmp
	cat $(CONFIGFILE) | sed "s/instructorfalse/instructortrue/" > .tmp
	cp .tmp $(CONFIGFILE); rm .tmp
instructor:
	cat $(CONFIGFILE) | sed "s/studenttrue/studentfalse/" > .tmp
	cp .tmp $(CONFIGFILE); rm .tmp
	cat $(CONFIGFILE) | sed "s/instructorfalse/instructortrue/" > .tmp
	cp .tmp $(CONFIGFILE); rm .tmp
student:
	cat $(CONFIGFILE) | sed "s/studentfalse/studenttrue/" > .tmp
	cp .tmp $(CONFIGFILE); rm .tmp
	cat $(CONFIGFILE) | sed "s/instructortrue/instructorfalse/" > .tmp
	cp .tmp $(CONFIGFILE); rm .tmp
slides:
	cat $(CONFIGFILE) | sed "s/slidesfalse/slidestrue/" > .tmp
	cp .tmp $(CONFIGFILE); rm .tmp
	cat $(CONFIGFILE) | sed "s/notestrue/notesfalse/" > .tmp
	cp .tmp $(CONFIGFILE); rm .tmp
notes:
	cat $(CONFIGFILE) | sed "s/slidestrue/slidesfalse/" > .tmp
	cp .tmp $(CONFIGFILE); rm .tmp
	cat $(CONFIGFILE) | sed "s/notesfalse/notestrue/" > .tmp
	cp .tmp $(CONFIGFILE); rm .tmp
color:
	cat $(CONFIGFILE) | sed "s/wantcolorfalse/wantcolortrue/" > .tmp
	cp .tmp $(CONFIGFILE); rm .tmp
bw:
	cat $(CONFIGFILE) | sed "s/wantcolortrue/wantcolorfalse/" > .tmp
	cp .tmp $(CONFIGFILE); rm .tmp
portrait:
	cat $(CONFIGFILE) | sed "s/landscapetrue/landscapefalse/" > .tmp
	cp .tmp $(CONFIGFILE); rm .tmp
landscape:
	cat $(CONFIGFILE) | sed "s/landscapefalse/landscapetrue/" > .tmp
	cp .tmp $(CONFIGFILE); rm .tmp
init:	config
config:
	/bin/echo '\\slidestrue' > $(CONFIGFILE)
	/bin/echo '\\notesfalse' >> $(CONFIGFILE)
	/bin/echo '\\instructorfalse' >> $(CONFIGFILE)
	/bin/echo '\\studenttrue' >> $(CONFIGFILE)
	/bin/echo '\\wantcolortrue' >> $(CONFIGFILE)
	/bin/echo '\\landscapefalse' >> $(CONFIGFILE)

html-split: $(PAPER).dvi
	$(L2H) -split 8 -bottom_navigation -info "" -local_icons \
	-init_file $(LATEX2HTML_INIT) $(PAPER).tex
	@echo copying $(IMAGES) $(ANIMS) into the $(PAPER) directory
	cp $(IMAGES) $(ANIMS) $(PAPER)

html: $(PAPER).dvi
	$(L2H) -split 0 -no_navigation -info "" -local_icons \
	-init_file $(LATEX2HTML_INIT) $(PAPER).tex
	@echo copying $(IMAGES) $(ANIMS) into the $(PAPER) directory
	cp $(IMAGES) $(ANIMS) $(PAPER)

html-nosplit: $(PAPER).dvi
	$(L2H) -split 0 -no_navigation -info "" -local_icons \
	-init_file $(LATEX2HTML_INIT) $(PAPER).tex
	@echo copying $(IMAGES) $(ANIMS) into the $(PAPER) directory
	cp $(IMAGES) $(ANIMS) $(PAPER)

html-noimages: $(PAPER).dvi
	$(L2H) -split 0 -no_images -no_navigation -info "" $(PAPER).tex
	@echo copying $(IMAGES) $(ANIMS) into the $(PAPER) directory
	cp $(IMAGES) $(ANIMS) $(PAPER)

htmlln:
	ln -s /homes/griff/lib/macros/html.sty.foremergencies html.sty

2up: ps
	2up -p${PAPER}-2pp.ps ${PAPER}.ps

4up: ps
	mpage -P -4 ${PAPER}.ps > ${PAPER}-4pp.ps

webnotes: 2up 4up html tar

tar:
	tar -vcf - ${PAPER}.ps ${PAPER}-2pp.ps ${PAPER}-4pp.ps ${PAPER} \
	| gzip > webnotes.tgz

clean: cleanlatex cleanfigs cleanps cleanhtml cleanpdf

cleanlatex:
	$(RM) -f *.aux *.bbl *.blg *.log *.dvi

cleanhtml:
	$(RM) -rf ${PAPER}

cleanfigs:
	$(RM) -f ${GENERATED_FIGS}

cleanps:
	$(RM) -f ${PAPER}.ps

cleanpdf:
	$(RM) -f ${PAPER}.pdf

ppp5:
	rsh ppp5 rm pap.ps pap.ps.gz
	cat ${PAPER}.ps | gzip > pap.ps.gz
	rcp pap.ps.gz ppp5:
	rsh ppp5 gunzip pap.ps.gz
	rm pap.ps.gz

ppp6:
	rsh ppp6 rm pap.ps pap.ps.gz
	cat ${PAPER}.ps | gzip > pap.ps.gz
	rcp pap.ps.gz ppp6:
	rsh ppp6 gunzip pap.ps.gz
	rm pap.ps.gz

ppp9:
	rsh 204.198.76.89 rm pap.ps pap.ps.gz
	cat ${PAPER}.ps | gzip > pap.ps.gz
	rcp pap.ps.gz 204.198.76.89:
	rsh 204.198.76.89 gunzip pap.ps.gz
	rm pap.ps.gz



==> figures/SFBB/conclusion.tex <==
\section{Conclusion}
\label{conclusion}

In this paper, we presented a new message broadcasting algorithm for vehicular networks.
In this algorithm, a message sender can select the best node among its neighbors that
re-broadcast the message fastest to other nodes. 
% The novelty of the approach is that each 
Each node only
keeps values of two parameters to record its moving trend. 
Together with the current velocity of each node, we can determine which node is the best candidate.
% Then the moving trend is used to select the best re-broadcasting node.
The simulations demonstrate that our approach can improve 
the delivery ratio and decrease the end-to-end delay over traditional farthest distance based algorithms.


==> figures/SFBB/definition.tex <==
\newcommand{\bibdir}{./}

\newcommand{\msgrange}{potential range}
\newcommand{\msgranges}{\msgrange s}
\newcommand{\closestneighbors}{$m$-width neighborhood}

\newcommand{\newunstruct}{new unstructured}



==> figures/SFBB/introduction.tex <==
\section{Introduction}
\label{intro}

Recent advances in wireless technologies have made Inter-Vehicle Communications possible 
in mobile Ad-Hoc networks (MANET), thus generating a new type of mobile network known as
Vehicular Ad-Hoc Network (VANET)~\cite{ex14}~\cite{ex24}. VANET has attracted considerable attentions from both the research community and the automotive industry. Many automobile manufacturers have started
planning to build communication devices into their vehicles for purposes of security, convenience and comfort. 
%In addition, the increasing importance of VANET has been recognized
%by the governmental organizations. The Federal Communications Commission (FCC) has allocated particular spectrum for Inter-Vehicle Communications.
With the development of VANETs, many attractive applications have emerged. 
On-board active systems can assist the drivers in avoiding collisions~\cite{ex16}. 
Safety systems can intelligently
disseminate road information~\cite{ex22}~\cite{ex25}, such as accidents, 
real-time traffic congestion, or condition of the road surface. 
Broadcasting schemes can also inform other vehicles of
approaching of police vehicles so that they yield to police vehicles~\cite{ex15}.


Message dissemination is essential in support of the applications of VANET. Researchers are developing broadcasting approaches to disseminate messages to other vehicles. 
The design of effective
vehicular broadcasting approaches poses a number of challenges.  Similar to MANET, VANET has no fixed infrastructure and instead relies on ordinary nodes to perform routing of messages. 
However, VANETs behave in different ways than traditional MANETs. The mobility constraints and high dynamic are unique characteristics of VANETs. 
Velocities are also restricted because of speed limits, traffic control mechanisms such as stop sign and traffic light, and scenarios of the road.
Furthermore, VANETs encounter
a major routing issue, i.e., the broadcast storm problem. The broadcast storm problem
occurs when mobile nodes send messages by flooding, causing frequent link layer contention with other nearby broadcasting
nodes and resulting in packet loss due to collisions.
Therefore, it is extremely difficult to design a sound message broadcasting approach, especially the one  that can
broadcast messages to other vehicles as fast as possible.

Current approaches focus on employing distance-based mechanisms. In these schemes, the sender node tries to select the farthest node in the broadcasting direction and assign it the duty of forwarding messages. 
However, these approaches may not select the best candidate that can forward the message to other nodes fastest.
In this paper, we develop
a statistical filtering based broadcasting algorithm. In this algorithm, each node maintains the acceleration and the variance of acceleration that can represent its historical mobility status. In addition,
each node can predict its future mobility trend by considering the two parameters and its current velocity. In the broadcasting process, the sender disseminates a message to all its neighbors in the broadcasting direction. Then it selects the fastest candidate based on considering its neighbors' future mobility and then designates this candidate to re-broadcast the message.
%The best re-broadcasting node can be selected because the metric to select the best node is the nodes' future mobilities.
Because each node only needs to maintain two parameters,    
the overhead  is low. Our simulation results indicate that  our approach can significantly decrease the end-to-end delay and improve
the message delivery ratio, compared with existing approaches.

The rest of the paper is organized as follows.
Section~\ref{related} discusses the related research on this topic. Section~\ref{sfbb} proposes a novel method to broadcast messages to other vehicles as fast as possible.
We evaluate the proposed schemes by simulations and describe the performance results
in Section~\ref{evaluation}.
Section~\ref{conclusion} concludes the paper.




==> figures/SFBB/maincontents.tex <==
\input{introduction.tex}
\input{overview.tex}
% \input{shadedarea.tex}
% \input{algorithm.tex}
\input{sfbb.tex}
\input{simulation.tex}
\input{conclusion.tex}
%\newpage


==> figures/SFBB/overview.tex <==
\section{Related Work}
\label{related}

This section reviews the work on the message broadcast protocols of Vehicular Networks.
Unlike other format of MANETs, applications developed for VANET have a very specific and clear goal of providing
an intelligent and safe transport system. Emergency warning for public safety is one of many applications that is
highly time-critical and requires a more intelligent broadcast mechanism than just blind flooding.
In~\cite{ex3}, the authors proposed a spatially aware packet routing algorithm to disseminate the message in VANETs.
This algorithm predicts the permanent topology holes. Then, the geographic forwarding is conducted
when the messages are disseminated to other nodes. This approach guarantees that the message will be broadcast to other nodes.
However, it costs too
much because the void areas need to be detected ahead. In addition, the location may change frequently in the VANET. Thus the scenario at a particular moment
is not the same as other time.

A. Amoroso et al proposed a broadcasting algorithm for VANET called FROV~\cite{ex4}.
% ``The Farther Relay and Oracle for VANET''~\cite {ex4}.
This
algorithm is applied in the scenario that cars have heterogeneous transmission ranges. In addition, the transmission of a car can vary while traveling, due to
changes of environmental conditions, such as the humidity of the air, rain, snow and fog. Moreover, topological conditions, such as tunnels, sharp curves, surrounding trees and
buildings, could further influence transmission ranges. The main idea of FROV is 
that the node selected to re-broadcast a message is the one whose re-transmission range spans further than
other nodes. To accomplish this task, FROV considers both
the position and the transmission range, in the direction of
the broadcast, for all the receivers of a message. This algorithm can handle the scenarios with extreme weather or poor conditions, but it does not
consider the mobility status of the vehicles that is essential in VANETs.

A multi-hop broadcast protocol for inter-vehicle communication was proposed in~\cite{ex5}.
This protocol assigns the duty of
forwarding and acknowledging the broadcast packet to only
one vehicle by dividing the road portion inside the transmission range into segments and choosing the vehicle in the
farthest non-empty segment without apriori topology information. When there is an intersection in the path of the
message dissemination, new directional broadcasts are initiated by the repeaters located at the intersections.
This protocol only considers the longest distance factor when selecting the best re-broadcasting node.

An approach that considers mobilities of vehicles was proposed in~\cite{ex6}. In this algorithm, vehicles are divided into several
clusters. Each cluster header maintains the moving status and density of the vehicles in its cluster.
This approach takes mobility into consideration, but it is very difficult to maintain
clusters in VANETs.

%Towards Efficient Routing in Vehicular Ad Hoc Networks.













==> figures/SFBB/sfbb.tex <==
%%%% note:
%   recursion discussed in ITGR routing section, may need a graph
%   combining entries in separate section one graph should be enough
%%%%%

\section{Kalman Filtering Based Broadcasting Protocol}
\label{sfbb}

\subsection{The Basic Idea}
% \subsection{Problem overview}

We start this section with a simple example to illustrate the basic idea of our approach.
% In this section, we describe our method to detect and calculate the shaded areas.
We assume that all the vehicles (nodes) are distributed in a two dimensional space and they are in the moving status.
% Every node has the same transmission range.
Each node has the same transmission range. In addition, errors of measurement for the mobility exist because of
environmental conditions~\cite{ex4}.

\begin{figure}[!htp]
\begin{center}
\includegraphics[width=8.0cm]{car1.eps}
\end{center}
\caption{The basic broadcasting scenario}
\label{fig1}
\end{figure}

Fig.~\ref{fig1} gives an example to show how the sender
$A$ should select one of its neighbors to re-broadcast its message.
After node $A$ broadcasts the message to all of its neighbors in the broadcasting direction,
$A$'s neighbors $C_1$, $C_2$ and $C_3$ receive this message. Node $A$ has to select one of them
to re-broadcast the message.
A simple strategy will let $A$ select the one that is the farthest away from $A$ in the broadcasting direction.
In this case, $A$ will select $C_1$.
However, this may not necessarily be the best choice.

% Let us assume that node $C_1$ is slowing down.

Let us assume that node $C_1$ is moving at a much lower speed than $C_2$ and $C_3$.
Further we assume the historical velocities up to this moment of
node $C_2$ are [..., 50, 55, 59, 63] (miles/hour), and the velocities of node $C_3$ are [..., 75, 71, 66, 64].
Our goal is to select a node that can re-broadcast the message fastest to other nodes.
Considering that $C_2$ and $C_3$ are moving much faster thatn $C_1$, they are obviously
better choices for carrying the message farther down the broadcast direction.
If we only consider the current speed, $A$ should choose $C_3$.
However, we want to select the one that can get out of the transmission range of $A$ and conduct the re-broadcasting first.
This can achieve the goal of the fastest re-broadcast of the message.
We can predict future velocities of these nodes based on their historical and current velocities, and then figure out which node is the first one that will get out of
$A$'s range. In this example, our strategy will let $A$ choose $C_2$.

\begin{comment}
Fig.~\ref{fig1} gives an example in which
$A$ is the message sender. Node $A$ broadcasts the message to all of its neighbors in the broadcasting direction.
$A's$ neighbors $C_1$, $C_2$ and $C_3$ receive this message. Then, $A$ will select one of them to re-broadcast the
messages. If $A$ selects the one that is the farthest away from $A$ in the broadcasting direction, $C_1$ is the option.
Now we assume that node $C_1$ is slowing down.
Considering the scope of coverage of re-broadcast, $C_2$ or $C_3$ are better choices and should be selected.
We assume the historical velocities up to this moment of
node $C_2$ are [...50,55,59,63] (miles/hour), and the velocities of node $C_3$ are [...75,71,66,64]. If we simply select the faster one, $C_3$ is
the choice. However, we want to select the one who can get out of the transmission range of $A$ and then conduct the re-broadcasting first.
We would compute the velocities of these nodes based on their historical and current velocities, and then figure out which one is the first one that will get out of
$A$'s range. In this example, the best choice should be $C_2$.
\end{comment}


\subsection{Kalman Filtering Based Mechanism}
The transmission range of the wireless network for vehicles
is normally 300-400 meters long. It is much longer than the width of the road containing  multiple lanes.
Thus we use a line to represent the road as in Fig.~\ref{fig2}. Here $l$ is a partial arc of the transmission range crossing the road. In addition, point $P$ is the intersection
of $l$ and the road.

\begin{figure}[!htp]
\begin{center}
\includegraphics[width=8.0cm]{car22.eps}
\end{center}
\caption{Simplified basic broadcasting scenario}
\label{fig2}
\end{figure}


We need to compute which node is the first one that can get out of $A$'s range.
The moving trend obviously must be considered.
%The naive method to find the moving trend is to let each node
%save all its history and current velocities, then each node can represent its moving trend by curve-fitting approach that approximates its mobility trend. Apparently, this method costs too much.
We come up with a model based on Kalman Filtering method~\cite{ex10}. In this model, each node only needs to maintain two parameters, its potential acceleration and
variance of acceleration, to represent its mobility trend. Then its future velocity can be computed.
Thus, node $A$ can figure out the best node to be assigned to conduct the re-broadcasting subsequently.


We observe the discrete moving status with every period $\Delta$$t$. Suppose we are investigating the nodes at current time $k$.
Node $A$ would like to find the node that will reach $P$ first and assign it as the re-broadcasting node.
We mark the transmission range of A as $R$, the velocity of node $C_i$ measured at time $k$ as $v_{i_k}$, and
%We would like to compute $c_i$'s potential ability about how fast it can get out of
 %A's range. We estimate $v_{ik+1}$ as $c_i$'s potential ability.
  the distance from A to $C_i$ as $|AC_i|$. Then the time to
reach $P$ is $T_i=(R-|AC_i|)/$$|$$\hat{v_{i_k}}-v_A|$. Here $\hat{v_{i_k}}$ is the predicted velocity of $C_i$ at time $k$.
The prediction is based on considering both $C_i$'s historical and current mobility status. In our approach,
 we predict $C_i$'s velocity for time $k+1$ to compute $T_i$.
 Once we know each $\hat{v_{i_k}}$, we will figure out the node
 with the smallest $T_i$. So the task is to compute $\hat{v_{i_k}}$. % which will be achieved by predicting the velocity of time $k+1$ at time $k$.
%The prediction of its velocity of time $k+1$ is important. For example, if two node $c_1$ and $c_2$ have the history velocities $[50,55,59,63]$
 %and $[76,73,66,63]$ respectively, we predict that $c_1$ will be faster than  $c_2$ at next time by their moving trends.
 %Because the node $c_i$ periodically measures and records its velocity every time slot $\Delta$$t$,

 The naive method of predicting the velocity at time $k+1$ is as follows. Let node $C_i$ save
all its historical and current (time $k$) velocities $v_{i_0}$, $v_{i_1}$, ...,$v_{i_k}$.
Then it can predict its velocity for time $k+1$ by the curve-fitting method that approximates
its moving trend. The problem with this method is that it costs too much. So we devise a model based on stochastic
filtering approach, particularly, Kalman Filtering method. In our model, each node only needs
to maintain values of two parameters, the potential acceleration and the variance of acceleration
at time $k-1$ and measure the status at time $k$.



%We would like to predict the velocity of next time by predicting the acceleration $a$.
We define the following notations to represent the mobility status for node $C_i$ in Table 1. Note that all the notations of
acceleration and velocity are vectors.

\begin{table}[htp]
\caption{Notations for the Mobility Status}
\centering
\begin{tabular}{|c|c|}
%\hline
%\multicolumn{2}{|c|}{Notations for the  Mobility Status} \\
\hline
Notation & Meaning \\\hline
$v_{i_k}$ & The measured velocity at time $k$. \\\hline
$\hat{v_{i_k}}$ & The velocity predicted at time $k$. \\\hline
$a_{i_k}$ & The acceleration measured  at time $k$.\\\hline
$\hat{a_{i_k}^-}$ & The acceleration at time $k$ evolved \\
~~~~ & from time $k-1$.\\\hline
$\hat{a_{i_k}}$ & The potential acceleration at time $k$. \\\hline
 $p_{i_k}$ & The variance of acceleration updated \\
 ~~~~ & at time $k$.\\\hline
  $p_{i_k}^-$ & The variance of acceleration at time $k$ \\
  ~~~~ & evolved from time $k-1$.\\\hline
 $Q$ & The error or noise in the process.\\\hline
  $Kg_{i_k}$ & The blending factor at time $k$.\\
\hline
\end{tabular}
\label{table11}
\end{table}

%begin the additional content for the job talk
\noindent Input: At time $k$, node $C_i$ maintains\\
$v_{i_{k-1}}$, $\hat{a_{i_{k-1}}}$, and $p_{{i_k-1}}$. \\
$C_i$ also measures $v_{i_k}$.\\
Output: $C_i$ outputs its potential \\
%velocity $v_{i_{k+1}}$.\\
acceleration $\hat{a_{i_k}}$.\\
At time $k$, $C_i$  computes $a_{i_k}$.\\
$C_i$ updates $\hat{a_{i_k}^-}$ and $p_{i_k}^-$ in order to keep its historical moving trend to predict its future velocity.\\
$C_i$ also computes the blending factor $Kg_{i_k}$,
which indicates how much the acceleration changes from last time to current time.\\
$C_i$ computes its potential acceleration
$\hat{a_{i_k}}$. This acceleration will be used to predict its velocity for time $k+1$.\\
$C_i$ computes the velocity predicted for time $k+1$.\\
%end the content for the job talk

At time $k$, $C_i$  measures its velocity $v_{i_k}$. And then it computes $a_{i_k}$ as its measured acceleration  by
% $a_{i_k}$=$(v_{i_k}-v_{i_{k-1}})$/$\Delta$$t$ ~~ (1)\\
\[a_{i_k}=(v_{i_k}-v_{i_{k-1}})/\Delta t\]
Node $C_i$ updates $\hat{a_{i_k}^-}$ and $p_{i_k}^-$ in order to keep its historical moving trend to predict its future velocity.
% $\hat{a_{i_k}^-}$=$\hat{a_{i_{k-1}}}$ ~~(2)\\
\[\hat{a_{i_k}^-}=\hat{a_{i_{k-1}}} \]
\[p_{i_k}^-=p_{{i_k-1}}+Q  \]
Node $C_i$ also computes the blending factor $Kg_{i_k}$,
which indicates how much the acceleration changes from last time to current time.\\
\[Kg_{i_k}=p_{i_k}^-(p_{i_k}^-+Q)^{-1}=p_{i_k}^-/(p_{i_k}^-+Q) \]
% $Kg_{i_k}$=$p_{i_k}^-(p_{i_k}^-+Q)^{-1}$=$p_{i_k}^-/(p_{i_k}^-+Q)$ ~~(4)\\
Once $C_i$ obtains the blending factor $Kg_{i_k}$ and the evolved acceleration $\hat{a_{i_k}^-}$, it knows how much the acceleration changes and the
evolved acceleration. Additionally, $C_i$ considers the measured acceleration $a_{i_k}$. Then it computes its potential acceleration
$\hat{a_{i_k}}$. This acceleration will be used to predict its velocity for time $k+1$.
\[\hat{a_{i_k}}=\hat{a_{i_k}^-}+Kg_{i_k}(a_{i_k}-\hat{a_{i_k}^-}) \]
% $\hat{a_{i_k}}$=$\hat{a_{i_k}^-}$+$Kg_{i_k}(a_{i_k}-\hat{a_{i_k}^-})$ ~~(5)\\
$C_i$ updates the variance of acceleration for future utilization.
\[p_{i_k}=(1-Kg_{i_k})p_{i_k}^- \]
% $p_{i_k}$=(1-$Kg_{i_k}$)$p_{i_k}^-$ ~~(6)\\
Finally, the velocity predicted for time $k+1$ is
\[v_{i_{k+1}}=v_{i_k}+\hat{a_{i_k}}\Delta t \]
% $v_{i_{k+1}}=v_{i_k}+\hat{a_{i_k}}\Delta$$t$ ~~(7)\\
In the entire computation process at time $k$, $C_i$ only needs to measure its velocity $v_{i_k}$ and record two parameters
$\hat{a_{i_{k-1}}^-}$ and $p_{i_{k-1}}$. Then it can predict its velocity at time $k+1$ by the calculation.


\begin{comment}


\noindent Note that $\hat{v_{i_k}}$ will be obtained by the prediction of the velocity for time $k+1$.
And $\hat{a_{i_k}}$ will be obtained by the prediction of the acceleration for time $k+1$.\\


 $v_{i_k}$: the measured velocity at time $k$.\\
$\hat{v_{i_k}}$: the potential velocity at time $k$. It will be obtained by the prediction of the velocity for time $k+1$.\\
$a_{i_k}$: the acceleration measured by $(v_{i_k}-v_{i_{k-1}})/\Delta$$t$ at time $k$.\\
$\hat{a_{i_k}^-}$: the acceleration at time $k$ evolved from time $k-1$.\\
$\hat{a_{i_k}}$: the potential acceleration at time $k$. It will be obtained by the prediction of the acceleration for time $k+1$.\\
 $p_{i_k}$: the variance of acceleration updated at time $k$.\\
  $p_{i_k}^-$: the variance of acceleration at time $k$ evolved from time $k-1$.\\
 $Q$: the error or noise in the process.\\
  $Kg_{i_k}$: the blending factor at time $k$.\\


The idea of our approach is: at time $k$, node $c_i$ keeps the potential acceleration $\hat{a_{i_{k-1}}}$ and the variance of acceleration $p_{i_{k-1}}$ of previous time $k-1$, which was
calculated from time $k-2$.
The parameter $\hat{a_{i_{k-1}}}$ represents  $c_i$'s potential acceleration and $p_{i_{k-1}}$ represents how its acceleration changes. So the two parameters represent its moving trend. Then at time $k$, if node $c_i$ wants to predict its potential velocity at time $k+1$, it uses the two parameters of time $k-1$ to compute a
blending factor $Kg_{i_k}$. Further, it predicts its velocity at time $k+1$ by $Kg_{i_k}$ and  $a_{i_k}$.
In order to maintain the knowledge of its moving trend, node $c_i$ conducts the following update of every $\Delta$$t$:\\
$\hat{a_{i_k}^-}$=$\hat{a_{i_{k-1}}}$ ~~(1)\\
$p_{i_k}^-$=$p_{{i_k-1}}$+$Q$ ~~ (2)\\
$c_i$ also conducts the measurement update as follows:\\
$Kg_{i_k}$=$p_{i_k}^-(p_{i_k}^-+Q)^{-1}$=$p_{i_k}^-/(p_{i_k}^-+Q)$ ~~(3)\\
$\hat{a_{i_k}}$=$\hat{a_{i_k}^-}$+$Kg_{i_k}(a_{i_k}-\hat{a_{i_k}^-})$ ~~(4)\\
$e_{i_k}$=$|$$\hat{a_{i_k}^-}$-$\hat{a_{i_k}}$$|$=$|$$\hat{a_{i_{k-1}}}$-$\hat{a_{i_k}}$$|$ ~~(5)\\
%$p_{i_k}=E[e_{i_k}e_{i_k}^T]$ ~~(6)\\
$p_{i_k}$=(1-$Kg_{i_k}$)$p_{i_k}^-$ ~~(6)\\
%$\hat{a}$

\noindent At time $k$, node $c_i$ keeps the velocity $v_{i_{k-1}}$, variance $p_{i_{k-1}}$ and the potential acceleration $\hat{a_{i_{k-1}}^-}$ of time $k-1$.
$c_i$ can measure its velocity $v_{i_k}$ and compute the acceleration $a_{i_k}$ by $(v_{i_k}-v_{i_{k-1}})/\Delta$$t$. So the potential acceleration $\hat{a_{i_k}}$ at time $k$
can be computed by formula (4). Then the potential velocity at time $k+1$ can be achieved
by $v_{i_{k+1}}=v_{i_k}+\hat{a_{i_k}}\Delta$$t$. In this approach, $\hat{a_{i_{k-1}}^-}$ and $p_{i_{k-1}}$ represent  the changes of the moving status. Hence the historical mobility can be kept
only by the two parameters, which illustrate the moving trend of a node.
\end{comment}

The direction of the road may not be parallel or perpendicular
to the coordinate axes. Moreover, a vehicle may suddenly change its moving direction or speed. So we decompose
the velocity into two velocities parallel to the axes of the coordinate plane (Fig.~\ref{fig4})
to take care of the general scenarios.

\begin{figure}[!htp]
\begin{center}
\includegraphics[width=6.0cm]{m1020_4.eps}
\end{center}
\caption{Velocities of X and Y decomposition}
\label{fig4}
\end{figure}

In the general scenario, node $C_i$ computes its velocity $\hat{v_{i_{{k+1}_x}}}$  in  X direction and $\hat{v_{i_{{k+1}_y}}}$  in  Y direction at time $k+1$,
then computes $\hat{v_{i_{k+1}}}$=$\sqrt{ \hat{v_{i_{{k+1}_x}}}^{2}+\hat{v_{i_{{k+1}_y}}}^{2} }$. It further computes $T_i$ by $T_i=(R-|AC_i|)/$$|$$\hat{v_{i_{k+1}}}-v_A|$,
the time that node $C_i$ gets out of the range of $A$. Then $A$ can figure out the desired node $C_i$  with minimal $T_i$.


\begin{comment}


%In the scenario of Fig.~\ref{fig1}, we assume that the  moving direction of the vehicles and message broadcasting direction are identical.
%Moreover, the vehicles in opposite moving direction are not involved in the broadcasting process. In addition to this situation, there are some other scenarios. We list three of them in this paragraph and will discuss all in the Handle\_msg() algorithm.
%In Fig.~\ref{fig5}, from  $A$'s angle, the vehicle moving direction and message broadcasting direction are identical, and the vehicles in other moving direction are nothing to do with the broadcasting process.
In Fig.~\ref{fig5}, from  $A$'s angle, the vehicle moving direction and message broadcasting direction are identical, and the vehicles in both directions need to be
informed of the message. Another instance is
in Fig.~\ref{fig6}, from  $A$'s angle, the vehicle moving direction and message broadcasting direction are opposite, and the vehicles in other moving direction can help forward the broadcasting message, but they do not have to receive the message.
%A real world setting is, node $A$ was advertised a car accident message from $B$, and then $A$ is broadcasting the message to the node  $C$, $D$,...in its same moving direction. Then, $A$ selects one of the nodes from $E$, $F$...in its opposite moving direction to help  deliver  the message.
One more example is that the road is one way. The current broadcasting node can only select a node in its same moving direction to re-broadcast the message regardless whether the re-broadcasting direction is the same or the opposite direction of the mobility.

There are a number of factors that will affect how node $A$ selects the re-broadcasting node, including the type of the road (one way or two ways), the vehicles' moving direction, the message broadcasting direction, the areas of the
message receivers (the nodes in $A$'s same direction or opposite direction). %The combination of these factors will result a large number of scenarios. We only list three examples in this
We divide them into two categories by focusing on the selection of the re-broadcasting node. The first category is that
\end{comment}

From node $A$'s perspective, the moving direction of the vehicles and the message broadcasting direction can be identical or opposite.
When the moving direction and the broadcasting direction are identical (Fig.~\ref{fig5}), node $A$ broadcasts the message to its neighbores, and then selects the re-broadcasting node in the same moving direction based on the formulas
presented above.
% discussed in this paper.
%that can get out of $A$'s range in the same moving direction first. The selection criteria is based on formulas (1)-(7).
When the moving direction and the broadcasting direction are opposite (Fig.~\ref{fig6}),
%(the areas in its same direction, opposite direction or both).
node $A$ broadcasts the message to its neighbores, then it selects the re-broadcasting node from those
in the opposite moving direction that can get out of $A$'s range in the opposite moving direction first.

\begin{comment}
Otherwise, it selects a node (must be in the same moving direction) that can get out of $A$'s range in the opposite moving direction first.
Fig.~\ref{fig13} shows this scenario. In the one way road, $A$ selects node $E$, the slowest one behind it that can get out of $A$'s range in the opposite moving direction first. We can simply substitute the values of acceleration and velocity to the formulas (1)-(7) to compute the results because all parameters are vectors.
\end{comment}
%One more scenario is  that in addition to helping deliver the broadcasting message, the
%nodes in the opposite moving direction also need to be advised the message (Fig.~\ref{fig7}).

\begin{comment}
\begin{figure}[!htp]
\begin{center}
\includegraphics[width=8.0cm]{carcase_0.eps}
\end{center}
\caption{Case 0}
\label{fig45}
\end{figure}
\end{comment}

\begin{figure}[!htp]
\begin{center}
\includegraphics[width=8.0cm]{carcase_2.eps}
\end{center}
\caption{Moving direction and broadcasting direction are identical}
\label{fig5}
\end{figure}


\begin{figure}[!htp]
\begin{center}
\includegraphics[width=8.0cm]{carcase_3.eps}
\end{center}
\caption{Moving direction and broadcasting direction are opposite}
\label{fig6}
\end{figure}

%\begin{figure}[!htp]
%\begin{center}
%\includegraphics[width=8.0cm]{carcase_5.eps}
%\end{center}
%\caption{Scenario example 3}
%\label{fig13}
%\end{figure}

\begin{comment}
\begin{figure}[!htp]
\begin{center}
\includegraphics[width=8.0cm]{carcase_4.eps}
\end{center}
\caption{Case 4}
\label{fig7}
\end{figure}
\end{comment}

 \subsection{Algorithm Description}

%In our approach , at time $k$, each node updates and keeps its variance $p_{k-1}$ and the potential acceleration $\hat{a_{k}^-}$ of time $k-1$.
In the broadcasting process, the location of the initiator is included in the broadcasting message. Once a node receives a broadcasting message, it computes the distance to the
initiator. We can define a distance threshold. The messages are only broadcast within this threshold. If the distance is greater than the threshold, the node stops re-broadcasting. When
initiating a broadcasting message or upon receiving a re-broadcasting signal, a node calls the algorithm SFBB. The node handles different scenarios by the algorithm Handle\_msg.

\begin{comment}
Otherwise the node handles the following five cases.\\
Case 0: the broadcasting
direction and its moving direction are identical, and the nodes in its same moving direction don't need to be advised the broadcasting message, but the nodes in the opposite direction need. Then the node re-broadcasts
the message to its neighbors in its opposite moving direction and selects the re-broadcasting node in its same moving direction. In this case,
the re-broadcasting node only helps deliver the message (Fig.~\ref{fig45}).\\
Case 1: the broadcasting
direction and its moving direction are identical, and the nodes in opposite moving direction don't need to be advised the message. The node then re-broadcasts
the message to its neighbors in its same moving direction and selects the best candidate in its moving direction (Fig.~\ref{fig1}). \\
Case 2:
the broadcasting
direction and its moving direction are identical, and the nodes in its moving direction and opposite direction need to be advertised the message. Then the node re-broadcasts
the message to  its neighbors before it in its same moving direction and all its neighbors in its opposite moving direction, and then selects the best candidate from those in its same moving direction (Fig.~\ref{fig5}).  \\
Case 3: the broadcasting
direction and its moving direction are opposite, and the nodes in opposite moving don't need to be advertised the message. Then the node re-broadcasts
the message to  its neighbors behind  it in its moving direction, and then selects the best candidate from those in its
opposite moving direction (Fig.~\ref{fig6}).  \\
Case 4: the broadcasting
direction and its moving direction are opposite, and the nodes in opposite moving need to be advertised the message. Then the node re-broadcasts
the message to its neighbors behind  it in its moving direction and its neighbors in its opposite moving direction, and then selects the best candidate from those in its
opposite moving direction (Fig.~\ref{fig7}). \\
In our approach, each node periodically updates and keeps the acceleration variance, the potential acceleration and the velocity of the past time. When
initiating a broadcasting message or upon receiving a broadcasting message, a node handles it by the algorithm SFBB.

\end{comment}



\begin{figure}[hbt]
\baselineskip=10.2pt
% {\scriptsize
{\small
  \noindent\underline{\bf SFBB()} \\
  \text{~~~~}\textbf{if} it is the initiator\\
  \text{~~~~~~~~}  Call Handle\_msg.\\
  \text{~~~~}\textbf{elseif} the distance to the initiator is greater than the threshold \\
  \text{~~~~~~~~~~~~}Stop re-broadcasting; \\
  \text{~~~~}\textbf{else} Carry the message; \\
  \text{~~~~~~~~~~~~}Call Handle\_msg right after it gets out of the sender's\\
  \text{~~~~~~~~~~~~}   range.\\
   }

\protect\caption{SFBB algorithm}
\protect\label{routingfig}
\end{figure}


\begin{comment}

\begin{figure}[hbt]
\baselineskip=10.2pt
% {\scriptsize
{\small
  \noindent\underline{\bf  Handle\_msg()} \\
    \text{~~~~}  Switch (Receivers)\\
  \text{~~~~~~~~} case `Vehicles in the same moving direction' \\
  \text{~~~~~~~~~~~~} Broadcast the message to the vehicles in its same\\
   \text{~~~~~~~~~~~~}  moving direction; \\
    \text{~~~~~~~~~~~~}  Break; \\
  \text{~~~~~~~~} case `Vehicles in the opposite direction' \\
  \text{~~~~~~~~~~~~} Broadcast the message to the vehicles in its opposite\\
  \text{~~~~~~~~~~~~} moving direction; \\
  \text{~~~~~~~~~~~~}  Break; \\
  \text{~~~~~~~~~} case `Both directions' \\
  \text{~~~~~~~~~~~~} Broadcast the message to all the vehicles in its range; \\
  \text{~~~~~~~~~~~~}  Break; \\
  \text{~~~~}\textbf{if} moving direction and broadcasting are identical\\
  \text{~~~~~~} Select the node  in the moving direction  that can get out of its\\
  \text{~~~~~~} range firstly in the moving direction. \\
  \text{~~~~}\textbf{elseif} moving direction and broadcasting are different\\
  \text{~~~~~~}  \textbf{if} road type is two ways\\
  \text{~~~~~~~~~} Select the node from opposite lanes that can get out of its\\
  \text{~~~~~~~~~} range firstly opposite to the moving direction. \\
  \text{~~~~~~}  \textbf{else} Select the node from it moving direction that can get out\\
   \text{~~~~~~~~~~~~} of its range firstly opposite to the moving direction. \\
   \text{~~~~} Send a re-broadcasting signal to the node. \\


     }

\protect\caption{Handle\_msg algorithm}
\protect\label{routingfig1}
\end{figure}


\end{comment}



\begin{figure}[hbt]
\baselineskip=10.2pt
% {\scriptsize
{\small
  \noindent\underline{\bf  Handle\_msg()} \\
      \text{~~~} Broadcast the message to all the vehicles in its range; \\
      \text{~~~~}\textbf{if} moving direction and broadcasting are identical\\
  \text{~~~~~~} Select the node  in the moving direction  that can get out of its\\
  \text{~~~~~~} range first in the moving direction. \\
  \text{~~~~}\textbf{elseif} moving direction and broadcasting are different\\
   \text{~~~~~~~~~} Select the node from the opposite moving direction that can\\
  \text{~~~~~~~~~}  get out of its range first opposite to the moving direction. \\
    \text{~~~} Send a re-broadcasting signal to the node. \\

     }

\protect\caption{Handle\_msg algorithm}
\protect\label{routingfig1}
\end{figure}


\begin{comment}
{\small
  \noindent\underline{\bf SFBB()} \\
  \text{~~~~}\textbf{if} the distance to the initiator is greater than the threshold \\
  \text{~~~~~~~~}stop re-broadcasting; \\
  \text{~~~~}\textbf{else} carry the message; \\
  \text{~~~~~~~~~~~~}Handle the message according to the following five cases right after it gets out of the sender's range;\\
  \text{~~~~~~~~~~~~}Case 0: re-broadcast the message to its neighbors in its opposite moving direction;\\
  \text{~~~~~~~~~~~~~~~~}collect the moving status of its neighbors before it in its same moving direction; \\
  \text{~~~~~~~~~~~~~~~~}select and designate the best node to conduct re-broadcasting; \\
  \text{~~~~~~~~~~~~}Case 1: re-broadcast the message to its neighbors before it in its same moving direction;\\
  \text{~~~~~~~~~~~~~~~~}collect the moving status of its neighbors before it in its moving direction; \\
  \text{~~~~~~~~~~~~~~~~}select and designate the best node to conduct re-broadcasting; \\
  \text{~~~~~~~~~~~~}Case 2: re-broadcast
the message to  its neighbors before it in its same moving direction and all its neighbors in its opposite moving direction;\\
  \text{~~~~~~~~~~~~~~~~}collect the moving status of its neighbors before it in its moving direction; \\
  \text{~~~~~~~~~~~~~~~~}select and designate the best node to conduct re-broadcasting; \\
  \text{~~~~~~~~~~~~}Case 3: re-broadcast the message to  its neighbors behind  it in its moving direction;\\
  \text{~~~~~~~~~~~~~~~~}collect the moving status of its neighbors in its opposite moving direction; \\
  \text{~~~~~~~~~~~~~~~~}select and designate the best node to conduct re-broadcasting; \\
  \text{~~~~~~~~~~~~}Case 4: re-broadcast
the message to its neighbors behind  it in its moving direction and its neighbors in its opposite moving direction;\\
  \text{~~~~~~~~~~~~~~~~}collect the moving status of its neighbors in its opposite moving direction; \\
  \text{~~~~~~~~~~~~~~~~}select and designate the best node to conduct re-broadcasting; \\
 }
\end{comment}


==> figures/SFBB/simulation.tex <==
\section{Performance Evaluation}
\label{evaluation}


\begin{figure}
% \begin{figure}[!htp]
\begin{center}
\includegraphics[width=8.0cm]{g1.eps}
\end{center}
% \vspace{-0.1in}
\caption{The packet delivery ratio}
\label{fig15}
\end{figure}



\begin{figure}
% \begin{figure}[!htp]
\begin{center}
\includegraphics[width=8.0cm]{g22.eps}
\end{center}
% \vspace{-0.1in}
\caption{The end-to-end delay}
\label{fig16}
\end{figure}


\begin{figure}
% \begin{figure}[!htp]
% \vspace{-0.32in}
\begin{center}
\includegraphics[width=8.0cm]{g3.eps}
\end{center}
\vspace{-0.1in}
\caption{The packet delivery ratio}
\label{fig19}
\end{figure}

We conduct simulations using the GloMoSim wireless network simulator~\cite{ex27}.
We use the tool BonnMotion~\cite{ex28} to generate mobile nodes.
The mobility mode we use is ``ManhattanGrid," which can generate the
nodes distributed in the areas similar to roads or streets.
The size of the environment is 2000X2000 $m^2$.
The number of vehicles varies from 50  to 300 with an increment of 50. We set the average packet generation rate from 0.1 to 0.9 per second.
The packet generation rate represents the number of packets generated by a node per second.
The MAC protocol is 802.11.


Many broadcasting protocols are based on the idea that the current sender selects
the node that is farthest away from itself to conduct the re-broadcast task.
This method is called ``DIST'' in the comparison.
We compare our statistical filter based broadcast protocol ``SFBB'' with the ``DIST'' method
using two metrics.
% are considered in our simulation.
The first one is the package delivery ratio, which
is the ratio of the number of vehicles that receive the broadcasting message over the total number of vehicles.
The second metric is the end-to-end delay. 
It is the time elapsed from the packet generated until the packet reaches the receiver in the desired area.
%It is the time elapsed between the instant the packet enters the re-broadcasting node and
%the reception time of the packet by another node.
%To evaluate the two metrics, the number of nodes is varied from 50 to 300
%with an increment of 50. We also set the packet generation rate to vary from 0.1 up to 0.9 per second.





Fig.~\ref{fig15} shows the average packet delivery ratio when the number of nodes 
changes from 50 to 300 and the average packet generation rate is fixed at 0.5.
The delivery ratio decreases when the number of nodes increases.
This is 
because 802.11 protocol performs poorly with more nodes due to the
packet collision. We can see that the ratio generated by SFBB is 9.2\% higher than DIST overall because SFBB can broadcast
a message in a new place faster with less collision than DIST. 
% And less collision exists in the new place.




\begin{figure}
% \begin{figure}[!htp]
% \vspace{-0.82in}
\begin{center}
\includegraphics[width=8.0cm]{g44.eps}
\end{center}
\vspace{-0.1in}
\caption{The end-to-end delay}
\label{fig20}
\end{figure}



Fig.~\ref{fig16} shows the average end-to-end delay with the same configuration as Fig.~\ref{fig15}.
It illustrates the end-to-end delay of SFBB is 9.1\% lower than that of DIST overall.
This is because SFBB can select the
fastest one to re-broadcast the message.




Fig.~\ref{fig19} presents the packet delivery ratio when the packet generation rate varies from
0.1 to 0.9 and the number of nodes is fixed at 150. Similar to Fig.~\ref{fig15}, the ratio decreases when the value of the packet generation rate increases.
%  due to the collision of dense packets.
This figure indicates that the delivery ratio of SFBB is 9.4\% higher than DIST overall because
the re-broadcasting nodes selected by SFBB enter a new place with less collision
faster than DIST. Fig.~\ref{fig20} shows that the end-to-end delay of the two approaches. 
Again, SFBB has a small end-to-end delay than the DIST method. Overall SFBB is 9.0\% lower than DIST.



